Leading higher-derivative corrections to Kerr geometry

We compute the most general leading-order correction to Kerr solution when the Einstein-Hilbert action is supplemented with higher-derivative terms, including the possibility of dynamical couplings controlled by scalars. The model we present depends on five parameters and it contains, as particular cases, Einstein-dilaton-Gauss-Bonnet gravity, dynamical Chern-Simons gravity and the effective action coming from Heterotic Superstring theory. By solving the corrected field equations, we find the modified Kerr metric that describes rotating black holes in these theories. We express the solution as a series in the spin parameter $\chi$, and we show that including enough terms in the expansion we are able to describe black holes with large spin. For the computations in the text we use an expansion up to order $\chi^{14}$, which is accurate for $\chi<0.7$, but we provide as well a Mathematica notebook that computes the solution at any given order. We study several properties of the corrected black holes, such as geometry of the horizon, ergosphere, light rings and scalar hair. Some of the corrections violate parity, and we highlight in those cases plots of horizons and ergospheres without $\mathbb{Z}_{2}$ symmetry.

==> JHEP3.cls.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%% JHEP.cls 3.1.2 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%
%% This file is Copyright JHEP 2002:  it can be freely distributed  but
%% NOT modified preserving its name, even in similar forms.
%% 
%% JHEP3.cls is a LaTeX2e class file used to typeset manuscripts in JHEP
%% style. It was written by F. Nesti as a (radical) modification of the
%% class `article.cls' from distribution 960601 of LaTeX2e.
%% 
%% For bugs, comments, suggestions email to nesti@medialab.sissa.it
%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% \CharacterTable
%%  {Upper-case    \A\B\C\D\E\F\G\H\I\J\K\L\M\N\O\P\Q\R\S\T\U\V\W\X\Y\Z
%%   Lower-case    \a\b\c\d\e\f\g\h\i\j\k\l\m\n\o\p\q\r\s\t\u\v\w\x\y\z
%%   Digits        \0\1\2\3\4\5\6\7\8\9
%%   Exclamation   \!     Double quote  \"     Hash (number) \#
%%   Dollar        \$     Percent       \%     Ampersand     \&
%%   Acute accent  \'     Left paren    \(     Right paren   \)
%%   Asterisk      \*     Plus          \+     Comma         \,
%%   Minus         \-     Point         \.     Solidus       \/
%%   Colon         \:     Semicolon     \;     Less than     \<
%%   Equals        \=     Greater than  \>     Question mark \?
%%   Commercial at \@     Left bracket  \[     Backslash     \\
%%   Right bracket \]     Circumflex    \^     Underscore    \_
%%   Grave accent  \`     Left brace    \{     Vertical bar  \|
%%   Right brace   \}     Tilde         \~}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  ***:to do  **?:question  ...:to choose  XXX:to delete  ???:unknown %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\NeedsTeXFormat{LaTeX2e}[1995/12/01]
\ProvidesClass{JHEP3} [2003/01/03 v3.1.2 LaTeX document class - F.N.]

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\logo{\raisebox{-10.5\p@}{\hb@xt@85\p@{\special{psfile=JHEPlogo.eps}\hfil}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% NEW SWITCHES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@preprint\@preprinttrue		% DEFAULT IS PREPRINT!
\newif\if@draft   \@draftfalse			% DEFAULT IS NOT DRAFT
\newif\if@hyper   \@hypertrue			% DEFAULT IS HYPER
\newif\if@proc	  \@procfalse			% DEFAULT IS NOT PROC

%\newif\if@title\@titlefalse			%
\newif\if@author\@authorfalse			%
\newif\if@abstract\@abstractfalse		% FOR FRONTMATTER DECLARATIONS
\newif\if@keywords\@keywordsfalse		%
\newif\if@todotoc\@todotocfalse			%
\newif\if@rece\@recefalse			%
\newif\if@revi\@revifalse			%
\newif\if@acce\@accefalse			%
\newif\if@Jcopy\@Jcopyfalse			%
\newif\if@JHEP\@JHEPfalse			%
\newif\if@conf\@conffalse			%
\newif\if@Jspecialurl\@Jspecialurlfalse
%\newif\if@restonecol
\@twocolumnfalse

\if@compatibility
    \setlength\paperheight {297mm}%		% DEFAULT FOR LATEX209 IS a4
    \setlength\paperwidth  {210mm}%
\else						% CHOSE PAPER:
\DeclareOption{a4paper}
   {\setlength\paperheight {297mm}%
    \setlength\paperwidth  {210mm}}
\DeclareOption{a5paper}{\@OImess{}}		% IGNORED a5
\DeclareOption{b5paper}{\@OImess{}}		% IGNORED b5
\DeclareOption{letterpaper}
   {\setlength\paperheight {11in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{legalpaper}
   {\setlength\paperheight {14in}%
    \setlength\paperwidth  {8.5in}}
\DeclareOption{executivepaper}
   {\setlength\paperheight {10.5in}%
    \setlength\paperwidth  {7.25in}}
\DeclareOption{landscape}{\@OImess{}}		% IGNORED landscape
\fi

\newcommand\@ptsize{1}                          % DEFAULT SIZE IS 11 PT

\DeclareOption{proceedings}{\@preprintfalse\@proctrue
			   \renewcommand\@ptsize{1}% PROCS: 11 PT
			   \AtBeginDocument{\@todotocfalse}}
\DeclareOption{published}{\@preprintfalse}

\DeclareOption{hyper}{\@hypertrue}	% HYPER IS 11 PT
%\DeclareOption{screen}{\@hypertrue}	% HYPER IS 11 PT
\DeclareOption{nohyper}{\@hyperfalse}	% PAPER IS ALSO 11 PT (v1.3)
\DeclareOption{paper}{\@hyperfalse}	% PAPER IS ALSO 11 PT
\DeclareOption{11pt}{\renewcommand\@ptsize{1}\ExecuteOptions{@FONT}}
\DeclareOption{12pt}{\renewcommand\@ptsize{2}\ExecuteOptions{@FONT}}
\if@compatibility\else                          % LATEX2.09 HAS NO 10PT 
\DeclareOption{10pt}{\renewcommand\@ptsize{0}\ExecuteOptions{@FONT}}% v1.4
\fi       				% CHOSEN TO FREE MEMORY LATER:
\DeclareOption{@FONT}{\if@preprint              % IF PREPRINT ALLOW ANY,
                        \else			% IF PROCEEDINGS OR PUBLISHED: 
%			\if@proc		% 
%			\renewcommand\@ptsize{0}\@NFmess{10pt}% ALWAYS 10PT
%			\else
			\renewcommand\@ptsize{1}\@NFmess{11pt}% ALWAYS 11PT
                        \fi%\fi
			}
                        
\if@compatibility\else
\DeclareOption{oneside}{\@twosidefalse \@mparswitchfalse}\fi
\DeclareOption{twoside}{\if@preprint\if@hyper\@OImess{ in hyper-mode}
				    \else\@twosidetrue\@mparswitchtrue\fi
			\else			% FOR PROCEED./PUBLIC.:
			\@OImess{ in published papers}
			\fi}
\DeclareOption{notoc}{\if@preprint		% to disable TOC
			\AtBeginDocument{\@todotocfalse}
			\else
			\if@proc\@OImess{ is automatic for proceedings}
			\else\@OImess{ in JHEP papers}\fi\fi}
\DeclareOption{draft}{\setlength\overfullrule{5pt}% EXTENDED DRAFT
	\newcount\hour\newcount\minute
	\hour=\time \divide\hour by60 \minute=\time
	{\multiply\hour by60 \global\advance\minute by-\hour}
	\edef\militarytime{\number\hour:\ifnum\minute<10 0\fi\number\minute}
	\let\old@eqnnum\@eqnnum
	\def\@eqnnum{\old@eqnnum\rlap{\kern\marginparsep
				\if@twocolumn\if@firstcolumn
				  \kern-2\marginparsep\kern-\columnwidth\
				  \llap\bgroup\else\bgroup\fi
				\else
				\if@twoside\ifodd\c@page
				  \kern-2\marginparsep\kern-\textwidth
				  \llap\bgroup\else\bgroup\fi
				\else\bgroup\fi				
				\fi
				\sf\scriptsize\@eqnlabel\egroup}%
				\gdef\@eqnlabel{}}
	\let\@eqnlabel\relax
	\def\math@note#1{\gdef\@eqnlabel{LAB: #1}}
	\def\norm@note#1#2{\special{}% SORRY AGAIN.
			 \ifinner{\ifdim\baselineskip=\z@% IN ARRAY..
					\baselineskip18\p@\fi%%
				\ifhmode%   ATTENTION TO RESTRICTED VMODE!
				\raisebox{.5\baselineskip}[\z@][\z@]{%
					\rlap{\sf\scriptsize #2}}%
				\else\vskip-\baselineskip%
				\raisebox{-.6\baselineskip}[\z@][\z@]{%
						\rlap{\sf\scriptsize #2}}%
				\fi}%
			 \else\marginpar{\raggedright\if@twoside\ifodd\c@page%
					\raggedleft\fi\fi\sf\scriptsize #1#2}%
			 \fi}%
	\AtBeginDocument{\newbox\drft@box\setbox\drft@box=\hbox{%
			\framebox[\textwidth]{\sf\small JHEP 3.1 DRAFT 
			\ttfamily(\cur@opt)\hfill\sf\bfseries\jobname\sf, 
			\today, \militarytime}}}
	\@drafttrue}

%\if@compatibility\else
%\DeclareOption{final}{\setlength\overfullrule{\z@}} % ***? NO FINAL?
%\fi
\DeclareOption{titlepage}{\@OImess{}}		% IGNORED
\if@compatibility\else
\DeclareOption{notitlepage}{\@OImess{}}		% IGNORED
\fi
\if@compatibility\else
\DeclareOption{onecolumn}{\@OImess{}}		% IGNORED
\fi
\DeclareOption{twocolumn}{\@OImess{}}		% IGNORED
\DeclareOption{leqno}{\@OImess{}}	%\input{leqno.clo}} IGNORED ...
\DeclareOption{fleqn}{\@OImess{}}	%\input{fleqn.clo}} IGNORED ...
\DeclareOption{openbib}{\@OImess{}}		% IGNORED


%%%%%%%%%%%%%%%%%%%%%%%%%%%%% MESSAGES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\JHEP@mess[1]{\typeout{Class JHEP Message: \protect#1.}}%
\newcommand\JHEP@warn[1]{\ClassWarning{JHEP}{#1}}
\newcommand\JHEP@warnl[1]{\ClassWarningNoLine{JHEP}{#1}}
\newcommand\JHEP@igno[1]{\JHEP@warn{IGNORED \protect#1}}
\newcommand\JHEP@ignol[1]{\JHEP@warnl{IGNORED \protect#1}}
\newcommand\@OImess[1]{\JHEP@ignol{OPTION '\CurrentOption'#1}}
\newcommand\@NFmess[1]{\JHEP@mess{Normalsize set to #1}}
\newcommand\@ENVwarn[1]{\JHEP@warn{Please use \protect#1 in place 
						of LaTeX environment}}
%%%%%%%%%%%%%%%%%%%%%%%%%% PROCESS OPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\ExecuteOptions{a4paper,oneside,hyper} %WERE ALSO 10pt,onecolumn
\ProcessOptions

%%%%%%%%%%%%%%%%%%%%%%%%%% REQUIRED PACKAGES %%%%%%%%%%%%%%%%%%%%%%%%%%
\RequirePackage{amssymb}
%\RequirePackage{cite}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%% START CODE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{size1\@ptsize.clo}
\renewcommand{\baselinestretch}{1.1}\normalsize
\setlength\lineskip{1\p@}
\setlength\parindent{1.2\parindent}	% AT 12pt 1.5em BECOMES 1.8em=tocindent
\setlength\normallineskip{1\p@}
\setlength\parskip{0\p@ \@plus \p@}
\@lowpenalty   51
\@medpenalty  151
\@highpenalty 301
\widowpenalty 1000
\clubpenalty 1000

\setcounter{topnumber}{3}
\renewcommand\topfraction{.95} % default .7
\setcounter{bottomnumber}{1}
\renewcommand\bottomfraction{.6} %.2		% .6 ???***
\setcounter{totalnumber}{3}
\renewcommand\textfraction{.05}
\renewcommand\floatpagefraction{1}
\setcounter{dbltopnumber}{3}
\renewcommand\dbltopfraction{.7}
\renewcommand\dblfloatpagefraction{1}

\textwidth  .72\paperwidth	% WIDTH OF TEXT, REMAINS .28% FOR MARGINS
%
\setlength\@tempdima{.76\paperheight}	% HEIGHT OF TEXT WITH FOOTNOTES
\divide\@tempdima\baselineskip		% EXCLUDING HEAD (AND FOOT)
\@tempcnta=\@tempdima			% rounded to integer (#lines-1)
\setlength\textheight{\@tempcnta\baselineskip}
\addtolength\textheight{\topskip}

\voffset -1in
\topmargin   .05\paperheight	% FROM TOP OF PAGE TO TOP OF HEADING (0=1inch)
\headheight  .02\paperheight	% HEIGHT OF HEADING BOX.
\headsep     .03\paperheight	% VERT. SPACE BETWEEN HEAD AND TEXT.
\footskip    .07\paperheight	% FROM END OF TEX TO BASE OF FOOTER. (40pt)

\marginparsep 9\p@		% HOR. SPACE BETWEEN TEXT AND MARGINAL NOTE
\marginparpush 6\p@		% MIN. VERT. SPACE BETWEEN MARGINAL NOTES

\hoffset -1in				% TO ADJUST WITH PAPER:
\if@twoside				% IF TWO-SIDED:
	\oddsidemargin .13\paperwidth	% LEFT MARGIN FOR ODD PAGES (10)
	\evensidemargin .15\paperwidth	% LEFT MARGIN FOR EVEN PAGES (30)
	\marginparwidth .10\paperwidth	% TEXTWIDTH OF MARGINALNOTES
	\reversemarginpar		% BECAUSE OF TITLEPAGE.
\else					% IF ONE-SIDED:
	\oddsidemargin .14\paperwidth	% LEFT MARGIN FOR ODD PAGES (20)
	\evensidemargin .14\paperwidth	% LEFT MARGIN FOR EVEN PAGES (20)
	\marginparwidth .11\paperwidth	% TEXTWIDTH OF MARGINALNOTES
\fi					%
%%%%%%%%%%%%%%%%%%%%%%% HYPER (AND DRAFT) STUFF %%%%%%%%%%%%%%%%%%%%%%%
%\let\textref\@gobble
%\if@hyper			% IF NOHYPER WE DO LESS DAMAGE AS POSSIBLE.***
\@ifundefined{pdfoutput}{}{\input pdfcolor.tex} % PDFTEX has \pdfoutput 

\bgroup\catcode`\#=12\gdef\hash{#}\egroup	% DEFINED \hash=#.
%\fi
\def\H@tilde{\string~}
\newcommand{\href}[2]{\rule{0pt}{0pt}\bgroup\let~\H@tilde
			\if@hyper\@ifundefined{pdfoutput}{%
				    \noexpand\special{html:<A href="#1">}%
				  }{%
				    \def\hash{}%
				    \pdfannotlink attr{%/C [0 .7 .9]
					/Border [0 0 0]} goto name{#1}%
					\pdfsetcolor{.9 .9 0 0}%
%
				  }\fi
			{#2}\rule{0pt}{0pt}\egroup
			\if@hyper\@ifundefined{pdfoutput}{%
				    \special{html:</A>}%
				  }{%
				    \Black\pdfendlink
				  }\fi
		     }

\newcommand{\name}[1]{\if@hyper\@ifundefined{pdfoutput}{%
				    \noexpand\special% NAME HAS NO TAGGED TEXT HERE.
					{html:<A name="#1">}\special{html:</A>}%
				  }{%
				    \pdfdest name{#1} fith%
				  }\fi
		     }
\newcommand{\base}[1]{\if@hyper\bgroup\let~\H@tilde
			\noexpand\special	% BASE HAS NO TAGGED TEXT.
			{html:<base href="#1">}\egroup\fi}
%------------------------------------------------------------------%
% SECTION TAGS and  THEIR REFERENCE IN TOC \d@t will be '.' for sections only
\if@hyper
\renewcommand{\@seccntformat}[1]{\name{sec\csname the#1\endcsname}%
				 \csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{\href
			      {\hash\hyp@typ#1}{#1}\d@t\hfil}}
\else
\renewcommand{\@seccntformat}[1]{\csname the#1\endcsname\d@t\hspace{1ex}}
\renewcommand{\numberline}[1]{\hb@xt@\@tempdima{#1\d@t\hfil}}
\fi
%------------------------------------------------------------------%
% CITATION TAGS ARE TOGETHER WITH BIB STUFF.
% CITATION HREF
\def\@citex[#1]#2{%			% UNFORTUNATELY REDEFINED!!!!
  \let\@citea\@empty
  \@cite{\@for\@citeb:=#2\do
    {\@citea\def\@citea{,\penalty\@m\ }%
     \edef\@citeb{\expandafter\@firstofone\@citeb}%
     \if@filesw\immediate\write\@auxout{\string\citation{\@citeb}}\fi
     \@ifundefined{b@\@citeb}{\mbox{\reset@font\bfseries ?}%
	\G@refundefinedtrue
	\@latex@warning
	  {Citation `\@citeb' on page \thepage \space undefined}}%
	{\edef\tmp@bn{\csname b@\@citeb\endcsname}%
	 \hbox{\href{\hash bib\tmp@bn}{\tmp@bn}}}}}{#1}%		% **HYPER**
	 \if@draft\norm@note{CIT: }{#2}\fi			% **DRAFT**
	 }

%-----------------------------------------------------------------%
% LABEL, REF AND PAGEREF, TEXTREF, ~ COMPATIBLE:
\let\old@label\label						% OLD LATEX COMMAND.
\def\label{\bgroup\catcode`\>=15\catcode`\"=15 \@@label}		
\newcommand{\@@label}[1]{\egroup\name{ref-#1}%		% LABEL IN HYPER TAG.
			 \old@label{#1}%		% 
			 \if@draft%			% DRAFT:
			 \ifmmode\math@note{#1}%
			 \else\norm@note{}{LAB: #1}\fi%
			 \fi%
			 }
\if@hyper
\let\old@ref\ref \let\old@pageref\pageref		% OLD LATEX COMMANDS.
\renewcommand{\ref}[1]{\@ifundefined{r@#1}{}{\href{\hash ref-#1}}%
		       {\old@ref{#1}}} % LABEL INSIDE HREF.
\renewcommand{\pageref}[1]{\@ifundefined{r@#1}{}{%	% UNDEFINED => NO HREF
	      \edef\tmp@ref{\noexpand\@secondoftwo\csname r@#1\endcsname}%
	      \href{\hash pag\tmp@ref}}{\old@pageref{#1}}}
\fi
\newcommand{\textref}[2]{\@ifundefined{r@#1}
			{%
			\protect\G@refundefinedtrue
			\nfss@text{\reset@font\bfseries ?#2?}%
   			\@latex@warning{Reference `#1' on page \thepage \space
				             undefined}}
			{\vrule height \z@ width \z@\href{\hash ref-#1}{#2}}}
%------------------------------------------------------------------%
%%%%%%%%%%%%%%%%%%%%%%%%%% END HYPER-STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%% JHEP HEADINGS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\ps@JHEP{% 			
    \def\@oddfoot{\ifnum\thepage=0\ifnum\Jacce@year>2001\if@JHEP
		\Jcopyright@box\fi\hfill % copyright only on front page of published papers
		\if@Jspecialurl\unhbox\Jspecial@url\else\if@JHEP\unhbox\Jpaper@url\fi\fi\fi %possible url
		\else\reset@font\hfil-- \thepage\ --\hfil\fi} % page numbers on other pages
    \if@draft\edef\cur@opt{\@curroptions}\fi
    \def\@oddhead{\name{pag\thepage}\hfil\if@draft\copy\drft@box\fi}
    \if@proc
	\def\@oddhead{\name{pag\thepage}%
		      \smash{\if@draft\raise 2.5em\rlap{\copy\drft@box}\fi
		      	     \vbox{\hsize=\textwidth\noindent
			     \copy\conf@box\hfill
			     \copy\@firstaubox\vskip.17em \hrule}}%
		      }%
    \fi
    \if@twoside\let\@evenhead\@oddhead\let\@evenfoot\@oddfoot\fi
    \let\@mkboth\@gobbletwo
    \let\sectionmark\@gobble
    \let\subsectionmark\@gobble
    }
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TITLE PAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\maketitle{\JHEP@ignol{\maketitle}}
\newcommand\auto@maketitle{\begingroup
    \renewcommand\thefootnote{\@fnsymbol\c@footnote}%
    \def\@makefnmark{\rlap{\@textsuperscript{\normalfont\@thefnmark}}}%
    \long\def\@makefntext##1{\parindent 1em\noindent
            \hb@xt@1.8em{\hss\@textsuperscript{\normalfont\@thefnmark}}##1}%
    \let\footnote\thanks%
	\newpage				%
	\if@proc				% IF PROCEEDINGS: 
	 \global\let\@nodocument\relax		% LaTeX FOULED:)
	\@maketitle				% 
	 \@thanks				% TITLE THANKS IN 1st COLUMN
	 \let\@evenfoot\@empty			% NO PAGENO.
 	 \let\@oddfoot\@empty
	 \setcounter{page}{1}%
	 \thispagestyle{empty}%			% PROCS HAVE NO PAGENUMBER
	\else
	 \@maketitle				% CALL ACTUAL FORMATTING
	 \@thanks				% TITLE THANKS
	 %\let\@evenfoot\@empty			% NO PAGENO.
 	 %\let\@oddfoot\@empty
	 \thispagestyle{JHEP} 
 	 \setcounter{page}\z@
	 \newpage				% FINE PAGINA
	\fi	
  \endgroup
  \setcounter{footnote}{0}%			
  \if@todotoc					% IF THERE IS A SECTION
      \noindent\rule\textwidth{.1pt}		% THEN MAKE TOC...
      \vskip 2em \@plus 3ex \@minus 3ex
      \tableofcontents
      \vskip 2em \@plus 3ex \@minus 3ex
      \noindent\rule\textwidth{.1pt}
      \vskip 2em \@plus 3ex \@minus 3ex
  \fi
  \if@preprint\else
  	\if@proc
	  \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space there is no toc in proceedings}}
  	\else
	  \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space is automatic}}
  	\fi
  \fi
  \global\let\thanks\@gobble
%  \setbox\@tmpbox=\vbox{\rm\@author}%		% FOR PROCS RESET HEADERS
%  \global\let\maketitle\relax			% NO LONGER EXISTS.
  \global\let\@maketitle\relax			%
  \global\let\@thanks\@empty			%
  \global\let\@author\@empty			% KILL ALL 
  \global\let\@date\@empty			%
  \global\let\@title\@empty			%
  \global\let\@abstract\@empty			%
  \global\let\title\relax			%
  \global\let\author\relax			%
  \global\let\date\relax			%
  \global\let\and\relax				%
  \global\let\email\@gobble
  \global\let\received\relax
  \global\let\revised\relax
  \global\let\accepted\relax
  \global\let\JHEPcopydate\relax
  \global\let\JHEPspecialurl\relax
  \global\let\keywords\relax
  \global\let\endkeywords\relax
}
%%%%%%%%%%%%%%%%%%%%%%%%%% ACTUAL TITLEPAGE %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newskip\titlesk@pa \newskip\titlesk@ja		% Skips for titlepage
\newskip\titlesk@pb \newskip\titlesk@jb		%
\newskip\titlesk@pc \newskip\titlesk@jc		%
\newskip\titlesk@pd				%
\titlesk@pa= 1.6em plus .4em%			% Before title (papers)
\titlesk@pb= 2em   plus .06em minus  .5ex%	% Between title/rule
\titlesk@pc= 2em   plus .05em minus 1.2ex%	% Before authors
\titlesk@pd= 2em   plus .06em minus  .5ex%	% After proc rule      	 
\titlesk@ja= 1.6em plus .4fil%			% Before title (proceedings)
\titlesk@jb= 2em   plus .06fil minus  .5ex%	% Between title/rule
\titlesk@jc= 2em   plus .05fil minus 1.2ex%	% Before authors

\def\@maketitle{%				% PAGE IS FLUSHED LEFT
\begin{flushleft}%				% PAY ATTENTION TO \par'S
%header for preprints
\if@preprint					%%% PREPRINT HEADER: 
\vskip-7em					%
\underline{\tiny Preprint typeset 		%
                 in JHEP style -		%
  		\if@hyper{HYPER VERSION}	%
		\else{PAPER VERSION}\fi } 	%
\normalsize\hfill%				% *** MAYBE PUT IN A ZERO BOX
\begin{tabular}[t]{r}\@preprint\end{tabular}% % PREPRINT NUMBERS
\else						%
  % header for proceedings
  \if@proc					%%% PROCEEDINGS: LOGO ETC..
    \vskip-4.48em\hfill\copy\conf@box
    \vskip-.7\baselineskip\logo\hrulefill
    \vskip-.4\baselineskip\hskip32\p@%	        % *** IDEM BOXIZE
		{\tiny PROCEEDINGS}
  \else
  % 					        %%% PUBLISHED: LOGO  ETC..
  %header for published (after 2001)
    \ifnum\Jacce@year>2001
       \vskip-7em\hfill
       {\small\scshape Published by Institute of Physics 
	               Publishing for SISSA/ISAS}
       \vskip-.7\baselineskip\logo\hrulefill
       \vskip-1.5\baselineskip\hskip21.73\p@%	% *** IDEM BOXIZE
       \hfill{\parbox[t]{30em}{\begin{flushright}\setlength\baselineskip{11pt}\footnotesize
				\Jrece@cs\\
				\if@revi\Jrevi@cs\\\fi
				\Jacce@cs
			      \end{flushright}}}%
    \else
    % header for published (december 2001)  *** TO BE REMOVED IN JHEP4...
    \vskip-7em\hfill{\small\Jrece@cs{\it,\ }\Jacce@cs
    \vskip-.7\baselineskip\logo\hrulefill
    \vskip-.5\baselineskip\hskip23\p@%	% *** IDEM BOXIZE
 		{\tiny \if@hyper{HYPER VERSION}\else{PAPER VERSION}\fi}
    \if@revi\hfill\Jrevi@cs\fi}

    \fi
  \fi
\fi\null
% end headers
% title page: skips are different for procs (p) and jhep or preprints (j)
% see above
  \if@proc
   \vskip \titlesk@pa
  \else
   \vskip \titlesk@ja		   % vspace before title
  \fi
% TITLE 
  {\LARGE \sffamily                
        \bfseries                  
        \@title\par}%                large sans-serif bf
  \if@proc
    \vskip \titlesk@pb             
  \else
    \vskip \titlesk@jb             % vspace between title and rule
  \fi
  \if@proc
% RULE
    \hrule height \p@%               for proc = 1pt
  \else
    \hrule height 1.5\p@%            otherwise = 1.5pt.
  \fi
  \if@proc
    \vskip \titlesk@pb             
  \else
    \vskip \titlesk@jb		   % vspace between rule and authors
  \fi
% AUTHORS\\ADDRESSES
  \vskip-\auth@skip
  {\normalsize \bfseries \sffamily
	\@author \par}                            
  \if@proc
    \vskip \titlesk@pc
  \else
    \vskip \titlesk@jc             % vspace between authors and abstract
  \fi
% ABSTRACT IF PRESENT (SHOULD)
  \if@proc
    \centerline{\parbox{.9\textwidth}%	% narrower abstract for proceedings
		    {\abstract@cs}}%
  \else
    \parbox\textwidth{\abstract@cs}%	
  \fi
  \normalsize
% KEYWORDS IF PRESENT
  \if@keywords	
    \if@proc
	\vskip \titlesk@pc	   
    \else
	\vskip .9\titlesk@jc	   % vspace between abstract and keywords
    \fi
    \par
    \@keywords				
  \fi
% DEDICATION, IF PRESENT
  \dedic@box				
% RULE (only for procs)
  \if@proc
    \vskip \titlesk@pb
    \hrule height 1\p@
    \vskip \titlesk@pd
  \fi
\end{flushleft}%			% FINISHED.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%% STANDARD STUFF %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\setcounter{secnumdepth}{3}
\newcounter {part}
\newcounter {section}
\newcounter {subsection}[section]
\newcounter {subsubsection}[subsection]
\newcounter {paragraph}[subsubsection]
\newcounter {subparagraph}[paragraph]
\renewcommand\thepart         {\@Roman\c@part}
\renewcommand\thesection      {\@arabic\c@section}
\renewcommand\thesubsection   {\thesection.\@arabic\c@subsection}
\renewcommand\thesubsubsection{\thesubsection.\@arabic\c@subsubsection}
\renewcommand\theparagraph    {\thesubsubsection.\@arabic\c@paragraph}
\renewcommand\thesubparagraph {\theparagraph.\@arabic\c@subparagraph}
%%%%%%%%%%%%%%%%%%%%%%%%%%% SECTION FORMATS %%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\secstyle{\bfseries}
\def\ts@flag{\let\d@t.%					% Sections get ``.''
	     \immediate\write\@auxout			% IF THERE IS A SECTION
	     {\string\global\string\@todotoctrue}}	% THEN SIGNAL IN AUX.

\newcommand\part{\par
   \addvspace{4ex}%
   \@afterindentfalse
   \secdef\@part\@spart}

\def\@part[#1]#2{\ts@flag
    \ifnum \c@secnumdepth >\m@ne
      \refstepcounter{part}%			% DAMN LATEX !!! BELOW,
      \addcontentsline{toc}{part}{\string\href	% UNFORTUNATELY, NO NUMBERLINE:
				  {\string\hash\space part\the\c@part}%
				  {\thepart}\hspace{1em}#1}%
    \else
      \addcontentsline{toc}{part}{#1}%
    \fi
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \ifnum \c@secnumdepth >\m@ne
       \name{part\the\c@part}\Large\bfseries \partname~\thepart
       \par\nobreak
     \fi
     \huge \bfseries #2%
     \markboth{}{}\par}%
    \nobreak
    \vskip 3ex
    \@afterheading\let\d@t\relax}
\def\@spart#1{%
    {\parindent \z@ \raggedright
     \interlinepenalty \@M
     \normalfont
     \huge \bfseries #1\par}%
     \nobreak
     \vskip 3ex
     \@afterheading}

\newcommand\section{\@startsection{section}{1}{\z@}%
                                   {-3.5ex \@plus -1.3ex \@minus -.7ex}%
                                   {2.3ex \@plus.4ex \@minus .4ex}%
                                   {\normalfont\large\secstyle}}
\newcommand\subsection{\@startsection{subsection}{2}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1.2ex \@plus .3ex \@minus .3ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\subsubsection{\@startsection{subsubsection}{3}{\z@}%
                                   {-2.3ex\@plus -1ex \@minus -.5ex}%
                                   {1ex \@plus .2ex \@minus .2ex}%
                                   {\normalfont\normalsize\secstyle}}
\newcommand\paragraph{\@startsection{paragraph}{4}{\z@}%
                                   {1.75ex \@plus1ex \@minus.2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}
\newcommand\subparagraph{\@startsection{subparagraph}{5}{\parindent}%
                                   {1.75ex \@plus1ex \@minus .2ex}%
                                   {-1em}%
                                   {\normalfont\normalsize\bfseries}}

% ---- turnaround for sections with figures ------ %
\def\bef@sec{\iffigprocessing\JHEP@warnl{Floating figure \the\ffigcount\space
						and startsection colliding}\fi
	     \iftabprocessing\JHEP@warnl{Floating table \the\ftabcount\space
						and startsection colliding}\fi
	     \edef\bef@everypar{\the\everypar}}	% HACK FOR FLOATS AND \everypar
\def\aft@sec{\let\d@t\relax			% RESTORE: NO DOTTED SUBSECS..
	     \edef\tmp@everypar{\the\everypar}% % DELETED CLUBPENALTY, BELOW.
	     \everypar\expandafter{\bef@everypar{\tmp@everypar}}}% RESTORE.
\let\old@sec\section				%
\let\old@ssec\subsection			%
\let\old@sssec\subsubsection			% OLD SECTIONING COMMANDS.
\let\old@par\paragraph				%
\let\old@spar\subparagraph			%
% ------- new forms ------- %
\renewcommand{\section}{\secdef\JHEP@sec\JHEP@secs}
\renewcommand{\subsection}{\secdef\JHEP@ssec\JHEP@ssecs}
\renewcommand{\subsubsection}{\secdef\JHEP@sssec\JHEP@sssecs}
\renewcommand{\paragraph}{\secdef\JHEP@par\JHEP@pars}
\renewcommand{\subparagraph}{\secdef\JHEP@spar\JHEP@spars}
% ---- unstarred forms ---- %
\def\JHEP@sec[#1]#2{\ts@flag\bef@sec\old@sec[#1]{#2}\aft@sec}
\def\JHEP@ssec[#1]#2{\bef@sec\old@ssec[#1]{#2}\aft@sec}
\def\JHEP@sssec[#1]#2{\bef@sec\old@sssec[#1]{#2}\aft@sec}
\def\JHEP@par[#1]#2{\bef@sec\old@par[#1]{#2}\aft@sec}
\def\JHEP@spar[#1]#2{\bef@sec\old@spar[#1]{#2}\aft@sec}
% ----- starred forms ----- %
\def\JHEP@secs#1{\bef@sec\old@sec*{#1}\aft@sec}
\def\JHEP@ssecs#1{\bef@sec\old@ssec*{#1}\aft@sec}
\def\JHEP@sssecs#1{\bef@sec\old@sssec*{#1}\aft@sec}
\def\JHEP@pars#1{\bef@sec\old@par*{#1}\aft@sec}
\def\JHEP@spars#1{\bef@sec\old@spar*{#1}\aft@sec}
% ----- end hack for sections with floats --------%

\if@twocolumn
  \setlength\leftmargini  {2em}
\else
  \setlength\leftmargini  {2.5em}
\fi
\leftmargin  \leftmargini
\setlength\leftmarginii  {2.2em}
\setlength\leftmarginiii {1.87em}
\setlength\leftmarginiv  {1.7em}
  \setlength\leftmarginv  {1em}
  \setlength\leftmarginvi {1em}
\setlength  \labelsep  {.5em}
\setlength  \labelwidth{\leftmargini}
\addtolength\labelwidth{-\labelsep}
\@beginparpenalty -\@lowpenalty
\@endparpenalty   -\@lowpenalty
\@itempenalty     -\@lowpenalty
\renewcommand\theenumi{\@arabic\c@enumi}
\renewcommand\theenumii{\@alph\c@enumii}
\renewcommand\theenumiii{\@roman\c@enumiii}
\renewcommand\theenumiv{\@Alph\c@enumiv}
\newcommand\labelenumi{\theenumi.}
\newcommand\labelenumii{(\theenumii)}
\newcommand\labelenumiii{\theenumiii.}
\newcommand\labelenumiv{\theenumiv.}
\renewcommand\p@enumii{\theenumi}
\renewcommand\p@enumiii{\theenumi(\theenumii)}
\renewcommand\p@enumiv{\p@enumiii\theenumiii}
\newcommand\labelitemi{$\m@th\bullet$}
\newcommand\labelitemii{\normalfont\bfseries --}
\newcommand\labelitemiii{$\m@th\ast$}
\newcommand\labelitemiv{$\m@th\cdot$}
\newenvironment{description}
               {\list{}{\labelwidth\z@ \itemindent-\leftmargin
                        \let\makelabel\descriptionlabel}}
               {\endlist}
\newcommand*\descriptionlabel[1]{\hspace\labelsep
                                \normalfont\bfseries #1}
%%%%%%%%%%%%%%%%%%%%%%%%%% AUTHORS/ADDRESSES %%%%%%%%%%%%%%%%%%%%%%%%%%
% *** After proceedings, the authors go in a hbox. => \break does not work!!
% *** if no address nobody closes the box!
\newif\if@speaker\@speakerfalse
\newif\if@dblspeak\@dblspeakfalse
\newtoks\prev@t
\newtoks\cur@t
\newbox\@firstaubox
\newskip\addr@skip\addr@skip=\if@proc .6em\@plus.02em\@minus.3ex
			     \else .6em\@plus.02fil\@minus.3ex \fi
\newskip\auth@skip\auth@skip=\if@proc .6em\@plus.03em\@minus.2ex
			     \else .6em\@plus.03fil\@minus.2ex \fi
\renewcommand\@author{\parskip\z@
%		      \def\@noaddr{\setbox\@tmpbox\vbox\bgroup\let\\\par}%
		      \def\\{\egroup			% CLOSE & aftergroup!
			\par				% FIRST TIME \\=>ADDR.
			\vskip\addr@skip		% GLUE UNDER AUTHOR
			\hskip1em%			% ADDRESS INDENT
			\vbox\bgroup\hsize=.9\textwidth	% 
			\small\it\raggedright		% STYLE FOR ADDRESSES
			\def\\{\par\leavevmode\ignorespaces}%\let\\\relax%
			\leavevmode\ignorespaces}%
			}
\renewcommand\author[1]{%
		\global\@authortrue			%
		\prev@t=\expandafter{\@author}%		% TWO TOKEN LISTS.
		\cur@t={\vskip\auth@skip		% glue before auth.
			\vtop\bgroup #1\egroup		% ACTUAL AUTH.\\ADD.
			\par}%				%
		\long\xdef\@author{\the\prev@t\the\cur@t}%STORE ALL IN \@AUTHOR
		}
%%%%%%%%%%%%%%%%%%%%%%%%%%%% SPEAKER %%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\speaker[1]{\if@speaker\global\@dblspeaktrue\fi
			\global\@speakertrue
			\global\setbox\@firstaubox
			\hbox{\let\thanks\@gobble
				\let\footnote\@gobble 
				\rm #1}%
			#1\thanks{Speaker.}\
			}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CONFERENCE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\conf@box
\newcommand\conference[1]{\global\setbox\conf@box\hbox{%
			 \itshape #1}\@conftrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% RECEIVED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\received[1]{\gdef\Jrece@cs{{\scshape\receivedname} 
                                       {\itshape #1}}\@recetrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% REVISED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\revised[1]{\gdef\Jrevi@cs{{\scshape\revisedname}
                                      {\itshape #1}}\@revitrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PUBLISHED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\accepted[1]{\gdef\Jacce@cs{{\scshape\acceptedname}
                                       {\itshape #1}}\@accetrue}
%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT DATE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newbox\Jcopy@date
\newcommand\JHEPcopydate[1]{\global\setbox\Jcopy@date
                        \hbox{\scriptsize #1}\global\@Jcopytrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEDICATED %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\dedic@box{\relax}
\newcommand\dedicated[1]{\gdef\dedic@box{\vskip2em minus 1.2ex
                              \vbox{\small\it\raggedleft #1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%% ACKNOWELEDGMENTS %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\acknowledgments{\section*{\acknowlname}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% EMAIL %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\email[1]{{\tt\href{mailto:#1}{#1}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% PREPRINT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\let\@preprint\relax
\newcommand\preprint[1]{\long\gdef\@preprint{#1}} 
%%%%%%%%%%%%%%%%% SPECIAL URL overrides paper@url %%%%%%%%%%%%%%%%%%%%%
\newbox\Jspecial@url
\newcommand\JHEPspecialurl[1]{\global\setbox\Jspecial@url\hbox{\tiny\ttfamily
			#1}\@Jspecialurltrue}
%%%%%%%%%%%%%%%%%%%%%%%%% FILE NAME AND URL %%%%%%%%%%%%%%%%%%%%%%%%%%%
\global\newbox\Jacce@month
\global\newcount\Jacce@year
\global\newbox\Jacce@number
\def\Jsplit@ident#1(#2)#3.{\global\setbox\Jacce@month\hbox{\tiny\ttfamily #1}
			  \global\Jacce@year= #2
			  \global\setbox\Jacce@number\hbox{\tiny\ttfamily #3}

\newbox\Jpaper@url
\gdef\Jfile@name{\hbox{\tiny\ttfamily
		jhep\unhcopy\Jacce@month\the\Jacce@year\unhcopy\Jacce@number}}

\global\setbox\Jpaper@url\hbox{\tiny\ttfamily 
		http://jhep.sissa.it/archive/papers/\Jfile@name/\Jfile@name.pdf}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% COPYRIGHT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\gdef\Jcopyright@box{\hbox{\if@preprint\else{\scriptsize $\copyright$
		SISSA/ISAS\ \if@Jcopy\unhbox\Jcopy@date\else\the\year\fi}\fi}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% ABSTRACT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% *** For beton! We need a cs, not a box. Maybe also for refs.. %%%%%%

\newcommand{\abstract}[1]%		% ABSTR. IN NORMALSIZE
	{\gdef\abstract@cs{		% cs FOR WHOLE ABSTRACT
	{\if@proc\small\else\fi
	\noindent{\scshape\abstractname}\ \ignorespaces #1}}
	\normalsize
	\global\@abstracttrue}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% KEYWORDS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@keywords{\relax}%                   % CS FOR WHOLE KEYWORDS
\def\keywords{\bgroup\gdef\@comma{,}\catcode`\ =\active\catcode`,=\active
		\@@keywords}
\begingroup
\catcode`\ =\active\catcode`,=\active\global
\def\@@keywords#1{\gdef\@keywords{\noindent{\scshape\keywordsname}
		\bgroup\def, {+}\def {_}%	%ATTENTION: NO EXPANSION.
		\href{http://jhep.sissa.it/stdsearch?keywords=#1}%
						{\let,\@comma\let \ #1}.
		\egroup}\egroup\global\@keywordstrue}%
\endgroup
%%%%%%%%%%%%%%%%%%%%%%%%%% OTHER ENVIRONMENTS %%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{verse}
               {\let\\\@centercr
                \list{}{\itemsep      \z@
                        \itemindent   -1.5em%
                        \listparindent\itemindent
                        \rightmargin  \leftmargin
                        \advance\leftmargin 1.5em}%
                \item\relax}
               {\endlist}
\newenvironment{quotation}
               {\list{}{\listparindent 1.5em%
                        \itemindent    \listparindent
                        \rightmargin   \leftmargin
                        \parsep        \z@ \@plus\p@}%
                \item\relax}
               {\endlist}
\newenvironment{quote}
               {\list{}{\rightmargin\leftmargin}%
                \item\relax}
               {\endlist}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THEOREMS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newif\if@twothms\@twothmsfalse

\if@preprint%\ifx\@thmcountersep\@undefined
%\def\@xthm#1#2{\@begintheorem{#2}{\csname the#1\endcsname.}\ignorespaces}% after thm number
\else									 % if published or proc
\def\@xthm#1#2{\@begintheorem{#2\if@twothms\else.\fi}			 % theorems are numbered
		{\if@twothms\csname the#1\endcsname.\fi}		 % only if more than one
		\ifnum \csname the#1\endcsname>1 \immediate\write\@auxout% and not within sections
				{\string\global\string\@twothmstrue}\fi
		\ignorespaces}
\fi

\newcommand\Proof{\noindent\emph{Proof.}\ }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% APPENDIX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\appendix{\par
  \setcounter{section}{0}%
  \setcounter{subsection}{0}%
  \renewcommand\thesection{\@Alph\c@section}}

%%%%%%%%%%%%%%%%%%%%%%%%%%% SOME MORE LENGHTS %%%%%%%%%%%%%%%%%%%%%%%%%
\setlength\arraycolsep{2\p@}		% TO MATCH eqnarrays<->equations
\setlength\tabcolsep{6\p@}
\setlength\arrayrulewidth{.4\p@}
\setlength\doublerulesep{2\p@}
\setlength\tabbingsep{\labelsep}
\skip\@mpfootins = \skip\footins
\setlength\fboxsep{3\p@}
\setlength\fboxrule{.4\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% THE EQUATION %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\theequation{\ifnum\c@section=0\else\thesection.\fi
			  \@arabic\c@equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIGURES, TABLES %%%%%%%%%%%%%%%%%%%%%%%%%%
\newcounter{figure}
\renewcommand\thefigure{\@arabic\c@figure}
\def\fps@figure{Htbp}
\def\ftype@figure{1}
\def\ext@figure{lof}
\def\fnum@figure{\figurename~\thefigure}
\newenvironment{figure}
               {\@ENVwarn{\FIGURE{...}}\@float{figure}}
               {\end@float}
\newenvironment{figure*}
               {\@ENVwarn{\FIGURE{...}}\@dblfloat{figure}}
               {\end@dblfloat}
\newcounter{table}
\renewcommand\thetable{\@arabic\c@table}
\def\fps@table{tbp}
\def\ftype@table{2}
\def\ext@table{lot}
\def\fnum@table{\tablename~\thetable}
\newenvironment{table}
               {\@ENVwarn{\TABLE{...}}\@float{table}}
               {\end@float}
\newenvironment{table*}
               {\@ENVwarn{\TABLE{...}}\@dblfloat{table}}
               {\end@dblfloat}
%%-----------------------------------------------------------------%%
\newcommand{\FIGURE}[2][v]{\begin{floatingfigure}[#1]#2
                                        \end{floatingfigure}}
\newcommand{\TABLE}[2][v]{\begin{floatingtable}[#1]{#2}
                                        \end{floatingtable}}
\newcommand{\EPSFIGURE}[3][v]{\begin{floatingfigure}[#1]\epsfig{file=#2}
                                        \caption{#3}\end{floatingfigure}}
\newcommand{\TABULAR}[4][v]{\begin{floatingtable}[#1]{\begin{tabular}{#2}
					#3\end{tabular}}\caption{#4}
                                        \end{floatingtable}}
%Check below, and put automatic width ***
\newcommand{\DOUBLEFIGURE}[5][ht]{\@dblfloat{figure}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#2}}}~~~~
		\parbox{.45\textwidth}{\centerline{\epsfig{file=#3}}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
\newcommand{\DOUBLETABLE}[5][ht]{\@dblfloat{table}[#1]\centerline{%
		\parbox{.45\textwidth}{\centerline{#2}}~~~~
		\parbox{.45\textwidth}{\centerline{#3}}}
		\centerline{\parbox[t]{.45\textwidth}{\caption{#4}}~~~~
		\parbox[t]{.45\textwidth}{\caption{#5}}}\end@dblfloat}
%%%%%%---------------- FROM FLOATFLT PACKAGE ------------------%%%%%%%%
%% Original file `floatflt.sty', modified by F.Nesti <nesti@sissa.it> to:
%% be inserted in JHEP.cls;
%% correct float placement when shifting past pages;
%% correct incompatibility with \marginpar;
%% correct incompatibility with \@startsection;
%% correct persisting indentation in following pars;
%% let float also at beginning of pages; 
%% avoid the widht specification.
%% 
%% Original was 1994-1996 by Mats Dahlgren <matsd@physchem.kth.se>. 
%% 
%%%%%%%%\NeedsTeXFormat{LaTeX2e}[1994/06/01]		%LEFT THIS STUFF TO 
%%%%%%%%\ProvidesPackage{floatflt}[1996/02/27 v. 1.3]	%RECONVERT TO PACKAGE.
\newcounter{OptionTest}
\if@twoside
 \setcounter{OptionTest}{0}
\else							% POS: 2side=p/1side=r
 \setcounter{OptionTest}{1}
\fi
%%%%%%%%\DeclareOption{rflt}{\setcounter{OptionTest}{1}}
%%%%%%%%\DeclareOption{lflt}{\setcounter{OptionTest}{2}} % CHOSEN.
%%%%%%%%\DeclareOption{vflt}{\setcounter{OptionTest}{0}}
%%%%%%%%\DeclareOption*{\OptionNotUsed}
%%%%%%%%\ProcessOptions
\newbox\@tmpbox
\newbox\figbox
\newbox\tabbox
\newbox\pagebox
\newcount\ffigcount
\newcount\ftabcount
\newcount\hangcount
\newcount\nosuccesstryfig
\newcount\nosuccesstrytab
\newdimen\figgutter   \figgutter=1truepc
\newdimen\tabgutter   \tabgutter=1truepc
\newdimen\fl@wd
\newdimen\fl@ht
%\newdimen\fl@gut
\newdimen\htdone      \htdone=\z@
\newdimen\pageht
\newdimen\startpageht
\newdimen\floatfltwidth
\newdimen\fltitemwidth
\newif\iftryingfig     \tryingfigfalse
\newif\iftryingtab     \tryingtabfalse
\newif\ifdoingfig      \doingfigfalse
\newif\ifdoingtab      \doingtabfalse
\newif\iffigprocessing \figprocessingfalse
\newif\iftabprocessing \tabprocessingfalse
\newif\ifpageafterfig  \pageafterfigfalse
\newif\ifpageaftertab  \pageaftertabfalse
\newif\ifoddpages
\newif\ifoutput
\newtoks\outputpretest
\def\@captype{}
%%---------------- ORRIBLE HACKS, SORRY -------------------------%%
\let\old@marginpar\marginpar				% 
\renewcommand\marginpar[1]{{\outputpretest={\outputtrue}% REDEF \marginpar.
			    \old@marginpar{#1}}}	%
\def\g@addto#1#2{{\toks@\expandafter{#1#2}%
		  \xdef#1{\the\toks@}}}%
\def\postpone@captions{%			%
%	\global\let\tmp@label\label		% REDEF \caption AND 
	\global\let\tmp@caption\caption		% \label, LATER.
	\global\let\later@capt\relax		% UN PO' PESANTI 
	\gdef\later@label{}%			% MA D'ALTRONDE...
	\let\J@ref\ref\def\ref{\protect\J@ref}% % protect ref in captions.. 
	\renewcommand\caption{\@ifnextchar[\J@@caption\J@caption}%
	\newcommand\J@caption[1]{\gdef\later@capt{\tmp@caption{##1}}}% LOCAL!!
	\newcommand\J@@caption[2][v]%
				{\gdef\later@capt{\tmp@caption[##1]{##2}}}% LOCAL!!
	\renewcommand\@@label[1]{\egroup\name{ref-##1}%	% TAG WHERE CALLED, AT LEAST,
			       \if@draft\norm@note{}{LAB: ##1}\fi% & DRAFTNOTE.
			       \g@addto\later@label{\old@label{##1}}}%
			}
\AtEndDocument{\iftryingfig\JHEP@warnl{Floating figure \the\ffigcount\space
					remains undone}\fi
		\iftryingtab\JHEP@warnl{Floating table \the\ftabcount\space
					remains undone}\fi
		\if@JHEP\ifnum\Jacce@year>2001\if@Jcopy\else
		\ifnum\the\Jacce@year=\the\year\else
		\JHEP@warnl{The acceptance date
		\the\Jacce@year\space is different from today's
		\the\year}\fi\fi\fi\fi} % the copyright date must be that
			  %  of publication if it differs from the one in the
		 	  % identifier it can be forced using command \JHEPcopydate
%%----------------- FIGURE ---------------------------------------%%
\newenvironment{floatingfigure}[1][v]%
{\@tfor \@tempa :=#1\do {\xdef\@fside{\@tempa}}%
 \global\advance\ffigcount by 1%
 \iffigprocessing {\count0=\ffigcount\advance\count0 by -1%
   		   \JHEP@warnl{Floating figures \the\count0\space\space and
       			\the\ffigcount\space colliding}}\fi
 \iftabprocessing  \JHEP@warnl{Floating table \the\ftabcount\space and 
			floating figure \the\ffigcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of figbox %HBOX FOR AUTO WIDTH!
}
{%
\egroup%				% CALCULATE WIDTH (NO CAPTION FOR NOW)
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
% New behavior:	wd < .6 columnwidth => floatflt.
%		wd < columnwidth    => float{figure}
%		wd > columnwidth    => dblfloat{figure}
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
 \global\setbox\figbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{figure}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
 \global\figprocessingtrue
 \global\everypar={\tryfig\oldeverypar}% must be set globally!
 \figinsert\par
\else%					% ELSE NORMAL LATEX FIGURE, SIGH.
% \JHEP@mess{Floating figure \the\ffigcount\space is 
%			wide becomes a LaTeX float}%
 \if\@fside v \def\@fside{ht}\fi
 \ifdim\floatfltwidth<\columnwidth
    \def\@@tempa{\@float{figure}[}\let\@@tempb\end@float
 \else
    \def\@@tempa{\@dblfloat{figure}[}\let\@@tempb\end@dblfloat
 \fi
 \expandafter\@@tempa\@fside]\center\unhbox\@tmpbox\later@capt\later@label\@@tempb
\fi
}
%%------------ TABLE ----------------------------------------------%%
\newenvironment{floatingtable}[1][v]%
{\@tfor \@tempa :=#1\do {\global\edef\@tside{\@tempa}}%
 \global\advance\ftabcount by 1%
 \iftabprocessing {\count0=\ftabcount\advance\count0 by -1%
     		   \JHEP@warnl{Floating tables \the\count0\space
            		\space and \the\ftabcount \space colliding}}\fi
 \iffigprocessing  \JHEP@warnl{Floating figure \the\ffigcount\space and 
			floating table \the\ftabcount\space colliding}\fi
 \postpone@captions
 \global\setbox\@tmpbox=\hbox\bgroup% begin of tabbox, ACTUALLY AN HBOX.
}
{%
\egroup% end of \tabbox, 		% ACTUALLY \@tmpbox
\global\setlength{\floatfltwidth}{\the\wd\@tmpbox}%
\ifdim\floatfltwidth<.6\columnwidth%	% IF NOT TOO WIDE OK:
  \global\setbox\tabbox=\vbox{\hsize=\floatfltwidth
			     \def\@captype{table}%
			     \noindent\unhbox\@tmpbox
			     \later@capt\later@label}%
  \global\tabprocessingtrue
  \global\everypar={\trytab\oldeverypar}%
  \tabinsert\par%
\else%					% ELSE NORMAL LATEX TABLE.
%  \JHEP@mess{Floating table \the\ftabcount\space is 
%			wide becomes a LaTeX float}%
  \ifdim\floatfltwidth<1.1\columnwidth
    \if\@tside v \def\@tside{ht}\fi
    \def\@@tempa{\@float{table}[}\let\@@tempb\end@float
  \else
    \if\@tside v \def\@tside{t}\fi
    \def\@@tempa{\@dblfloat{table}[}\let\@@tempb\end@dblfloat
  \fi
  \expandafter\@@tempa\@tside]%		% ACTUALLY CALL THE LATEX FLOAT
  \center\unhbox\@tmpbox\later@capt\later@label
  \@@tempb
\fi%
}
%----------- prepare for tries ----------------------------%
\def\figinsert{%
   \global\nosuccesstryfig=0%
   \global\outputpretest={\do@test}%
   \global\tryingfigtrue \global\doingfigfalse%
   \global\pageafterfigfalse}%
\def\tabinsert{%
   \global\nosuccesstrytab=0%
   \global\outputpretest={\do@test}%
   \global\tryingtabtrue \global\doingtabfalse%
   \global\pageaftertabfalse}%
%----------- init -----------------------------------------%
\AtBeginDocument{%
 \edef\oldoutput{\the\output}
 \output={\the\outputpretest\ifoutput\oldoutput\fi}%
 \outputpretest={\outputtrue}%
 \edef\oldeverypar{\the\everypar}% PERCHE' NESSUNO LO RIMETTE PIU' A POSTO?***
}
%---- tests during \outputpretest -------------------------%
\def\do@test{%
   \ifnum\outputpenalty=-10005
%	\output
     \setbox\pagebox=\vbox{\unvbox255}%
     \global\pageht=\ht\pagebox
     \global\outputfalse
     \unvbox\pagebox
     \dimen0=\pageht\advance\dimen0 by 2 \baselineskip
     \ifdim\dimen0>\vsize\pagebreak[4]\global\pageht\z@\fi
   \else
     \global\outputtrue
     \ifnum\outputpenalty>-\@Mi			%ie \marginpar's give penalty.
	\ifdoingtab\global\pageaftertabtrue\fi
	\ifdoingfig\global\pageafterfigtrue\fi
     \fi
   \fi}%
%-------- check for side ----------------------------------%
\def\chk@side#1{% DEFINED \fl@sid, BUT IF CHOSEN A DEFAULT, ELIMINATE ALL ***
	{\edef\fl@sid{#1}%
	  \if\fl@sid r\global\oddpagestrue\fi
          \if\fl@sid l\global\oddpagesfalse\fi
          \if\fl@sid p%
              \ifodd\c@page\global\oddpagesfalse
                \else\global\oddpagestrue\fi
          \fi
          \if\fl@sid v%
             \ifnum\theOptionTest=0%
                 \ifodd\c@page\global\oddpagesfalse
                   \else\global\oddpagestrue\fi
             \else
                  \ifodd\theOptionTest\global\oddpagestrue
                    \else\global\oddpagesfalse\fi
             \fi
          \fi
         }}%
%-------- get point in page -------------------------------%
\def\get@pageht{{\everypar={\relax}\setbox0=\lastbox
       		\parindent=\wd0 \parskip=\z@ \par
         	\penalty-10005 \leavevmode}}%
%-------- try at everypar ---------------------------------%
\def\tryfig{%
	\global\fl@ht\ht\figbox
	\global\fl@wd\wd\figbox
	\global\let\fl@gut\figgutter
      \iftryingfig
	\get@pageht
	\dimen0=\vsize
	\advance\dimen0 by -\pageht
	\advance\dimen0 by -2\baselineskip
	\ifdim\dimen0>\fl@ht
	  \chk@side\@fside
	  \dimen0=0.3\baselineskip
	  \vrule depth \dimen0 width \z@%height 1.5\baselineskip
	  \vadjust{\kern -\dimen0
	  \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\figbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\figbox\hss}%
             \fi
             \vss}\null}}%
	  \global\tryingfigfalse
	  \global\doingfigtrue
	  \global\startpageht=\pageht
	  \global\htdone=\z@
	  \dohang
	  \ifnum\nosuccesstryfig>0%
	   \JHEP@mess{Flt. fig. \the\ffigcount\space set on page \the\count0, 
	 		shifted \the\nosuccesstryfig\space par(s) forward}%
%	  \else
%	   \JHEP@mess{Floating figure \the\ffigcount\space 
%			set on page \the\count0}%
	  \fi
	\else
          \global\advance\nosuccesstryfig by 1
	\fi
      \else%				% IF NOT TRYING
	\ifdoingfig
	  \get@pageht
	  \global\htdone=\pageht
	  \global\advance\htdone by -\startpageht
	  \ifpageafterfig
	    \global\doingfigfalse% IN CASE A PAGEBREAK JUST BELOW?
	  \else
	    \dimen0=\fl@ht
	    \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
%	    \typeout{FLOAT HT: \the\dimen0, HTDONE: \the\htdone}
	    \ifdim\htdone<\dimen0%
		\dohang
	    \else
		\global\doingfigfalse
	    \fi
	  \fi
	  \ifdoingfig\else\global\figprocessingfalse\fi% IF NO MORE DOING.
	\else
	  \global\outputpretest={\outputtrue}% NOT RESTORE EVPAR IF NOT DOING?
	\fi%			% END IF DOING
      \fi%			% END IF TRYING
}
\def\trytab{%
	\global\fl@ht\ht\tabbox
	\global\fl@wd\wd\tabbox
	\global\let\fl@gut\tabgutter
       \iftryingtab
	\get@pageht
       \dimen0=\vsize
       \advance\dimen0 by -\pageht
       \advance\dimen0 by -2\baselineskip
       \ifdim\dimen0>\fl@ht
	 \chk@side\@tside
         \dimen0=0.3\baselineskip
         \vrule depth \dimen0 width \z@
         \vadjust{\kern -\dimen0
         \vtop to \dimen0{%
             \baselineskip=\dimen0
             \vss \vbox to 1ex{%
             \ifoddpages
               \hb@xt@\hsize{\hss\copy\tabbox}%
             \else% leftsetting
               \hb@xt@\hsize{\copy\tabbox\hss}%
             \fi
             \vss}\null}}%
       \global\tryingtabfalse
       \global\doingtabtrue
       \global\startpageht=\pageht
       \global\htdone=\z@
       \dohang
       \ifnum\nosuccesstrytab>0%
	\JHEP@mess{Flt. tab. \the\ftabcount\space set on page \the\count0, 
			shifted \the\nosuccesstrytab\space par(s) forward}%
%       \else
%	\JHEP@mess{Floating table \the\ftabcount\space 
%			set on page \the\count0}%
       \fi
     \else
       \global\advance\nosuccesstrytab by 1
     \fi
     \else
     \ifdoingtab
       \get@pageht
    \global\htdone=\pageht
    \global\advance\htdone by -\startpageht
    \ifpageaftertab
      \global\doingtabfalse
    \else
      \dimen0=\fl@ht
      \advance\dimen0 by .85\baselineskip	% .85 ENOUGH: WE ARE AT NEW PAR
      \ifdim\htdone<\dimen0%
         \dohang
      \else
         \global\doingtabfalse
      \fi
    \fi
    \ifdoingtab\relax\else\global\tabprocessingfalse\fi
  \else
    \global\outputpretest={\outputtrue}%
  \fi
\fi
}
%----- hanging lord -----------------------------%
\def\dohang{%
   \dimen0=\fl@ht
   \advance\dimen0 by -\htdone
   \advance\dimen0 by 1.999\baselineskip	% (16/12/98) WAS 1.49 BUT
   \hangcount=\dimen0				% TEX ROUNDS ON STRICT INTEGERS
   \divide\hangcount by \baselineskip		% IN THIS DIVISION!
%	\typeout{HANGCOUNT: \the\hangcount.}
%   \ifnum\hangcount > 0	% IF ZERO ALSO INDENT MUST BE NULL. (7/6/97)
     \dimen0=\fl@wd
     \advance\dimen0 by \fl@gut
     \ifoddpages
       \global\hangindent=-\dimen0% placing right
     \else 
       \global\hangindent=\dimen0% placing left
     \fi
   \global\hangafter=-\hangcount
%   \fi
}
%----------------------- TWO NEWITEMS ---------------------%
\newcommand{\fltitem}[2][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item \parbox[t]{\fltitemwidth}{#2}\\[#1]}
\newcommand{\fltditem}[3][\z@]{\setlength{\fltitemwidth}{\linewidth}%
  \addtolength{\fltitemwidth}{-\floatfltwidth}%
  \addtolength{\fltitemwidth}{-0.5em}%
  \item[#2] \parbox[t]{\fltitemwidth}{#3}\\[#1]}
%%%%%%\endinput
%% 
%% End of ex-file `floatflt.sty'.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% CAPTIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newlength\abovecaptionskip
\newlength\belowcaptionskip
\setlength\abovecaptionskip{8\p@}
\setlength\belowcaptionskip{0\p@}
\long\def\@makecaption#1#2{%
  \if@hyper{\edef\@pippo{the\@captype}
	    \name{\@captype\expandafter\csname\@pippo\endcsname}}\fi%
  \vskip\abovecaptionskip
 {\let\label\@gobble%				% FN 10.2.97 REMOVED LATEX BUG:
  \let\index\@gobble%				% LARGE CAPTIONS PROCESS LABEL
  \let\glossary\@gobble%			% TWO TIMES.
  \sbox\@tempboxa{\small {\bfseries #1:} #2}%	% 
  \global\dimen0\wd\@tempboxa}%			%
  \ifdim \dimen0 >\hsize
    \small {\bfseries #1:} #2\par
  \else
    \global\@minipagefalse \sbox\@tempboxa{\small {\bfseries #1:} #2}%
    \hb@xt@\hsize{\hfil\box\@tempboxa\hfil}%
  \fi
  \vskip\belowcaptionskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FONTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\DeclareOldFontCommand{\rm}{\normalfont\rmfamily}{\mathrm}
\DeclareOldFontCommand{\sf}{\normalfont\sffamily}{\mathsf}
\DeclareOldFontCommand{\tt}{\normalfont\ttfamily}{\mathtt}
\DeclareOldFontCommand{\bf}{\normalfont\bfseries}{\mathbf}
\DeclareOldFontCommand{\it}{\normalfont\itshape}{\mathit}
\DeclareOldFontCommand{\sl}{\normalfont\slshape}{\@nomath\sl}
\DeclareOldFontCommand{\sc}{\normalfont\scshape}{\@nomath\sc}
\DeclareRobustCommand*\cal{\@fontswitch\relax\mathcal}
\DeclareRobustCommand*\mit{\@fontswitch\relax\mathnormal}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% TOC %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\tocsecs{}
\newcommand\@pnumwidth{1.55em}
\newcommand\@tocrmarg{2.55em}
\newcommand\@dotsep{4.5}
\setcounter{tocdepth}{3}
\newcommand\tableofcontents{%
    \section*{\contentsname\label{-TOC-}}
%        \@mkboth{%
%           \MakeUppercase\contentsname}{\MakeUppercase\contentsname}%
    \@starttoc{toc}%
    \gdef\tableofcontents{\JHEP@igno{\tableofcontents\space already done}}}
\newcommand*\l@part[2]{\def\hyp@typ{part}%	
  \ifnum \c@tocdepth >-2\relax
    \addpenalty\@secpenalty
    \addvspace{2.25em \@plus\p@}%
    \begingroup
      \setlength\@tempdima{3em}%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      {\leavevmode
       \large \bfseries \tocsecs#1\hfil \hb@xt@\@pnumwidth{\hss
		\href{\hash pag#2}{#2}}}\par
       \nobreak
       \if@compatibility
         \global\@nobreaktrue
         \everypar{\global\@nobreakfalse\everypar{}}%
      \fi
    \endgroup
  \fi}
\newcommand*\l@section[2]{\def\hyp@typ{sec}%
  \ifnum \c@tocdepth >\z@
    \addpenalty\@secpenalty
    \addvspace{1.0em \@plus\p@}%
    \setlength\@tempdima{1.8em}%	%WIDTH OF SECT. N.
    \begingroup
      \let\d@t.%
      \parindent \z@ \rightskip \@pnumwidth
      \parfillskip -\@pnumwidth
      \leavevmode \bfseries
      \advance\leftskip\@tempdima
      \hskip -\leftskip
        \tocsecs#1\nobreak\hfil %HREF HERE WOULD GET ALSO THE TITLE(...)
        \nobreak\hb@xt@\@pnumwidth{\hss \href{\hash pag#2}{#2}}\par
    \endgroup
  \fi}

\newcommand*\l@subsection{\def\hyp@typ{sec}\@tocline{2}{1.8em}{2.3em}}
\newcommand*\l@subsubsection{\def\hyp@typ{sec}\@tocline{3}{4.1em}{3.1em}}
\newcommand*\l@paragraph{\def\hyp@typ{sec}\@tocline{4}{7.2em}{4.3em}}
\newcommand*\l@subparagraph{\def\hyp@typ{sec}\@tocline{5}{10.5em}{5em}}

\if@hyper
  \let\old@dtl\@dottedtocline
  \def\@dottedtocline#1#2#3#4#5{\old@dtl{#1}{#2}{#3}{#4}{%
						\href{\hash pag#5}{#5}}}
\fi

\def\@tocline#1#2#3#4#5{%
  \ifnum #1>\c@tocdepth \else
    \vskip \z@ \@plus.2\p@
    {\leftskip #2\relax \rightskip \@tocrmarg \parfillskip -\rightskip
     \parindent #2\relax\@afterindenttrue
     \interlinepenalty\@M
     \leavevmode
     \@tempdima #3\relax
     \advance\leftskip \@tempdima \null\nobreak\hskip -\leftskip
     {#4}\nobreak
     %\leaders\hbox{$\m@th
     %   \mkern \@dotsep mu\hbox{.}\mkern \@dotsep
     %	   mu$}
     \hfill
     \nobreak
     \hb@xt@\@pnumwidth{\hfil\normalfont \normalcolor \href{\hash pag#5}{#5}}%
     \par}%
  \fi}


%%%%%%%%%%%%%%%%%%%%%% LIST OF FIGURES AND TABLES %%%%%%%%%%%%%%%%%%%%%
\if@draft			% ONLY IF DRAFT! ... 
 \newcommand\listoffigures{%
     \section*{\listfigurename
       \@mkboth{\MakeUppercase\listfigurename}%
               {\MakeUppercase\listfigurename}}%
     \@starttoc{lof}%
     }
 \newcommand*\l@figure{\def\hyp@typ{figure}\@dottedtocline{1}{1.5em}{2.3em}}
 \newcommand\listoftables{%
     \section*{\listtablename
       \@mkboth{%
           \MakeUppercase\listtablename}{\MakeUppercase\listtablename}}%
     \@starttoc{lot}%
     }
 \newcommand*\l@table{\def\hyp@typ{table}\@dottedtocline{1}{1.5em}{2.3em}}
\else
 \newcommand\listoffigures{\JHEP@ignol{List of figures (draft mode only)}}
 \newcommand\listoftables{\JHEP@ignol{List of tables (draft mode only)}}
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BIBLIOGRAPHY %%%%%%%%%%%%%%%%%%%%%%%%%%%%***
\newdimen\bibindent
\setlength\bibindent{1.5em}
\newenvironment{thebibliography}[1]%	%UNFORTUNATELY MODIFIED..
     {\bgroup\raggedright\small\section*{\refname
        \@mkboth{\MakeUppercase\refname}{\MakeUppercase\refname}}%
      \list{\name{bib\@arabic\c@enumiv}% HOPE!
	    \@biblabel{\@arabic\c@enumiv}}%
           {\settowidth\labelwidth{\@biblabel{#1}}%
            \leftmargin\labelwidth
            \advance\leftmargin\labelsep
            \@openbib@code
            \usecounter{enumiv}%
            \let\p@enumiv\@empty
            \renewcommand\theenumiv{\@arabic\c@enumiv}}%
      \sloppy\clubpenalty4000\widowpenalty4000%
      \sfcode`\.\@m}
     {\def\@noitemerr
       {\@latex@warning{Empty `thebibliography' environment}}%
      \endlist\egroup}
\newcommand\newblock{\hskip .11em\@plus.33em\@minus.07em}
\if@draft
 \let\old@bbt\@bibitem\let\old@lbbt\@lbibitem% LOOK THE DISASTER HERE BELOW.
 \def\@lbibitem[#1]#2{\old@lbbt[#1]{#2}\reversemarginpar{\sf\bfseries\small#2}}
 \def\@bibitem#1{\old@bbt{#1}\reversemarginpar{\sf\bfseries\small#1}}
\fi
\let\@openbib@code\@empty
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% JOURNALS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\def\@spires#1{\href{http://www-spires.slac.stanford.edu/spires/find/hep/www?j=#1}} 
%                               	%PITY THAT target IS NOT IMPLEMENTED.
\catcode`\%=12
\catcode`\|=14
\newcommand\apa[3]    {\@spires{APASA%2C#1%2C#3}
		{{\it Acta Phys.\ Austriaca }{\bf #1} (#2) #3}}
\newcommand\apas[3]    {\@spires{APAUA%2C#1%2C#3}
		{{\it Acta Phys.\ Austriaca, Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\appol[3] {\@spires{APPOA%2C#1%2C#3}
		{{\it Acta Phys.\ Polon.\ }{\bf #1} (#2) #3}}
\newcommand\advm[3]  {\@spires{ADMTA%2C#1%2C#3}
		{{\it Adv.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\adnp[3]   {\@spires{ANUPB%2C#1%2C#3}
		{{\it Adv.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\adp[3]   {\@spires{ADPHA%2C#1%2C#3}
		{{\it Adv.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\atmp[3] {\@spires{00203%2C#1%2C#3}
		{{\it Adv.\ Theor.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\am[3]    {\@spires{ANMAA%2C#1%2C#3}
		{{\it Ann.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\ap[3]    {\@spires{APNYA%2C#1%2C#3}
		{{\it Ann.\ Phys.\ (NY) }{\bf #1} (#2) #3}}
\newcommand\araa[3] {\@spires{ARAAA%2C#1%2C#3}
		{{\it Ann.\ Rev.\ Astron.\ \& Astrophys.\ }{\bf #1} (#2) #3}}
\newcommand\arnps[3] {\@spires{ARNUA%2C#1%2C#3}
		{{\it Ann.\ Rev.\ Nucl.\ Part.\ Sci.\ }{\bf #1} (#2) #3}}
\newcommand\asas[3]   {\@spires{AAEJA%2C#1%2C#3}
		{{\it Astron.\ Astrophys.\ }{\bf #1} (#2) #3}}
\newcommand\asj[3]   {\@spires{ANJOA%2C#1%2C#3}
		{{\it Astron.\ J.\ }{\bf #1} (#2) #3}}
\newcommand\app[3]   {\@spires{APHYE%2C#1%2C#3}
		{{\it Astropart.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\apj[3]    {\@spires{ASJOA%2C#1%2C#3}
		{{\it Astrophys.\ J. }{\bf #1} (#2) #3}}
\newcommand\baas[3]   {\@spires{AASBA%2C#1%2C#3}
		{{\it Bull.\ Am.\ Astron.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\bams[3]   {\@spires{BAMOA%2C#1%2C#3}
		{{\it Bull.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\blms[3]   {\@spires{LMSBB%2C#1%2C#3}
		{{\it Bull.\ London Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\cjm[3]  {\@spires{CJMAA%2C#1%2C#3}
		{{\it Can.\ J.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\cqg[3]   {\@spires{CQGRD%2C#1%2C#3}
		{{\it Class.\ and Quant.\ Grav.\ }{\bf #1} (#2) #3}}
\newcommand\cmp[3]   {\@spires{CMPHA%2C#1%2C#3}
		{{\it Commun.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ctp[3]   {\@spires{CTPMD%2C#1%2C#3}
		{{\it Commun.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\cag[3]   {\@spires{00142%2C#1%2C#3}
		{{\it Commun.\ Anal.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\cpam[3]   {\@spires{CPAMA%2C#1%2C#3}
		{{\it Commun.\ Pure Appl.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\cpc[3]   {\@spires{CPHCB%2C#1%2C#3}
		{{\it Comput.\ Phys.\ Commun.\ }{\bf #1} (#2) #3}}
\newcommand\dmj[3]   {\@spires{DUMJA%2C#1%2C#3}
		{{\it Duke Math.\ J. }{\bf #1} (#2) #3}}
\newcommand\epjc[3]  {\@spires{EPHJA%2CC#1%2C#3}
		{{\it Eur.\ Phys.\ J. }{\bf C #1} (#2) #3}}
\newcommand\epjd[3]  {\@spires{EPHJD%2CC#1%2C#3}
		{{\it Eur.\ Phys.\ J. Direct.\ }{\bf C #1} (#2) #3}}
\newcommand\epl[3]    {\@spires{EULEE%2C#1%2C#3}
		{{\it Europhys.\ Lett. }{\bf #1} (#2) #3}}
\newcommand\forp[3]    {\@spires{FPYKA%2C#1%2C#3}
		{{\it Fortschr.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\faa[3]    {\@spires{FAAPB%2C#1%2C#3}
		{{\it Funct.\ Anal.\ Appl.\ }{\bf #1} (#2) #3}}
\newcommand\grg[3]    {\@spires{GRGVA%2C#1%2C#3}
		{{\it Gen.\ Rel.\ Grav.\ }{\bf #1} (#2) #3}}
\newcommand\hpa[3]   {\@spires{HPACA%2C#1%2C#3}
		{{\it Helv.\ Phys.\ Acta }{\bf #1} (#2) #3}}
\newcommand\ijmpa[3] {\@spires{IMPAE%2CA#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\ijmpb[3] {\@spires{IMPAE%2CB#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf B #1} (#2) #3}}
\newcommand\ijmpc[3] {\@spires{IMPAE%2CC#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf C #1} (#2) #3}}
\newcommand\ijmpd[3] {\@spires{IMPAE%2CD#1%2C#3}
		{{\it Int.\ J.\ Mod.\ Phys.\ }{\bf D #1} (#2) #3}}
\newcommand\ijtp[3] {\@spires{IJTPB%2CB#1%2C#3}
		{{\it Int.\ J.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\invm[3]  {\@spires{INVMB%2C#1%2C#3}
		{{\it Invent.\ Math.\ }{\bf #1} (#2) #3}}
\newcommand\jag[3]   {\@spires{00124%2C#1%2C#3}
		{{\it J.\ Alg.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\jams[3]   {\@spires{00052%2C#1%2C#3}
		{{\it J.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\jap[3]   {\@spires{JAPIA%2C#1%2C#3}
		{{\it J.\ Appl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jdg[3]   {\@spires{JDGEA%2C#1%2C#3}
		{{\it J.\ Diff.\ Geom.\ }{\bf #1} (#2) #3}}
\newcommand\jgp[3]   {\@spires{JGPHE%2C#1%2C#3}
		{{\it J.\ Geom.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jhep[3]  {\href{http://jhep.sissa.it/stdsearch?paper=#1%28#2%29#3}
		{{\it J. High Energy Phys.\ }{\bf #1} (#2) #3}}
\newcommand\jmp[3]   {\@spires{JMAPA%2C#1%2C#3}
		{{\it J.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\joth[3]  {\@spires{JOTHE%2C#1%2C#3}
		{{\it J.\ Operator Theory }{\bf #1} (#2) #3}}
\newcommand\jpha[3]   {\@spires{JPAGB%2CA#1%2C#3}
		{{\it J. Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\jphc[3]   {\@spires{JPAGB%2CC#1%2C#3}
		{{\it J. Phys.\ }{\bf C #1} (#2) #3}}
\newcommand\jphg[3]   {\@spires{JPAGB%2CG#1%2C#3}
		{{\it J. Phys.\ }{\bf G #1} (#2) #3}}
\newcommand\lmp[3]   {\@spires{LMPHD%2CA#1%2C#3}
		{{\it Lett.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ncl[3]    {\@spires{NCLTA%2C#1%2C#3}
		{{\it Lett.\ Nuovo Cim.\ }{\bf #1} (#2) #3}}
\newcommand\matan[3]  {\@spires{MAANA%2CA#1%2C#3}
		{{\it Math.\ Ann.\ }{\bf #1} (#2) #3}}
\newcommand\mussr[3]  {\@spires{MUSIA%2CA#1%2C#3}
		{{\it Math.\ USSR Izv.\ }{\bf #1} (#2) #3}}
\newcommand\mams[3]  {\@spires{MAMCA%2CA#1%2C#3}
		{{\it Mem.\ Am.\ Math.\ Soc.\ }{\bf #1} (#2) #3}}
\newcommand\mpla[3]  {\@spires{MPLAE%2CA#1%2C#3}
		{{\it Mod.\ Phys.\ Lett.\ }{\bf A #1} (#2) #3}}
\newcommand\mplb[3]  {\@spires{MPLAE%2CB#1%2C#3}
		{{\it Mod.\ Phys.\ Lett.\ }{\bf B #1} (#2) #3}}
\newcommand\nature[3]  {\@spires{NATUA%2C#1%2C#3}
		{{\it Nature }{\bf #1} (#2) #3}}
\newcommand\nim[3]   {\@spires{NUIMA%2C#1%2C#3}
		{{\it Nucl.\ Instrum.\ Meth.\ }{\bf #1} (#2) #3}}
\newcommand\npa[3]   {\@spires{NUPHA%2CA#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf A #1} (#2) #3}}
\newcommand\npb[3]    {\@spires{NUPHA%2CB#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf B #1} (#2) #3}}
\newcommand\npps[3]  {\@spires{NUPHZ%2C#1%2C#3}
		{{\it Nucl.\ Phys.\ }{\bf #1} {\it(Proc.\ Suppl.)} (#2) #3}}
\newcommand\nc[3]    {\@spires{NUCIA%2C#1%2C#3}
		{{\it Nuovo Cim.\ }{\bf #1} (#2) #3}}
\newcommand\ncs[3]  {\@spires{NUCUA%2C#1%2C#3}
		{{\it Nuovo Cim.\ Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\pan[3]  {\@spires{PANUE%2C#1%2C#3}
		{{\it Phys.\ Atom.\ Nucl.\ }{\bf #1} (#2) #3}}
\newcommand\pla[3]   {\@spires{PHLTA%2CA#1%2C#3}
		{{\it Phys.\ Lett.\ }{\bf A #1} (#2) #3}}
\newcommand\plb[3]   {\@spires{PHLTA%2CB#1%2C#3}
		{{\it Phys.\ Lett.\ }{\bf B #1} (#2) #3}}
\newcommand\pr[3]    {\@spires{PHRVA%2C#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf #1} (#2) #3}}
\newcommand\pra[3]   {\@spires{PHRVA%2CA#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf A #1} (#2) #3}}
\newcommand\prb[3]   {\@spires{PHRVA%2CB#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf B #1} (#2) #3}}
\newcommand\prc[3]   {\@spires{PHRVA%2CC#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf C #1} (#2) #3}}
\newcommand\prd[3]   {\@spires{PHRVA%2CD#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf D #1} (#2) #3}}
\newcommand\pre[3]   {\@spires{PHRVA%2CE#1%2C#3}
		{{\it Phys.\ Rev.\ }{\bf E #1} (#2) #3}}
\newcommand\prep[3]  {\@spires{PRPLC%2C#1%2C#3}
		{{\it Phys.\ Rept.\ }{\bf #1} (#2) #3}}
\newcommand\prl[3]   {\@spires{PRLTA%2C#1%2C#3}
		{{\it Phys.\ Rev.\ Lett.\ }{\bf #1} (#2) #3}}
\newcommand\phys[3]   {\@spires{PHYSA%2CA#1%2C#3}
		{{\it Physica }{\bf #1} (#2) #3}}
\newcommand\plms[3]   {\@spires{PHLTA%2CB#1%2C#3}
		{{\it Proc.\ London Math.\ Soc.\ }{\bf B #1} (#2) #3}}
\newcommand\pnas[3]  {\@spires{PNASA%2C#1%2C#3}
		{{\it Proc.\ Nat.\ Acad.\ Sci.\ }{\bf #1} (#2) #3}}
\newcommand\ppnp[3]  {\@spires{PPNPD%2C#1%2C#3}
		{{\it Prog.\ Part.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ptp[3]   {\@spires{PTPKA%2C#1%2C#3}
		{{\it Prog.\ Theor.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ptps[3]   {\@spires{PTPSA%2C#1%2C#3}
		{{\it Prog.\ Theor.\ Phys.\ Suppl.\ }{\bf #1} (#2) #3}}
\newcommand\rmp[3]   {\@spires{RMPHA%2C#1%2C#3}
		{{\it Rev.\ Mod.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\sjnp[3]  {\@spires{SJNCA%2C#1%2C#3}
		{{\it Sov.\ J.\ Nucl.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\sjpn[3]  {\@spires{SJPNA%2C#1%2C#3}
		{{\it Sov.\ J.\ Part.\ Nucl.\ }{\bf #1} (#2) #3}}
\newcommand\jetp[3]  {\@spires{SPHJA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ JETP\/ }{\bf #1} (#2) #3}}
\newcommand\jetpl[3]  {\@spires{JTPLA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ JETP Lett.\ }{\bf #1} (#2) #3}}
\newcommand\spu[3]  {\@spires{SOPUA%2C#1%2C#3}
		{{\it Sov.\ Phys.\ Usp.\ }{\bf #1} (#2) #3}}
\newcommand\tmf[3]   {\@spires{TMFZA%2C#1%2C#3}
		{{\it Teor.\ Mat.\ Fiz.\ }{\bf #1} (#2) #3}}
\newcommand\tmp[3]   {\@spires{TMPHA%2C#1%2C#3}
		{{\it Theor.\ Math.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\ufn[3]   {\@spires{UFNAA%2C#1%2C#3}
		{{\it Usp.\ Fiz.\ Nauk.\ }{\bf #1} (#2) #3}}
| }}}}}}}}}}}}}}}}}}}}}} "|" is here a comment (catcode defined above) to
| }}}}}}}}}}}}}}}}}}}}}} include parenthesis for emacs to parse properly. 
\newcommand\ujp[3]   {\@spires{00267%2C#1%2C#3}
		{{\it Ukr.\ J.\ Phys.\ }{\bf #1} (#2) #3}}
\newcommand\yf[3]    {\@spires{YAFIA%2C#1%2C#3}
		{{\it Yad.\ Fiz.\ }{\bf #1} (#2) #3}}
\newcommand\zpc[3]   {\@spires{ZEPYA%2CC#1%2C#3}
		{{\it Z.\ Physik }{\bf C #1} (#2) #3}}
\newcommand\zetf[3]  {\@spires{ZETFA%2C#1%2C#3}
		{{\it Zh.\ Eksp.\ Teor.\ Fiz.\ }{\bf #1} (#2) #3}}

\newcommand{\newjournal}[5]{\@spires{#2%2C#3%2C#5}
		{{\it #1 }{\bf #3} (#4) #5}}

\newcommand\ibid[3]{{\it ibid.\ }{\bf #1} (#2) #3}
\catcode`\%=14
\catcode`\|=12
% HEPTH's: \hepth{9912999} %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\hepth}[1]{\href{http://xxx.lanl.gov/abs/hep-th/#1}{\tt hep-th/#1}}
\newcommand{\hepph}[1]{\href{http://xxx.lanl.gov/abs/hep-ph/#1}{\tt hep-ph/#1}}
\newcommand{\heplat}[1]{\href{http://xxx.lanl.gov/abs/hep-lat/#1}{\tt hep-lat/#1}}
\newcommand{\hepex}[1]{\href{http://xxx.lanl.gov/abs/hep-ex/#1}{\tt hep-ex/#1}}
\newcommand{\nuclth}[1]{\href{http://xxx.lanl.gov/abs/nucl-th/#1}{\tt nucl-th/#1}}
\newcommand{\nuclex}[1]{\href{http://xxx.lanl.gov/abs/nucl-ex/#1}{\tt nucl-ex/#1}}
\newcommand{\grqc}[1]{\href{http://xxx.lanl.gov/abs/gr-qc/#1}{\tt gr-qc/#1}}
\newcommand{\qalg}[1]{\href{http://xxx.lanl.gov/abs/q-alg/#1}{\tt q-alg/#1}}
\newcommand{\accphys}[1]{\href{http://xxx.lanl.gov/abs/accphys/#1}{\tt accphys/#1}}
\newcommand{\alggeom}[1]{\href{http://xxx.lanl.gov/abs/alg-geom/#1}{\tt alg-geom/#1}}
\newcommand{\astroph}[1]{\href{http://xxx.lanl.gov/abs/astro-ph/#1}{\tt astro-ph/#1}}
\newcommand{\chaodyn}[1]{\href{http://xxx.lanl.gov/abs/chao-dyn/#1}{\tt chao-dyn/#1}}
\newcommand{\condmat}[1]{\href{http://xxx.lanl.gov/abs/cond-mat/#1}{\tt cond-mat/#1}}
\newcommand{\nlinsys}[1]{\href{http://xxx.lanl.gov/abs/nlin-sys/#1}{\tt nlin-sys/#1}}
\newcommand{\quantph}[1]{\href{http://xxx.lanl.gov/abs/quant-ph/#1}{\tt quant-ph/#1}}
\newcommand{\solvint}[1]{\href{http://xxx.lanl.gov/abs/solv-int/#1}{\tt solv-int/#1}}
\newcommand{\suprcon}[1]{\href{http://xxx.lanl.gov/abs/supr-con/#1}{\tt supr-con/#1}}
%\newcommand{\mathph}[1]{\href{http://xxx.lanl.gov/abs/math-ph/#1}{\tt math-ph/#1}}
%\newcommand{\physics}[1]{\href{http://xxx.lanl.gov/abs/physics/#1}{\tt physics/#1}}
\newcommand{\Math}[2]{\href{http://xxx.lanl.gov/abs/math.#1/#2}{\tt math.#1/#2}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% BopHook %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\if@preprint\else
\if@proc
\newcommand\PrHEP[1]{\@JHEPtrue\special{!userdict begin
/iseven {dup dup 2 idiv 2 mul eq} bind def
/BHend {
  translate rotate 
/Courier findfont 30 scalefont setfont 
0 0  moveto 0.80 setgray (#1) show grestore}
 bind def
statusdict /duplexmode known 
  {statusdict begin duplexmode end}
  {false}
ifelse
  {/bop-hook {gsave iseven {-90 550 570} {+90 50 300} ifelse BHend} def}
  {/bop-hook {gsave         -90 550 570                      BHend} def}
ifelse 
end
}\let\PrHEP\gobble}\else
\newcommand\JHEP[1]{\Jsplit@ident#1.\@JHEPtrue\special{!userdict begin
/iseven {dup dup 2 idiv 2 mul eq} bind def
/BHend {
  translate rotate 
/Courier findfont 30 scalefont setfont 
0 0  moveto 0.80 setgray (JHEP#1) show grestore}
 bind def
statusdict /duplexmode known 
  {statusdict begin duplexmode end}
  {false}
ifelse
  {/bop-hook {gsave iseven {-90 550 570} {+90 50 300} ifelse BHend} def}
  {/bop-hook {gsave         -90 550 570                      BHend} def}
ifelse 
end
}\let\JHEP\gobble}\fi
\fi
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% INDEX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%..?
%                          	% REMOVED
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FOOTNOTES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\skip\footins = 1\bigskipamount plus 2pt minus 8pt

\addtolength{\footnotesep}{1pt}
\renewcommand\footnoterule{%	% NO HYPER...
  \kern-3\p@
  \hrule\@width.4\columnwidth
  \kern2.6\p@}
\newcommand\@makefntext[1]{%
    \parindent 1em%
    \noindent
    \hb@xt@1.8em{\hss\@makefnmark}#1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand\contentsname{Contents}
\if@draft\newcommand\listfigurename{List of figures}
	 \newcommand\listtablename{List of tables}\fi
\newcommand\refname{References}
\newcommand\indexname{Index}
\newcommand\figurename{Figure}
\newcommand\tablename{Table}
\newcommand\partname{Part}
\newcommand\appendixname{Appendix}
\newcommand\abstractname{Abstract:}
\newcommand\keywordsname{Keywords:}
\newcommand\receivedname{Received:}
\newcommand\revisedname{Revised:}
\newcommand\acceptedname{Accepted:}
\newcommand\acknowlname{Acknowledgments}

\newcommand\today{}
\edef\today{\ifcase\month\or
  January\or February\or March\or April\or May\or June\or
  July\or August\or September\or October\or November\or December\fi
  \space\number\day, \number\year}

\setlength\columnsep{20\p@}
\setlength\columnseprule{0\p@}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% DEFAULTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\pagestyle{plain}
\pagestyle{JHEP}
\pagenumbering{arabic}
\@addtoreset{equation}{section}
\if@preprint\else\if@proc\else
		\let\pagestyle\@gobble
		\let\thispagestyle\@gobble
		\let\pagenumbering\@gobble\fi\fi
%\if@twoside\else\raggedbottom\fi
  \onecolumn
						
% FOR REQUESTED FRONTMATTER ...
\AtBeginDocument{\bgroup%		SOME NICE (LOCAL) MESSAGES... 
	\def\@APPwarn#1{\JHEP@warnl{\protect#1 should appear 
					before \protect\begin{document}}}%
	\def\@APPerr#1{\ClassError{JHEP}{\protect#1 should appear 
					before \protect\begin{document}}}%
%	\if@title\else\@APPerr{Some \protect\title{...}}\fi%
	\if@author\else\@APPerr{Some \protect\author{...}}\fi
	\if@abstract\else\@APPerr{\abstract{...}}\fi
%	\if@email\else\@APPwarn{\email}\fi%
	\if@proc\else\if@keywords\else\@APPwarn{\keywords{...}}\fi\fi
	\if@preprint
		\ifx\@preprint\relax\@APPwarn{\preprint{...}}\fi
	\else
		\if@proc\if@conf\else\@APPwarn{\conference{...}}\fi
		\else	\if@rece\else\@APPerr{\received{...}}\fi
			\if@acce\else\@APPerr{\accepted{...}}\fi
			\if@JHEP\else\@APPerr{\JHEP{mm(yyyy)nnn}}\fi
		\fi
	\fi
	\egroup
	\auto@maketitle
	\if@proc\if@speaker\else\JHEP@warnl{One \protect\speaker{...}
			must be specified among authors}\fi
			\if@dblspeak\JHEP@warnl{A single \protect\speaker{...}
			should appear in proceedings}\fi\fi
			}% IN THE BEGINNING THERE WAS THE TITLE, TYPESET IN TeX 
\endinput
%% 
%% End of file `JHEP3.cls'.
0502086.tgz                                                                                         0100644 0002252 0000027 00000331336 10252115170 012306  0                                                                                                    ustar   albrecht                        theory                                                                                                                                                                                                                 � B��B �Zmo�8����\H����DQ
��7����A�@��n���vw_wێO���!%w'�l27ڍ�Y|+��*��N����t���_�Oi��$�N)E&�)�ڤq�|���q�H�~�h��T�B������ӭ��M���vv��R��M��>�;8�����O�����e{�*���ն����Wr~���^��R��,��z��]\�����\�����R6��<__�����,���R��~�^��WR�ɿm�-z/v�v5�\߭���u���JFI�(��JZMv�ռZ�޶��N|_����󿷗���|���p������l}����&�����U�OD�\}Ė���t;�m����7��J��O�n6�v�k�}����v�~���B�����JN�>��+���h��_���y�%�����f���ILЮ^��2VJΙ��Wr ^�����	Ϥ�.�9�<�M�;�s��Ew.Ξ�I���6x�y�����n9ݷ(^��;y5]�Zy6��-���ZK�ۻ%(7����D -!���n��η�c��^�:�ֽS򨎖'��;�R?-�Z������l��M��q���n���/�+L󞔷��V���q��C�p\-Y;L��*����9�+���I���7���Q���C�Ck-������w�v��.>���v������RI���RN/wR�z�%���`����v�\�����m�|�k�ΰT?pΐ��²��wX5��Pٻ���m着U����-�9ԅ���l�Y��n�!!/@t?O��4ĥ�^|�gW���g��
���OMx��[��_�짋e��,h��Dګ����j��q��u��9��j��~�I% ,1�P���\N�r��NŤ\��x1)��yu3�v���v�4�ٚ�@��3	!�nr�^KH�
C<E�w�n�s���r=�c
������]�3���Hn)$y&����j�AX�"�y��*�U�KN4�f�ህ l`d��3���z�*�.���z#�ל���|T�E�e:e��<��f�Ǐ�G��:���@����*����h����Ub��(9T��#4Ψ��d1���>��̿�7A���G�{���nz�AG�5�q.��d7�0r��>���L��	!�	�|��>��QV7~F�<x&A��g��M;o����E��pr��F����ԋ�=gV-������2��q���|;��޾/V��ۇ����=-n��n��_%<
�jQ��u}q���T/j�����z!螇�2H���=������hDf |1��\w����� ��
���xN���B���v�������rw��ؑ��&�=�
3�#�<u�V��bg�����l���7�=�O��e���� �s��d��qf���8AL�RK(T�^���j�\��6~M���P+���������i�+̃���Y���հ�O����邒��C�a�����@�����낲��}c����3��͟�!P!���~g������g-�{����`P���V+��`ɹ��m�O�Y��v���rS�a_�g�d���n6��5���Mw�k���"sr�^�*]�V���mr�����L�ɛ���}�_O��υ�r@��M|D�z��@NH#����[����"�Cc�HIS�g��
0�[��t�1���g��Y?l`~sp����s3�?nx x����L����v�����1���#�O)E�*=�X@��9�8���7�����ݷ�����S��aB�v�11ĴOgb��8W���o�IY��n0��5���׏����"�~;��������S)!X�#���!�p�n[�:�{Q/v����勳���K���P��߷���	�/�w��;t�g��o����8����Vχ��<�9�2��ç>�D�0�뮽��y�� �#��$�cʘz�?P��vp^�z�^O��(4]��O;7x��W�����j��{zmll0�ۣ�8�^*J���%1d�a�6P����-����.��P�]��^/|4\���~��sw.7"�P������!3�N�3{�Nb�h���'���b��Sx#b��aх�Ӆ&�v����x�e�����[&c���B:��5��'�02���S;�B�}�H���\yQ�'x[����yo9�#�uv��6X|�Ǖq�Me���8Sy�JoH��yq؞��b�p�����[�W�M��v��aX��)���$\�YgNi�4[��uE��v)���c��x�x<�S	��ʜЩ�M�F�9r���4��t���FQS+]!�)mT��U�"�S��5M����*R�Aŕ+���JťK�2uU�����0t�S���l��JDʔq���8���J�$�`:J]�]�2]�*s��U��M�\�7&;�ژ�!�yBӀ��L!�ǕuU�$��e�DI��e#�����sq)�n�����v�����+ł\�a���ݟ�,v�jR�����,�v�eMj�k��eV)j�S��R���`�a�j*G�2Iit���:�U��F�:A�M���I��$�2i�D����ei����<���򢴶a%�,:�D�b=\e�W���RʺB�/�z����n25��"iUh�l���P�&u���:b�Xh�"q!#U�x��IeS><�"�E�5}&$�9K�<�5�Q�\�6C�N2csW���h,�҂6�{� ����
�J���*[k�JU	�5X���7	�(�L��.���	Eᷪ���于1`SG|;U[ґ��g��І
/�
l���C�˨2&��`N"Pդ�b'P ��cJ���V~���{�c�47��jFZ��� )G���J2�%>ˑ�.}��[��>�%�y�R��V[*��]>�v:�b`�+Sz�jhB�C��m�[�2z�i�	O��Q��K���PT���*���F��zU�e֐g� }kR��e�9���Ah,V�2*`Z19����U�XUW*�1��	Pظ���e�	�K��4�@�MQ�#�1s-Ѩ6޺�.�b����/�F�s�nm�l�k���!=�BP����v��s��в\�:��+UbB����L�5����J%�*��)qa����$'9�,��!I1v��Ɠ��#�"��$7�����������9�X��R=PՑ���C䦴y�n30�Ɗ��@�1�?v�@�}�4=���1{��������j��EA�i*����,t�`T�Ў�� ��W�`�3P:?�V�ViQ)���������<�5��P.ү�F|7��'�<t,�!�|,={">��u��@��2����C�T \D�"0�����G!�`�Ԁ(��.�<J����`��T!*����R����2��0�r�DYH�ii-�9�`�s��1�jڠ�k�H�~U��S���l!İ�Q�R��A�c0��1��P�Q�"ۃ��ڗD=����
R;*,���%)�{*���+D��	�O.�������B�#��TQY/[N�'bMR3�
X���⍨�o�Ĕ��%���ʳ(�$gQV��9!H]��ϥ����զ6��y��W�]Zȅ@�\a�J�9�ڳ;�� �Y⌆�0�Ёd��s=����(;F����߂�/9��@�&���"PF`��?���Q�V91�T)�A�M�8H��iXi0�� ��#-ıL�f���w@�->�hߌ4Dl߀���4�41�O�Kc�4�+�AZ���(H��]i	��(H��i�f��4��8HK*1�O#��>�.M������>�.M���ȯip�� -EX3
�`��Am�(H�ai���4k�>�.M���1�O�Kc�4J���Ȩi��A��^d����(H�Vt��N��4�Q��=�O�Kc�4�41�O�Kc�4�L������8H�ai��A�=�`!�A��8HC42�����i�ç��F��Ӛ,�,�Re᳦Q�X�p�R'�Ԁ��GP�%9�������=�4����	6�.�H��Dy��q�7��d���7 �Q�?��"c��r2@3���)]�,�d������2�ǽ"����g��5���&��#�$-?{;����.q��&��r"�1��ʛ
�`�{�Φ������:~�o���YeM&jS6&t�����g�I|����G����f���> ��Cc�Y�TO� ���{o��{b --UQ��~=���V�4���ɀ3GU>��ǒ<�+����҂�6E<�	0j%w R���'}��&���zG��j|�Q�X$����|"��Q���S���M�0'lI��'�-ϣbAZ}>�M�:G9_����3h�h��Ѩa�4m�#4����w(.�U���9-����� ��Tx�S�>��dMŵ�4�|�j�8y��,��3Q�h��s�R�Nx�̃@X��7�G����g�G����g�G����g�{��i���dڗU��h�YN��^g#�e,�҅�J���,�?�>�R�����濘(�Ij��#il,M��i��o*�o�����
�[�*|�����%u�W_��.������T��҈��4Zh�&���tG�*�a�=F�I��@�Q9��7�	�]^p!d����.x�O�H���/0����~ĭ�/1�s*����:C���i��7�Cc��ȟ�����w�&q�/�8R�RLΊA+yb��2�~*tm���`mb���^q!����Eգ(�X��[��k1;yg^�!m��Wk��B���Ԁ̩�F�(�L�p��`�4�6�n1r$9�Ӿ'�5�q�� .���xu�_bЌI��s���*��hU���m���`��m8�M�6�-����,x�-x�N���r�r��}P��%&�>�Yr(��	4ak��#�^���ޢI� @Ԕ  y6ܐUA�3i�]���08M>�l��.bl��Pa���9d�� �2���aӱ8F��9�حc��JF��at%�P*����
���⃅wgXƐ&\y�=���{��$è�w8Sv�T�c�u ;C)"$��"���v/U>RB��@
1Q�!����X;;� ����)�/.6 N*��";����&^n�y���v;�l/��j�m#�����a ^^w�#�4���rO�M-`��p����y{ו&��N}��3�C�I���n����eǖ�I<���$(!"	 %+�Y������s�n %/��y~L��B-w=�vK]���q��7�B����0m� ���� ���[�j1��&0)S�9`]�M$��c܏)�H�)x���"إ�J%y;�4�@�6p&D�$pNd�,��ل�F�|�`p�&�a�����I=��ᰇ�DF�a��e�ip� �0���'��1&���J� l�n�x�/u��:r�����)$��$b�� �G��S�eY����@�0�����Z�Pj��H�*�� F�!���� G� $�eZ��RR�!�S�@w�]Y-2�(�e�CX틖R�CR��h%��y%̎c����4]���!��Ƅ~& �:��ǆ��P!����\-P��	$���{�RJa�c�M�� �X_A�1Qo�p!�3L���+��������iH����-/E<�!�B���ch���e��җ�?w��<H�V9D<��Q�p�?��sz?ƫ��T�¸(�*R�ce΃^���CCC���{�B�a�8J<������#� ��nA��ǝ��.�N��� L�2(�(�a��"�W�I�{xx&�%bX(w��|����!|���	Eē��+��A�H���8^��T�Oc@�a>ta_�8Bw<Lk��@L;p\��r��ufv��"�@�4C��:Z��|XIǂ*�(ǀ�M��Ɛ<Dj���D 3�%f��a-�1F���B�f#��A��0���/F�h�'N��"dƆHCg'��ʠ�?C��%���`-3r.=�ӡM@y_�"��сS9��m&i7�3���:uF�0�x\�t!"gF��@�>PF��ѩ�P�'�s�}!v�b���l@ B9�cF����e�)L	8�4H��J��T߫�F�""����~�pi�e��J� }D�!���b��6 +�(̴<�N���ER�,PD j�Ȅ_�-u�lD��;9Q�u�ѧ�|,q(��b� �,C����Z��r�p�
�J�h�M �A0b��x]�[P��d��c;��Ağ��K9O8�U%��C�z��9�frG�i�	�]C�p8Q'��8�X��V��/���DR"�ȶ�|V��'�L�%�r����$��#��1��P2�Xq!0dH��PHf�
�ٌW}���
x�9(�`�u$��`5�AD�:�:H������/�:��K��4z��V�Z!_�eC�xQ�L�#�
�J����$�*� �ϩ#<Ɛ+�Cb#؃l�"���jX�� h��<�'�A��v%3��5c4�;q,Ѝw�R���Ne���b
�I+�	�$�sל$&e_����@#D��6Q�����UT�A3� s��6C��n"\�ϋF�3�lC �48�@�E����
`\�5,@�&E'}Ş@�Q����Tlf \�����AN�G����φJ0�2��aa��-��F�:d*^�h���C��p�a���8"��fy�B���T*>yrS�r������̄!@} 2A�nQ"B��h@�"��HI���0!P9,+B&0R���������0N��/�!����ߢ��W�d�8V,�EN}q(h�@9��\_zT�J:� cZE�ȽъD���h<�\D.��V��KH2V�'֒
Y��	3�2䢼2��P$�)uh�E��B-�@[K��Er#�������%7P4&-���50v��n��:�*G��YhT��_� S�@]ņ.����9a���H���H��T�J�v��TG�*�уM�i����N�a�	�����$��V�Y�Ѐh�&E�z�8�S�����6J�X*O7���Ī8jmm"|�S5�yu��������:bO.�L^i�!����!�;��� ��'\�����*by�[��ʪE� ������0���,����.o,���!�d4��לxU
�?���x<,�0��#t �����h�<�\���f)�k��(��@ыa?ʸ�1A���
e�������[��	�H��q���g;0�Jw�
Z�HUVj��St,��ZUN���gB��.ZY�)�l~ZJk���Ԟ��U���H�����*B���}=%@��)�ņa�E�p�j�wr0��6�(h�
A��5�á��j���㨦��H�}x<��L*�<��r��-~�걆0Za�.EڋM��и '�a�
y.��	�0l�04#`��M�+��p3�)^�g�)�U�Tͫdt��bU%`DX^�9N��s�({����3q ��B`��&Ǎ�W�� P,eDD��,'ò` Z�S�d�E�++ ����1DAd��O�� `[=v~�����P��_I!*�I�	 ]����W�D(��Q<���qc5���&���"����IhQ�@��ȌsD�Ԃ�i 4���ϕq@S�H�V �3��>-+�o �@�j��c=
��%�� ��J�1H���#Bt���-�O�6D� �yG)|/0��t�k� �72���8�Z���l'G�Z�D�R���c}�!a 52ۖ�oT�Ԙ�E�9d��jERC`K�`1�c�J��F1�~����ed��*c�Km�
���[����k��b��t��S\�{@�К�}4��J�B�g��6�#?d��f
ٻ��=�B��D(�@����.sx$]���]�]<��`�ܸ�5x���\��R��	 :�pԃ��Aq?H��z�k��t-w�]��w�������=�������x��Nl�'�?� X'����=�5��m���-� ���W���`[0Al�t �T��ǻ_�}���F�|܀�)�� � Qh����P��6@Xp���0��M5�\�\L�z��Z� a��R���*SeD Uk{�A������!J� 8�eF%]�E^�aV�>w-2��<�w���!�Q6'�M��P"�D�1T-�{�P5+��Q�NN�;Y5.9:��ȥPh�Q�7S�#/.^�,4�Hr,Դ�n�L�H<�b[p��dŢ4Yn7�(G���b�)MU�+�����:��D�D^(��1ɩZN�\x/���j������a����$��5X$��	�4'b���� �+�SE_h��-r,�J�h��JH��0*;��PXP�i�'�j���!� *HyU6��z̽��hԇs�ʵ��H+)du܋�Nn���,@�γ ڪl=�J#h,�N��@�-�meQPj�N�(���B���\=N�n�ҚQT���0�zـV���l��Ԧ��X����f(��� L�o�@��r$"#�߱VS`�9���蹂
��%3ږ{f��8˱�00a�qK0*S�}ST���h�aͮ��&�T�$�f@�:b�0\�7�jo.(|E �"��'�č�J�Lmf8�� p�.R�P�J���=H�5�	F@FvPvi��1� B��`Tv����I�"�M���4��)������j��
�&���­����P|�BSJD��>j�����X�R�%��yi��������@�^S�Ix���ʾyy �T��4k#�O?�1�K�h��˘nl�Z*�42��@_LN�
����B�G�|0@415*�#�{P��R!
�aBH@@�I֓1����ublQ֥`iPB�Ɉ�=ѐ��X6�0�F�v����P��<��i@���B����H8t�д�Q��@Y�N�8��ZH���=��95X��
�0>�՘�F��(�Ƹ#�K@�ǬP�~!� ��`h}ޢ��T� FK����ᢦ��|D�`2��⥇�2��}�0E-CB5�|���!���_ =Ҝ��W�������0&�	��'y�� *F�v��8S��|I�E;�Jx%(S�T��ؠR��r䗺��Z#��i3 A�g�b]�{�$ �$  �O�S0���iCȻ�i��2��h��e�:���F��>�)>t�24�r��A�e#� ˾���Ɇ8��1ޭ�[M�~Ji8����
�:E*�J2F�@V���D���(+hB�3�E��@*��;�
�Ѷ�����9,'F	�6hԃ��Vo�"���sE����j���'���a�:0d��4������"
)�U`ZV)�!�j*�ҥN���M����8o�� u�*O6���C�� ���1|��r�V�Nd��XR9Lԑo*�gHu�VAdU����̡W�B�~��DT&*j��"EɕHX��(@Z ���>���HvԂ���A�!<��+�C$��:�)gq#�f(T�Ai`�)�ÑDZ��Ա��2�B�*���(A�Q �G#]�r0�U$�_BhƄ����@����lh*#\WM�L9@��5��]���ցhH�$U4cq��|r����A����c������-�����z!Lb��6Ͱ��!愎��5���MD������OM��B[JBe��>����;�:�IMX.J�mAK�q��	L�4�J��YB"����AܚX�,�I����Q�
P(�}Pl�Re��&��/nb�Jj\
DM�TЌ��$��=��F�LԊ7õQ�272����3�X)1enQyف(�ZP��A�$�2P�#u���
���A�;ٓ�x�n��A� Y�����8� �n�d�MK�����
Ĳ�1�8p�F�+��9���/C�:Jr
i!X-�d���5 p���Ņ��\¸��YF�肔L���%Z)�xD���d��H 娓�?Ȇ�&8dgp;:y�I5���l=lE]*?aY��95:P��$���@��F�(G���d�*�P��� ��A�43���$�H s8`�~���G$c�(u��1X;���(���7Q���X�H!��J�$�XS0������G�S <F��z�@TZQ��P�SD�{ �ʺ��A�c�N�ͥ�j�)H��I�8
�Ѡwу��\�>��9�H�2��A�a�(�Dn-d�c��C��񽂔�dV��A�-���þC�ŰUu�}?��LɼX��:c�hŢ�l���U�J5�A#��vS��Қ�DQ9^[b�aA�p�@���23G	���Ča�>/��@{�1�GC���&�x(�k���g:"zQ�T�j�ɑ���3�v!��:���р����C�V�1ʅ�f�j)߈6\�#�q�41�2V!��� !,Ȋ>1cN�Hŝ ����Ң �(�}b#rO��R
�N�A@��<dI��X#`D����f|�� ��C������ ݹ�d}��4��3��|T*�5�3�c4�t�L��+'@��T���s��b�҇;Q�C����J��l(�����"Vޕ{&`)�� �܆J�)��2Q�!%e*n���w�Ve�V��[T��"a=ҠXO<]`0�T��ʤ�� �J1�&{_Xv��l洧<֦��
N�Q���vU���k*���\�	�jX�F�`a,����4M?����/:,O×��ޗ�\Y� ��H�� )'�uR�,C�l�������V]�̋�}��/a�M�͙2�F��&u�vcf�A�k����j�͘���E�:3�"�1Q�QhF^���L��c�0�ď�c}.{���5-%0C���m&�l7e�,r>F:��'�v�<7�� @�] .WV�n�]R����THI��;/���J5*�c�E��cS���až8���������A6�)�(���2$B��ϊ��=G�i�Pw�zE,̍��n�V>Ԕ5��56dg����"b6$E0��%�*:��x0JJ��9<�.����'�H(>�U�'� ɀi����ಗ������rX��=x�5���+����-Q�,�_���gV����㎥�����x�6I�,�<�Ͽ�#�c���z聤�i���W���i�4��ʛ��G+���S,��U�����/8[��G�r��@Z�����C3z�������]�������_S��������ޡ����P�D�s��`��8������4)Je5��/����,y�����T�\���b/o� ��W�K�G/����T����j�C��H�@���g��݃���ʦl?\������+X�~-(R��I��x��P�P�N��!M#��jˍ�0`���� �&�R�eN@��!���x�
��lA�%�����tuG�qA��	O!(����j�9)QF�@d���a�!�1�gL��U�'EA3=�/�L�T�կH}��H�D�-�i���G����¯�uR!���B �>��	Qd�V!{���KdGj�&�{�4�,�TѴ��&k�7+5w{QDNDT+I�F�/����������7@�D����������&�D�W"/���FIa��qd��݁.�*�`�#�� ��	�`�U�Ъ�7�S��ǎ @s��Z"�®�\$���Ut�Hf��L��� 0k�����߰�&��<i&ޔ9�ՙ�~F ��萊��JԀA��D@y�u�E���X�Q�)	���~�L	��C�FP���d�=k )JT/N*�r�?F>4G���aGՃQ��'�Y�p��K!�4���
��16`����I�-���h�>�$�� �V`u�N&(d	 �!a�	�t4e=�͇���7u��<�I��k���83�5�`��	���4GG�Q��xl(]Y�4�H��S��2T�����.�.DG"6c �DC�425(�r�
	�*���
�p[9���gD�lPɥ�Q[B䎤�
F�z��[����a�$�lTbW=�<CfA ���i���B$��*�5 ��g�UR{:� Y���9�Y�{8�vQ��.6� �k�9�_������X�YƔA)!7�`ށ�'K�oC�r[b��tA�!�T,4[��>&=Tg%Lt�]IAI\e��� �'�1��iT��Уl�:%�[A	�J�:�n�F�פ0��f�5�N��6���la|����G��]3j��2�c�
)p�dM���A���V�e@�s��U� '���V���F��Q���WD8�d9� &4!���(*�����h�$UE=��Q���+G�qH�sEGF�}3ȥ������u�Ծ^�6�i:Ssa�B�I�p�4*b!X��{�2�
�\�2��&12c�iQ.�'��D�� (ӵ.A�����OH|�"�k�v+��,or02��ANFn�>F�#��� J�h��CҶ�p�Rф�#�/%����T: ��H�xֺ�i��k��ya�}ב��˾*�cF�������؉PM��P| c�=��;�>��Y_��8|�	ꙀP:�@� %��`�����wq�i���ZQQ�$3_�.s&��L/�q�%��(Q&A�����(��)����h��+Ch���f�b�p��Hʑ]��AS��U8�@��"��H�%3��iG� <�..BFq���:X"�_�gҡ�Č��u|�)�%�l�;�Y59�2#�l���x"р'=5ug�D��E"+�b�4a*V�旾F�[���@�";J۟�#V��$����@��*�:"$�������g-f!��nL_�Y ���h�ȸ�af2:���e�ޒfGp��� �	�k6#@��h�,Z%A-+����ۛZ.gE����Hd�#'Q�ϋ����_�x9�>�M*֜�<Uk��M4f�#m��]�y,Y�
-A;jqJ�	M-N�i<��ð�z
W�	1gd5r�G|�c�p�ؓٴD�y�9e1�̔��{[1q�����`�9���Z�2�b*��L���a����a��̮�"��q�#5	0G��X� H�*����%���lP�Ę��3�QP؄F���]C���C�M��MyGD�l\�%j��Y��Y�<���s2 ��F����$�C:�f�
�����0Ep1��$�dB��N60�z �`��mٌTiȆ"� RJ����{B+�@���`��fE�A��R@ �ZsR��� �t���� j�p�� �8���)�%��>w)�A+
�O�R��Pi@�p+���@�&0h�?���c�bXi���Jd�� ������i�)u�l��hP�p3s:�|:fb��U� P��W�K(}Wy�D�d��H[i(%�>`XtI�[+��#Tڃ����̕c��
��QG��:�i�`�r��ƚ ��_e�
Ug`*���#`k`Bm_�.�TGЇ��]YF���@���:�D �D1�Ր�}�|+S1Lmz�/�k��p��
C$�k�j�����?Y��NY͵�
X}�B4*f!N��oNh�(�ƞT kW"H_�eO��h@��!I�4��$�n��#�[8��Ŋ\�5�#f�о��|�SÒ���u��o ��Lm�,|��L�&�pWe�,�1�Q'2���I�����Ț�%+˕I���K&��ؒQ4`D!�����j2u��$���4�<uH33�qtz��7��l[��<��HY5Eqe ���( �f=��N��qY%��r�IDjA	J ��!���Wd �����d�4LX���"���	X{�ٮ���1���4�B�RcC	�[�c;h�R�ӊ�-������6	��m*Q�tH���0��m?w���Lc�f��'X*�Q9F&C�JP�X�ꏠ�8m��9P��cᎯ�F�2qJ�d�@�M�Qb
f=G�9`u�(�'��9ٸ�G�Ԧ"*4.�6��:�hXdZU�IReل�$h��̘�*fQ�R�����D�E`}���C�@��twb��v-5����HU1���D�4�vH��kE�l�ax��v2N����xǨ;M��(Ӡb,�F�H�������pK2k59�d1��Z�DXMF6��H���pj.�}�&^�9�D���K1.�"�M��)%��\f_d奒Xr0X3�aݢȱv �k9����j��bWfY�`iR>�1��s�6.2j��ی�h��M&@�)c{PQ��2L��P0u�3s!�H�N�ehA��E��JP� |y�gZ�s`e���*�YcU��A�q��@ԅM$rĘ�)$�+Q�����t�Y?���n��r��\KQ>[1"p����<rB��1��D-��� ���
g�������P�����,�R����(F$���<A��#��x̸��A"�d�h�C��EdC���[ò�
EJ�[4d�7뢎��5�8T
D]EE�b���a8كu��CO�)A�+�u����
�{�'�4�͔.����Z9��}s���E�9V�o/dC��0�X�!5q=��#�i!�H>�d� �i�%gȉ��Q{�L[���='m��oB�&jc�&��y���>g���&�VX�?���YXr��@��V��5{]d�WX�X�RO�b�_�fW԰���(��L��+nX���� lp��ڞ1�{S�wj���2�Z�I�7 �0� m��v���%2���P������Mg��/��x�x�#�;.������{~��+XAn0n���,eH��|�BC�u��TC���KNP�����f���nks�@�*_n+�>��{�G>�ݟ[~%o��~}��BF�sA�����A#O�L�H�-�@d�� 9��VrlCT�N,d�7 u(\�@p�0��2�r����r�x)�&�t��ۂ��ASB�(l�x��̪�]��'�n����*�sq�1�{ZpT�T�7��$"^zN�Ч*����r8U���"5���S#�[�X�݈E��ֲ R�dCgpp:�¸�ќ����+����2E��)[��P�zicv�/5�ޕ�a	�099��X���f���]���H3j�P��1b�N����j�_�Q��tԯX�Ҍ�@����LN���pԗr�6N��"�0��eV��;�Є6Hr�4�5E�����lr��ʑr3J� �uJQ��X�
�A?�{�Q���g&DCU��*�)K���ʁ�B�K�ګI�ʧ��%��66�,�t��=V��V��;�0V�
���u�㴧��J�������"�Zi$s��Z@$��h�L4x�)h��X; ����J��E��V������!$ł״�)l�cwH���"D%��U�R��i������-�"�d�J��i��.2�l^%B \(Ġd����(�4�R�͔���O������$���1YxE%ς��LQD�=b9-���b:-mk8�zk��<JN��Nta,����6�NoN'�@�ƒ�q*ϧ[W��('cC̗�2~ꥠ��[�
s(X�J�I���V׫*�M����(D��W�4�a����e��>�ӶB�I�+j��|�%(ۨ�g>$y5O��������f��1��ƽ:�?d�+�p<mo�҈cz�2+��D��=����L1qy���7T�GF�0O���e�!�y�Q�H�Z��{�΀�E��;%q��e2φ�ڡ���xT�����N��Β#B45L�=q�܊����Z�q·wD�c�k|���I�ܳv#<�T� �,:�9`���P�Y��#����kc_�� c�VH�`5�t�Wu,n��4#cN�s�|N�Z6���#e�-�fc��+h��5r��;��:��
H��tD�3HH;T`5�EU԰�a Դ�xʡ|i��Ѓ٘H+g��bh�c�N9GH���Pl��x���6����HP�y��C�ho��W2ۮ��b���`ёx s`(2����"��� �[4ǀe�L�BE8��jO��U�0��������$!�Gv��Գ������B���Ek����Y�d^��PT��)�Ý$;�X�@�o�E>hPd�E�����~���~���s'�uK��j1H�tF3P����`Q�' $��λ�%��q��5b���AA�%�������,���]C��)aj�m|t{zN���@�(i�y#�
�)�Z��C�,*]���T���X��	�\����%�h�X�7
Z,�2�J]�x�Ң�e�pN��S��"����G-i:�z���V���"O��ط�����T�zY�W	�J�LM�(2�HT)�`�y�*?hΡ
��n�0+'����J$Q��#��H%A��� 	1�6�"��� {���"���"J�1�c�F�%ZԠ��J ��)�9�y";nغ�4,�Rk�`��m��(S�YV�d�x?)-��$� +0�8��{���	�H-YT\��AE����(���*`�^O�Li�$��	��8�SX�m�kr��Eq@ȼ����C�{z��j#!&u<�FN�.b1�P`*@�CX#D.AYy?@Â1ԽxrgD�:h�@aE�t�hd6R�t����\��:ɿA�
��q4v!�<���%�b��9���sA����KF�*7����g�4 (Q�\�bD����D.´qu�5C#�vo�2z�F��*�b虁���>2�f� 4�=2eu��,���H��e&���=��ք|T�^+KR�ֺ��aoi�f�SsP.�4(4�'��!泪ۧ���]&׎ݝ�����!�&Y��V�N1-,��':��{�X]0��H�J�EU	K�X@=��JE�� �(�:�
}����j#�-���Y1JJ`a"vS9�9O���~2��QeM�옴�BM�h��f#UwR�\X�M�<H$��p��z�2�Jz�ܐ\.M�`Yъp��_��^1f	`�(_�j.dH����E�A@Ԩ3&�����~�*k4fHc�3�x�}j7P��W�1�U�\���R���DN.�����E�F+��%-���Ok���fC�9��d=���ע2	=�����ftV��X�
���d#V��rwn5��������4��f&�Zl�P�3[�v5�"j��13��ې(��8�Z�r�>5B\ՃIbN	�H�|0�F��@o���&���C<
/|6w�O�_�if���%�D���ؑ:a�%l'��Z�iЗ�6%ϱd�po^�4��;jBc#����8~��^�m݈se� ���!GP�Hs��a�˛�D�Q��_=6��N�Z��+�����������ɸf��@k�(�� z�K���X%E�d�yt��v(Y��?���x|D�y]�+�46'0���uj��������M8Ӱ]�ije�cрٞq������2�i�g��I����v���C��i��r����*f�3�(cE�QҢ$^E�6�Ҵ�z�I�t�2��ҭ����ò9�N�a�id,b-7�ʍ��d���}=�&ܯ����(��3l9��X��Qp�D��R��+AS6�
�(��&d<��7�<��ԃ����nE-�f����PX��㓳�Jd�R��`�H�j"1�ه�$�+�ǂ��5� GE:R�I�ZД�PH~����2t�J����J�3��-�-���eO3=�R�x d��N�e`�5P�QˎT�����j/�m4�J�5��dH�Q4a�4��u��qm�Nq�g��Q@��(\�J��Ԭ�\U ��53�,��!3�P9��`2�xv��b. �� )-�@�f��H�1�A�[!�����&������JS�J��13������`���o	�J,*T8���5�1B�c,��!K"�ߥ��(�Tky`��z�ʘ'@���]��43&����!n#�����8,kty�p�|d��Hs����~T�g&R�I�����%�œ6��O���N�E@gO��}A�Hy��q�P�g1e$��;�B@���8AD��]�fe类ӋQT�{�(K�����5^��% ~�g;�#��g'�w=|��6�!� ��K��R�`{4��]|C���z���=� ��:�5G�Y�樃�]�k���F���5�V^�pA�o��r�����LT�#�����fȏ������pd�B�$6� �����!M�`!P���r���Th\4�Xtd=Cݱ~N]��P�T��AaEܢ욖选;�!{RsK�2���;bمAs2��"<h��:��9y����-�s�l<� F��d��p4��:�0¡C�
���GTE���L� j��6�G����VI���#�7��Ja�[�� �Ԍ�Z��ue��_c���T������54�S�v�h��b��i�P; c|2��-���	#2��
XL�{�O�b���'��'ઈ<Г�`C�γ�*��L��� �2�R��q����>�xjh؉bS!DDz`e呩\�xß]
s�4RWS/�$��[��c�����/X�g'j]�2b>Bi%��t�0-�0�����A����4���*Ѐ��ҏ8�+�\�p�Z�ݤ�r�\ԔbR^��&x`t�D¨��PJ@���B䱕̀��'��`�eR6!0�Uq��a "Fz�URڹ	��� "\�̭��
)ъ� )���GeH�"�x����*M�*Q��Ȏ �LV�y#���ԁ�	�B/QS֢-A������~��4n�(���"d����[��GC����K9�հ�1��\�)�I-��d��X��`ɨ�O�\+Oy�J�2x�-�"ΰل��gADmFg]��!2����@#��)�$#z����>�G�*4Fp����8j%�Mt:�P,�0oH9�4E_!xDh����Ɓ�4��d��'��iQB� �֕�d����t��`�#='�	;��'�Ť~�c�Vl�tWTWa�0����bY�"��i� ;�QKD� ��Q���-���R���
b� DQ�0�A��������+�� ����-b=@�|�P����=��cU@�D}|H�}X����C?Dˢ���M'�ph�e����ZX�:�I
h"&E��Ә�T+G��ʧ�L`��OGu,!b��r+��c��XpQ�Yd�;�Q3"���2���:*g�`
z\#��'�j֛b1?�Y�q�lr��7>�aR�F*��Rm���|�mn�%���>�|�F���M�M�[6�#���#�q��A!�@�����@ϜiQ�1C�,ʠ���|�̐:��q��h��~�(r6�Y!� �����H�d@��>CV?} ��a�u��",�S��I��,�rh�qb���-N��N���d&�Q��0�k�q��?5��������o�6e#B5�T�&�dH���zF�x�a:��Q��*���z�O��W�H�c$�R��f�r����M<#x\Z$G��\�|�Ò��<���	D�����]	*wZ9��T-#�Sd�5��e��I�Ʋ�i�@"!�)���e�8_*�hl(0T*W)q��������5�@�����"S�.��ep1R35FV$��u���`�&J��^r��ı<��C���B���B���p��[��<|�
�{�ꤚD�_	�z*��!08fOV'jO��C�hF�9D�pe��#5���]�j-�	�H�	��[� ��cd��0�L{Ν-��`6-53��m����4K�8Ʈi|
0Ԝ%D��j$q?So�>l"YD5FA�}{l����X7)�چb����O�����ح~O�:�(8��uX��q��)J��<\;�Z!D��ڝ^#[ꠇ�NrDUN�x�^s�w�f!NbZEF�Bb ���zu�z#k��!=�*\-gŘ�}�_y����%��}��*a��#s�j6{����cG���6���/��vWn�qJ�n���m�FI7N���ʒi�y@���4��Ȕ��U��
}���n,	���
�M�6Dy�E�{���̏�]��w��Ye�PH��P���4�dDk!��E��K8*c�sFZU.5�QYή��[�@e���v��n8#�x`��vS��D���A��]e�׊�����5P�8R���\��8G�� "g���&s\�o9�Y $Ԃ�m�U��h�u�����od��!0�(�0�{���J�9�_�5JJ�3��H��
����ؤ�Hx~�����Vc��-wG����*<-�\������RhA�6��<�!� a�	V�hmH���hR�GŰ�Ȕ��Ti����5��	��
CcX�xI�(s�{h�f�ET�UH���<4`�f*�W@� ����-�eHM'��M`���*�Ւ�j�1
�E&U�>C���dek��"N�We��+� ��.���i{Ud�t� ̜�T�UuIjo#��3�"Qy��#�_�ᱵk��C:-�M���2(��F�5p��U����*����v��%�e��r�$3@��1.��%Ϸizd�"����v���5@�痀�нt���,8E�Ax1��}dY������c	����%x-$@�Ϯ�+�3��:�*=Z�1�e,H0R1�#jP��?�=��Ec�܂G0�!�ǉ�)Qׇv�{�%j^b��ʎ��ĈP�,�W]��Tr"rVi��l���4�1+�t�yu�R�#�E�Ԩ��HXq 	A��}H������wF��6:.z��V����
�R��	��0,�2�cŠ!	;k��F ����7��#��C�ۈ�>� UD8�k�R��L�*��+JN+ؖY*���3���b Z�u%/@%��v�`�I<ي'���	5p$�76�,�Ģ�h3B�I�T4���i	OM9�hGb̈2m,w8�	1������A����(.��!-ʜڐ�	ɺ,���ż�ə�	F�*��L�3s�����J��Y�~�R)�@P���^ᜄ1�k��΢f�>-�6"GUɰ���sH��Ő# u`�P�X�\�[�r�vw�D�5�Ym�-g	�C A�_�0��K�+�jw�0L��bQ���+k:���i�/�aX@��@���5-E���H�+�f���ntV�F8i�*a;W�,�ΞിT+���(�_j]e=#�c�T,�:`XBF|�&h�h��(4\�JF(��
�C*����CVm�q��
*z��w <E� N�2��O�ެlZ���Ϯva܌�1�O�=��|�Ӓe	��-�J��<�D]�Jp��L�>h�,;�������Cfu�^���.u_�%7e�@o�*Yv�j
�
��Yh �kl�������t:i�pM�
x�oJ@�Z�6>���xN0���E�A��ñ#�e@>ìsѵ|�15����2p�BX����l}ѭ����P�9��C�>ZQY��_S���*2&��S�(�9��BF�Ԋ�V#�����\C7�"��=�ΠȤc���Q0%�l�c`j}���Y
�yG���*xӲW��7�4�5$J��u`��a��AU9�
@K��G��kWxh���:>���3V'�^�c�B�l+D�����~D�(�!5��R��`<z�uD�P6����)��ș�OO�RVxp>nZj��]�V䡦cs�v�9Q���h}� ��L���������>���:��Ϙ�:d���1�u���=c"�됉�ϘТ�(xoty:�ӧ_<��V����r��v��p|�\,�(��O�G�3�:<=�7���yY��q��mW��|'L�hȣއ�QS�E�z�,�C������w�8D$rX �/Y�~*���2)ĸ_*Z���CVKSq�1e��\v�v��BF���\�D����Y�!����/ϩ,�Ŭ�0��93Y����΃��c#SAG�+j�A�Fq*�����i���/V��RBp� ���b��BB*<��V�����a�I��/ĬN�?�%V��9�4�����b��+�C=�2@�<]H��<#3�K �RF�����1������)�N���-�	����"���db�p�P&��8�"��9a���ߴ���O�47�F�e�Y\)��X�M�z��գR�J��&�O����&r�o`&fP&"ű�q�@S�9@�Jі���H�03��h�D"@*�̹��jN�d��1Aa���8���g\,T����7�d��&�`��2���T����:���.r���g�)!^)B,0?��(HPԨ,�LMX8�
�h!��S��
d��#��x��<�
��L�`@Y�"҅�e���ɫo*A	�3vgQg���$G���<NnP1e��.�'���,�@lθ˸�`U��:X~!�"ä"�����E~'��^���������\���g�Ϧ��+�1�NV׋����>�.��׫��2Zzz5���e8;Y���@��br5]<��]��e�����b�\nǲq�����J�P�K8�����UUVE�z�;���O�����{u-�����}�{$p�#�{e"ĕ0���c�]������a��d/Ɋ��惽$�2��w�=�3γ��S��L.}��id�j�t��	ddM�'.��^
��|/I˴�Q����ө�Nȶ���t�*0�"̓<׾⽫p:�|���Χn��r�8��=�_/�����������vv����8����5�;�_'����ë�?��{��_P�$������Q�_�?<K�y�/a�������j����/�'/Vw��z1�/��w��������g����� 9��S�չ�5.��`!Ds��0|~y}u>_��a^MV'/Χ���a��Z:�����^\<A���C�R�asyq8?���^�@�������������tv��?���Ph�_hEV���|�>��/V��+#ÝV�D��`<���*$��J\�N�wS����p�E�Z\O��ѳ���4<��/톼>������^��� ���it���W���Ux����<��#Y����[���j�}�Ƈ�}��)OC�����_O�X��8?o.毦��mx<�<՛O��{�ix��|�Orw������l��p��Ax���ϏO��������lv~�?�I$�I�`%��&�������ux�\/��W���*\������ �k+�4䛶�O�����~
��^]	뾜>����4v������~!��#�$��}��xB������m�h�
�[V��3�}��
�o0�o��gg����t�|�����'��7�}�_S��u�GǶ@]�1�g�-���@�F�){�7Y�����*d��G��>���E���6���ܙn����$�W�Z1��#�P(@����w�巘œ� ���7��K�����<��a���i�M��,�7q�ac������������z��؞U�)>e���K����aj/����K1^"�<���k����ø�u���^/\��z;����?�����1��__�Pfq��}Z��Ӎ�eI�mC_k��oCiϗ�W�.P}�9��}�|1]�@�`�p6�ޜ��d~��DjrzJ�	"F�k��;�/{���y�O���|9%+Ү�UL���|y� ������ �D'w����=Iz���;��������;�a�i�@;����=��:������?��B�0�Y7���GD�0�Z����������A|X�S
�+j~�7��Z7�g��o� (X�vǿh�:��n��;��2��fw�Zk����#B���[s��{�a�������#q����$n��|1��R�M!��vE#�\��$���τܔI���ڛOn���J4� �X����D���z�T׹�`�89��;k[�(L�(�,Nܫ>Ed+w�������ȓ���Z5 nX��h�����wn��VL�k����jPw�ܫ��:�o���#y�4�@����l�/�o:�엌 �'�o6�����B�ڳ�~Н��8�5�y�~�i��_0�߲����Oݻ���/@� # -�mF�C�6���g���$'����r�����q��xc�� ���w�\�t)�Y�"P��1t{����5�_:ͧ�y�&t��,��%B��jʫ��g��T����OUU�;��z���d15�:�����S�������J���K^T���ɻ��N;�� |n]S����=طu6oo�I����,��m���G��4�{ w�2:�����#~��2W��պG��mo�_[�a� �-~�"�#!��%����5�wE�{��>&�K:�b��]�lܶ�Fn��?����쎮)5���_H���|��;�*�����&D�0�MC��B����[H��Br��[H�o!{{��-�oo!�����-��P��������P��B����@�; e�6�|�|\�� ��[ 3~Ќ���; g����<����l2�o2�v����wu�����.��&��w����w�?�]�[���?�F�Y����.#�}�ǫ���ڮZO}�<�d���C�?�S���w��[b�־��M��G���1|�a�f��u ���񋁿��6ȿ��ȿ|� p�B�������\�
��;DH����ҏ�1o��M�[�y����Ϗ�?�v®x����������?�ϻ���ϻ�����~����m��^�^��|�zv��ao��_LV�������_�f�Sy�?�i�1|����/q/����������qx>=]��ӳ����K��������<<V�~z*o��!ok8�Dx��������,�C���<y~>g�2d�t)M�^Oe���,����gK|!#zF���l�/����'��ry���2�Gވ�z��x~��,�m��Q�|��U�+#���^�<Mמ6մ��[`��w#YkM��t��O�gW|� �C\���:�����:�����`&��fI y}�s�h��D�i;���p(�[�m�K
�g�s٩�W���x/(�C@>�� ��8��IX��Ka����D^�v���N?����v�&������������3/�-;syz6�\!�,
c��a;/&/�x`}Χ��
܄�7�
�h��0��Є[ކ7ҥ��'�n��la�"��0����G��5:5��}�~a{U��i��7����f��n��h�)>4�$=T,X�L�uo�*���7���PiJ�ό�O�A&�\�c�����]���d���Q�����kU:����Mb�����:���'�l��v�u�*��j时?d�GkK��O�����k��~ɍN|n�!sV�
��ւ�ϫ�1c,c�����R��կ��:�[�v�(���XAu��:�t����q�}Ü��o�o��ͺ��^����B�7ڳ�����Ķ6��Ӡ��P�d::�#!S���4
E`~�`������jv2�k7-΢-�3�?�O�:��
�DzP��_��Q|������^�&���M:9��"M��?Q��;�޷�ȣ8,Cݦ�Ϋ$�6�X;��T;�x#���m�$oo%ͣ�����#�����"I��J�ֱ�y�n�bo����˦$q���L��m�����VU���JYo{�*�:���cI��mcI���+��;�ʻ�I�Uo�A�m��꭭ Y�m�p��P��'��✉�rq���3?�b��0�\�8��w��o�������D�;��7V����.���ƛ?���-}��P�w��o������-���}�͟�w�6`��v��9��y����`�Y,�'��Ա\4��[Ȕ�>��7�A^����������?�Đ4�+i<�D�*eI..2�"s�2w'qww'�\ȣ��;z�;��Sn��;x���Sw'uw\�q�W��Dv�u^�oב�����uݺ^]�������{/?�{{h�ml)��b�Oڐ+�Uw����_Ѡ����������[��0��o�� ԋ����RA�����4	-i&����0x�-��J�0M�/��ô �H�&\�0���C�ˊ0�{e��=�'�s�'G{"C�x.rb��yg�����â"2�%��a�����+ӰB;����f��r��|*Y�։\�N-��%�P��e��A�L�.b���<p�{��]����wQ8�j.�ΝM<��ݖ��.6���)7��ܩ�^t���˲y���Ӌ�;�wG�7�.�Q��4{Ѽ�m<J�G�����;���s���N�.6�T����I}�.{��LQ�.0�\��.)�
�۔U�-׊jv!��X�b�`��Z��.�B�!����2�K߃�}� +�����q$��!Q��i��ŀ<"x��-I�Z�̕w(�UJs��3�������
�EU�\ki]�k"9D�V+��K1�<�e�s!��u�±]nZsQ���ݞg���]� �*�`�nC�M$S�L�El��>����ܸ�\����;����E��IҹS;1�rܿ޸�L�M.�M�������Pj�w��_�6;�gڟB�T����Ml�����BQ�[��sSQİ_�%Q>,(�?M��������,U %��3X���x�0'������W�����R��"n��B���(j&��
f#|�I��V��P<�h�H���c���ݑ���p9=A��m�.k�w�r�p9q�.+�V>
W�OS*��d�6���E��G��ܻ����e�"�/
wQ:�-��w��E�����ĿhP�w�v.���z(��:�aMtmPrj���߆���O���z���'	Ko�a�r�Jd��;ĵ������f��@Eɿ pd�g��!pd�(gN ��SE`rQ p�\���E�\f��e�\e��U��[;���C]}	ND_U�Z��<���wG߉�����t+�u����tu6��}��n����c�m.�{;}�ÆHdN|^[l�n�#���0�Md~o2T��,�ְ���6{ػ�w{Ⰳ�NO݆��'��o��c{�w`on�[�����.�[�aoj؛�a������Ұ76��{+��԰�P�%���d���B��N{+���a/g���0_��W�Ӓ㜋�N7�����ԫ9�QƬ!mM����R��������ŅW�/g��2z�����������a���CЖ������=��{���P�����C��_��<��{���P�����C��������=��{���P�����C����n����=���*~=��{��7}���3�����C��������=��{���P�����C��������=��{���P�����C�������������=��{���P�����C�������_�P�����C������+㑹��+ȑ���+Q������N��+��:`L��Ef��x� f��(޸�:w���[�D
T��y�t�*w�s�}T�E�yK�Fw\%�4꼓l\���za����Y�"�20[.r#�����G(�\�t[�.�;��"S�5ܚ�n���Y��)Ք�K:��H���_Zy�&d�\���հa�?C5�"w�����q+\�A���7A�����q�P�����z�V��|�>R̴t��J�Q��Q���pV�pKWX���ܕ��]������K�C��C��Ci�!u�-���V���h��H�E� M�QW�/q����s�v0u�$SH�h��5�K�����O{�Yͯ)5ԭ'��[�����^�����������[k�*Z����J쪀su�b+�j��BL�¨+�آ+:g�C}]�B ��YA(ݭj��E����>h5�2�L�[�*,@	�r�1�
ޯ�>_��N��e��Y�K����_�������B������vP�
��M� �*����*ܧ�+�P�"�����
@����]�>]�̡-�7�bkְ��a�c�@�ԊC)��c��ƙ:�N�n��}\�/'S8!�P2�*�����M���b��f���׫�m��uFv�tU�5y�Y��gv�����o����������E�,t�Ouy3j��1�Ī~)2��̕�⋬�WdU�+���0�R&�V�Ե"5�X��Gv!�R�-y�F_�5�Pt3	��,y��W���Xs31�e�>���꒺kٯ��������N�(����,���俎��h��mR)�\a�m�жp����e��f9l�:����.��h��m����k�h��;Ndm.�ڹ�%s��,�w'ڮ׳�eh���m���m�A��L����lޮ1]W��a��x���m�����Z��Ԫ����&kx���9�M���6�M�xK�x��Z%�*	��rc����m����&ޒ=�������V�����m��4a��"����������]��$�P��C����Ӈ�����=��{���P��Wgc����=��{���P�����C��������=��{���P�������C��������_����M���L8x���P�����C��������=��{���P�����C��������=��{���P�����C�����C��������=��{���P�����/��w7D=��K��=������ߓ���+ב�������E�;g�W0��B������E�qрj�q'�\�w����۬�wǝ{��5w:���;��S�/�;w�N�-o�l��Ru���z-�G��\4����~�n�p�x'��)]�5W���S�w\��ĕ��^��_ԹpŢ2Wu���\����_�.�������E��_Z�?C7+ة�g��t�JW׊���\n���1�����*W�����\��ҕ+݊�4/\ٰ�-��K\i��J�a�rW�QV�`�t�����E����l����7H�����P��1��%֊%�j�E��X��2J�^c��BW��S��j���EŚ?��%��a��ػ�!Z����vʅy�����\��R1�dݯ����k�YiΦ�_n��g�����g9++C�Y�/��_��6$�j���=�
׋x�B����_��[M,v�Zo��v��5��6���S��a�������kK�9l~���pX�jx�U2�����:lL:�hl~K%�j� g���n�0'��:d�V�ۂ���wK�NW�/1�}�
b����+����_�[念
b*�z�����*���z��*�����=��*'c��C�ԐVn�J�����ʻ��6w���:�j�r�+���r����R��)��Y��)��m\�i�푶�P�CZ�ܟ����v�5�,ӹ���ܟCZW��!m������nn���א���yis����:���?����e|���������qYFq��Y'Y���~�����[�wtj�qr>Y.����շ7������68�F���KA�����Ջ��r���o.�'ˋ�����jy6{�|q�MNOWs|�9�7W�u{������W�������A���|O���ϧ��������6槧���K�������B�Tzz1]^��~{s4YL�g'7޽�mߜ�����j*_�].t�ܓn���'K4|~�b�������ώ'{�v�t��^\ܠ�γ勉,���{�\6���?�ٹ̡�����,���	��}���۳g'�����þ�����3��g������Ï���?��{����\��=����{x|v3X�r�>|������+�-������������ӫ��ۛ����wI8|�d'�|��_����	?%�����O�~'ww6�Ӌm��ݝ����{{ss��x|�|�1��QGݿ�g���z��s ���N���w�5=��&�������{�?��1?kW����Oڧ����i�����a�l���5�-�Hć����n��A�O.�O'�����x�`�z�7O�ڨ�����v~"�1]N�߄Of���;�^��/n����a8�/�_��?�,f���l=;y1��#���o�B�ã������ś��?/g����l��|6�<
��.��[v�x6_��O���}�i��H��O����8�7��p�@�8����'����ɋ[iJ��t��_/�W������k"�M���O�g�7��ů|pt�X`�W�Ɣ�Λ6>^̯���/>9�ꓽ�p0z�����h""�,��j"Z�~���l�w�,i���g���C��r3��M�e\���M�g�g������x��1�_�y�a�\3�{z5Y�旡V��X���W�����Z��W���� +!�!�#E(��! ���٩��>��&M��IxxaA�0�+8�	�5�+8/�`���Η�G;�f���C`���|~br˫���Kz��v"Z/��ײ�6R�a���c�L>�\�d&'/��" ����Pڐ�OP�7<�?�,f���/q$��_Le�;_ʠ��g���ٯ|�?��'Mw�h�]n�	�*_�B(8N�dq1ċ��a����j";*��9��WS���?���_O�:�����|5��ίe;�.| �`�����B���1���DǓ����K�q2���>�@��<�_O�ۓ�s��l��j�i�\��K�t�'���+�+a��&��[�)�<hv�j1�pd| ����k������	��WhR��Ht@�z���QR��8�Q>���|z�j �6�B����B�����_�(�C�\�`N��7��Hg���砖�U�br*$Afz~>��q�dŗ�痄TY��G	��BkVקo���D;ԁ�
������aTW�����9:f� &$��@�p�������M��/��t훅 �b� ���ב��-t��_�����Ik���V�����A����l&�{��t����T|Y&%�I$׋  {n�̓K�A���Q���a��� �j1;��@m蚒apT�g��|��Mwqi��l?�����c�F�{\0�^A���a�'� ��E(��w����]
y�n�-��t2-R����jz��ۖ��T��̛�+�O�@pù�2\�p�Nb����ӹ��($5 g��7�$��q�(jƂ�����9h�!�����
�����pn���
v]N1XY��``�'K��g�ӯ&�(�?��"�?�<F3�<����y�\%�~������3{�X�c,��DH�`EF#LB`O~ΖB�e�NN��r����$<[�/�OFO{��+a�޸mA\�i�s]��"dpv.��YE�4l��rPT��n�A�����	$ m�,��<���%Z��V�b����QF
����8,����`�]̖`�\�٧ْ��u9&Ix<rg7VGZ@<���̸Ђ/�Q�q���}�u.�'�]}�����4�8��=9��\o�<�R[���+P��<y|t~~�]�I|��p�A�f�=AEƙb��9_�uG��k�P���镴=�<���̧gB�q ?�ra^N�V�����ǓV��cUwwdr�G�C��Rr\Q�g��س�)73a�x�lUW�<�����?����{�":F�-!�Rh�D�+p������BPmо�V���`���J:�ȌI�`N�O��4�#���d�5H���悚|�b��K!�T ��?���k[�B��U8�@��Ȅ��X�	�[��ƱkŎ�t�s������1�� ��<@�d�sc�g���F�|�,�bP�� �ZVEx�l��-O��B�����$��rym��dF٦������ř�9�)��w9��
r���k�!�+O�B&и�&O�	=@��qgH0ݮͮ�v�
��37	���t2=w�@�#T�0��\'�D3���V ��PĠ�i�A�����IQ�/E)A>=����́�T�݁YdOiP X�W�����5�5�zg?��\L���`�Cחuv1�8Y�!�jt��������B����Kh=��dJ�~�Bu�|�y��\M��\��O��ªssypq����K��殼��(	�dN����w�o��s0>Y��
9���4� V���a(�F���g��p�ip�[����BI�e@hUcT�wPdҸ�C��yy���k"���W3Q���>?��70�	5��6/��`K����[T��ڇ��x�j�$L��ߑn^O�O���p!�[��n+;�	\5�������������s�c�ݐF;w<��.�!��a7�03`��#(���h�i��2���ҙ`>W�$�J����s����ÐI����z~" �
&�����Q������5��j./��n2Ws�L|i�84נYTӊ�f�8��W/SX^L/��H��r��-
Ћ��zD��?�&����4�m!���B5��9���/���z�؀dw�]j�K���s�L�4�hb��em�e���A�ݦ�0O�Zl�1�z�.�z/��h_��a�s�nYQ��Y�dL"ix��t�c!��_ $�����qU�[�u<Y��0r���I���fI�x�i._܅_��w��.����]8�����k�%�D��f ���i9]Q0�.|?�MrKc�t�r������z�ȷ$��4�ޅ.��r�����lʥ��>L�� ��V��.��d1��zFg��}��S��%�^45��]��9w�@O�&���eE3�F����1j�D�Yax�����o�o��+��*�^�_��M���h_�*_n���1�(�/ѥ��Ue�^� (�E��\3=+g�/���s�	���(!�
�G����T��%�07v�»Y9����de�Χ�v@Ub�Pe#!b�_ܡ��o���`�n��J��M"�8����A�����������N�u�����# ޫ�������T��r��e1��޻������mC�Jㄜ�I?�͠�����
�������9|Y�+Ӌٸ��`Ȧ���;E.�V	�t*��9�6�a�K��h�;������ߍR�)�5k4��YK��?^/�>��;�m:{9�����P��X� ���
���� ]�(�W��zv���q��4fj�8l�
=?7%
��E�s`%�+`�c�!�Y�H�RM&U��&*N����b�(*6�Rr�� ���h���T�/�����	��!���&����3�Ɏ���g�L*�t�:n��Uci��kԱ��=����k(�Wpdn;����^���4�w1q�
6�������4=��^��
�>]�P�`���N��:4�7Vy��K�����ݘ-Í�n��ۙ�8Rr{��w٭������X�<y}{�Ԭ%̈́����'˙��i�6���w�EX9��1+�F�dG/dُZn~�~̋����91J�|��Q�h���u�X���D��xi`���J�_�{w��2x����m�.O�Rz�v=pn�S�	N��A#iփ0���v>��:���ƶ�@Ϝ*̫��H��$���b*S��+��H���a7�n�`�<%tvu>=���;�?D��<_L.�Q��q��qf#�gXj�C�Kz��!pr�adA�>���{�/]7}���nr]*�܁\˜8�`����&^�&gLΥ���3�����C�nT�V߉�&�(q?[5����G���U�r��2�I���������e[_�e��_Qn=P�֒���ۈCg00]����j����w6�}d=v�D~��{s�0�f�o�eǩ������L�H��u����T'�_l�����eH\���e�|�L[9�H�fW�A���o�+w�fϯNbu醣.�u�`JW±�ɒ:6��ӳ��Y#�
ZE@��fh���ι�&�{��RzU0�s�ý1z�_ۊ:}r|�:��L�bMY�	+��mϾݜ���r�fx��Κ���l���.�T�,i�Âb���z���� ��l5�-6~�j��(DZ,{J&��|���x����^�k1c���j�J ��+�%`���ܓ��kH���F'��d)BՔ>.�"�%,�3ȫ>w���	�ux[臈��	ז(PP��ݐ�Ǆ�{�x)�D8�d��U�2��e���]"���� �۠`m�ڰ3�8��U��2��l��vP�@��W�#]��s!w�[�g��P�t;�2ؚ�0l����D��d�3W�{���S��L��6��B��w��۾ڰ���� 0�������<alQ�7,ޥ*�K���[�4 ����>�b	Ə����u���7Du�轣�tO�v1�F��Ծ�����XӪ3�ޮ�q�t�͗T(�,���d�_"
a�����>���������]����&�-��m��u�/s�0��}�[�Ǜ<�����!��W�������������n?�G3`���{�:Bۏ;�Q�X�ZG�5j��l��6��?7����;Nw�d���l>(��e��g���?k(����
/�v�!o]�r�f���m�~����c�TT�����W_\��;m;��FGQHL�5��g��ؔ?�`�/�s���/.&糿O�,��`�?dJ��$�hx�[j5v������/�	���c]>>B��3<y
���:�����*�HHigj7������)�li�)p���3��\������]],�f�������e�:+y�������g.�7�7'�؍�#L\ݑ�D�vo}"&J��^?��ATحCBGN��|�=0bg[����D�-s8��V�E������6������`C��6,(���6M+鞀��N��G�&hr����u��#�W�r:�R��󎫷Z����ٙ��Ӥ\��5l|��(� �j���b&�2��0�-Ǯ����˰c�z�+��q4O�l��g�X�I��vK9B�:�d:�nz����'����O^����PX$�S��I;�=�o����|1;��a��&�7�~q���硊��B@�0]��6Yx��@���OoAy��$��t5�{BB���n���Y�×��y{�.£�'�A��U؆��P.?��$n(�?~�a�ڈ��K��J�[���n^��m�*��J�+NL�tgjG��^_3ۀ�%�I~w����+i�O��׭�[�;)[=�N�4f$��^7F�no2�y�`=b�]}�7��&_����o����
g�nuj��w���%2�B9WY�N(n$J!����ͯe���� ���y��8m0]��QZ�r0�10�9�d�ٙ�{�A�d�|Q�f�7Ш2����){#�C�e�5�2��甐7�wX+7�� �~%�jcvs��d��T��9"p����r~��u�xA,�O�(�w��E���,���R�?�6Ч�#ΠӋ�7����&΅e��B ϒ��5�!LiR2���!o�0���^�#�����M��T���Ϝ��5�� qoc�Bu��G��M�"���2����U�T\�d��#6_��ad�}��&d�ﷇn¦
����>D�:Q)鎰���\4(�C�"D���O��OD\ҏ U�+yel�A���ji�z��M �^�)����D;;y�������0���sN[�`�z��/� �-�[�'_��k���~3|r� ��<Ėle���~Ig#�A ̩����9������ ��lx�Ͷ�ⱹ);��Ԓ5���8W8���Mc����`<߫듑j�jٺ��6}�wǯ�@K`@�ƽ�N�r�����D����±��Ccx��E�[��7K4]�n��+��y�ݍHHv��=����Ul���U�J�A��}�'f������K/��Y�&�M%�o�N��tc���]'��<-��k�X���}j�ߑE��#Y���.����@�徧m� �Q"H��Ֆ����6�a���nCE�4�ۈGa����ں��k�T5���A�瓣aӃ�|v4���7Dy��l[4���cI���g��?>��[f��y�4�M7'z��[���b�A��y�8�]������D�Rc3xC�v�� C۴FJ�>�����"��x����|�1<��Q����V)��ߧ���x�����- ۹��`�E\��z��n�F�^���!�r;uK$O���^L.W���ݺ�3���o���ن����~�ϴQ9pNe���AoE�͈/K���Ś��uVh�$�¢�KsI�ZZf�m;�e��d�^���w3 3�ő'�d3]k>n��������[�h�ؿ�/p���2'&ο.p5A��uv5Z�Vq~vv�|�Õ�c�o����3c:;���w�,�ҥ�������<!��r�?P��̟Mf��Q�4L�����T��	���n���Z�Ȯ`�oɺk,��+ɬ[�D�����u���׶��ظ�a����[$#t�#>k��'\�_��ص)��0�^�G��F���[^���������dcG�D�?P�Ыؖ1�ɚ�����v��,�'�,үZkg���p
Q8]�-n�6d�݅m�I�>iE=�n��'y���M,|{ū���""���w��CG��(�錒�:J�%�vF�w�������9^�,B݆ۨ�O�&! �rߢN����N@s�ݼ!w`'.Ve�b~}�T��[,v��	��UA��Q���S^���6��ѽ�ٛ��z�[�E��9_���N�-!c������Q�ӴB���n| 柷��&[���q�f���Ƨ@o�M�F���59������[�ǃw�M��Ni�k��������Z��>A��w�
?�Z�zX��2c�2�nu���	�#�:vSM�4��0K������9o<�q}"��}��/d +�m��^�N-�^?�^2���6�+k	�5���w`8>Y� #O��W��������j~4�<[��UǮozǅ_3is�6p2_o�~IXM5�q5՜v�pɤ�W׈	�d���ѩF8�����b�G�:���Je��6Ȳ�-ݺ���l��AW�$�TN��k�d�H�_D��Ik��7SXk���4����u���)\�O�vr��3Ԥ[g\
ZS���5>��F2մ~ݘ�>a�?3�J����;Q�y��rr���lÏItO��hJ��l������L����'��׋%]1 �	�����s�5�e`��-���ǝ���)4c�4OoJ�&�@�s���)`�z1��]��C�j#�|��9m������.���^��=y���䢶����r���~r��En*B VL�q�mHq����mw��C��5� ,#wn=�l�~GE�)۶9�B���&��X'p���J�^��v!�!�|r�gKb�k��Y�.���4e�n�3�E�S��T��M��
H.����D�6�{�h�6B���+�21l.�E�~A�N�W���̖a#1S�ХO��,(��MW�;����]U�=!Ln!�d;Οϙ���(NЌ�q��A���X�o�65x�k]/�9�X�����tīZL�DH���4Vlף�B��(�_o����_��.Q�#@�b�����q ���:���W~��;�����P�P��y���|����#Q��#x�(A������x�_˼�7������{T�<����m�$�|K�Zۍ����p��m|�UT�V��71?Qf��h�}�Q|w�>�	d(*�亢��L3K�w��_� :,wH-�`z $�M��@��1��]���2q,/&ZoIMl�@z�3[��<�r��o�b\N�0��*$(k�{q�*]�8�� ����Y��旋kRS['���%��L�QZL���t���5���n ���b6��x7Yo`�l"#�n�D|#C^M��h{2�a|# e���/�<ף,"��dy��Ѿ����6��z�c�b��`�r#E����=A[/�������6��H�j׼}�x��*���{�n�@�����@� �����˃�a@�_Tղ�� g��X���tx����VD4�^ce@}�\��n?l`͘Y#��F�U�,5N�)�4���g�&��d�&}����w,yx�w���9�O�֥���M9#̞	�Z��ʍl����sJ���������}�O&����kl_���Z���ն�����z�Yh�x���_��K������ ��\�b �:��
��A�C��V*���(yS�z��[Mݟv�f�k:�p�|6���'���~ #�ȳ�R:1yї��LW�aOt��֑p��֚c����z�8#�g�G�^���IG��ܘzq"2.��m����� ��T, �yW�3��ƈ�җf��Y��x��7����Z�R5�7�N�!����-IU�b�;�P͘���`K��e7?������35е�B�i�Jt�c:a��Rvg���/r�P �]�����B�����fi���q���?�~m��3P���-`Ȓ��燚�p>��_|ߺ�C�6De�tΚ�!��o��P!e x�р�r�B���ڈMU,��g'/C�!Q{��qc������dqۘ�^�@2��dz�M|]0�T��z�r�i�+Yc,��)kU�v%O��+�d:����T�jU�FQYS��t�V����G�}���Wi.C�MtgF�J��4+�R����>�V�^��e��5��㝼1o�Ȼ�Ӎ�1�ل��B���a�eOd�qt�ގ2�'῅����ML<l��]��U����r�ʋ�y";7y;|�As��0���z�]��.�ubm�x���^Ti��x��\����e߸��T�a�^����d�Kd����g�O?�ϧ�o^|�����r�'�<�q`���G��_�G���fy(l�$7GJn��(����\X�*�ݮ��k�v����|?���.X�������`Ut)6$�e��v��.����<B'Rۈ�`���p��f�׍]��g�'f^�iX&��i��-����f������ډLk��~���gz˙��\��@�39�����@oh�Θ!�D�%��A�M�����7���=WNm!�f��	��Mu]H\s��#��UzeA�X!B+��9C\�M�M}_-�kޒ�3��*ZQ��&8��5���D.dL�79�2 ]U�=+�<����/�SV0V��r��J�?\#�	�vzQo���5�	m`*��0��\R���v�_L_3 ���Z$�8P%��� �@�L�:H�!�?�q��� .������f&��D��msf���]WɌg4��ypupҧ��[�Y&���o�+��h ��?���6�f�ם�7�r�ϑ�n���s:�a�0|6������q(&�d�{J�j���SV�s�h�Q<�E��6��Y��="/�9p�_?� 5��)"�y���V�N-��ks���5�����l��s���kF�^ؔ9��t�U�l�z�N��M�j������Osa#�P�h�+=5��l��`j+ƹ�D �A�ɶ"�&�/���-5�L�j��f��*=���f]i�֪c���y(n���m�{ebwg^k�h�S:S$91����(?�`�������*������������ ��x��:��������p��qv�M�vZ�ʒ�<���/&,=|���'�\�J�
�L�m��c�I;3�H;6�������t��V��4f��O�;��4����w7�ⶓ�:n��uܚ؈���Ʋ�i��F펴�_���k�Y�|�+|����z��Ke7��֍_���̑ݯ�ã�K��7�<�!	��w��${�>�60�eΐ=;�������������-}������=�+}t�w���a}~ݦUau�ɶ�v�:V�Vxt�c������X��'88ϮD�龿}L����^�fnn2xk/ԇ0~XؾP���]�����_�L͂��N�]d�!;x߹��7���U ;��nuo�]��+�����F��ٮ��-i�'�qNϹY>�ؔ��2w]gwo�f��٢�Qg�ݞێ�;�����m��a��}�u
������ð;G�na>GZa������#��,�
y��Kԯ��6������<�������N�����ACBݡ��i�k�6͚Y�c��S<ղkk��]I�`��S�����垙�􀎠��xAñKOn��zH��Gk�\-����:�������c�����L�`b�{L:�Iϼ���zAПuGӎ�%en�n�bu]���v.�~����❃�w<Mw�4=�Y5���ͨ��`Ax��Ue�=+���������Zw�S눓�� �&|��A3��>�h-��n�c�D������wd"�K�iv�|��S�c�׷7��:]p��c�h}Tk�@g?:�Ϟ??�	�����+����#����1n��7��g�$-���0H[޺4ݕ9�����X����ۖ�����lN��<����\�^豒��`��vf9E2og�܈ۦ��Jd�	�x3]�eoU;�����u����,|~�������9�t0 9^���LB9����n��c��:@,� �J��Σ�T�d8����ur���e��p���3�"���N;�^�	����N��@��m:�W�H�o��@�P<� ��it�r�־���̆�Rv�}���8�������P��^�-Ǔhˁ7�g;�㘴5:Zj���.ϼ��� ��w$Y�Tg5C��;k��mh�
��^�ސ���mh�|�xwP���켾���PV�m�������v���N���D-���Kx�6��U#��㵥����[��O_�d(�G����b�ZȽ�������N#��R�@�c��骵�������4��P(�vF��Ƀgf���H&�.ȏ���{y$�{C��UtR����a��ֳ�:@ݡY��%�z���0SOޕ������As�*FM>��P<��kw��LW!w�w�۸w�\B-���(���M4M\��������׆�@�����[�ꍿ���v�ke��ͣ���f�f����GG�|+�H��%ơ�3Cd&/Wi����|v���o2	E��3�mj���Wyn��H��]��0�:�Ξ�U�n_��k��p��ۛ��������n���L�r)]��t�� �s�=k~;��eL�ɼ�5s$�5�_�N�qS8ɼ#.�c�Gϱ�_�b!v>\����M�Kg��x;�5��֍= "�c$30o�E����^��w٦�������D�.i4�o��ZO</>p��|t�h�W(.���;F�R��%�~~�}ԥ�~�lg5�onIR��P8ϟ]_��fLS3۝�z���)��,��<�!���ۺ��R�_��B��$���;������A��
pu���~ !�ǖ�غCs��Ii�v�XA|A@�m�f����Ⱦ�_v7�ʶ�H��	%J�.v3��1U5Zb3�� ]����;1�t�pj��ܜ�$��x��tED���N�w�ʥ��ƕK����`w"	�5���K��<�y�:;��b]������|4��vA�c�oZ����/SQ�?���k�n��_�'��?�z�U�����4�i�
h����6�.n��0��)�rL�BW�c�̡����Kh���. '� }tyZ*���K�. ������r�����v���s����Mr!��嵈 ��m�{/�wdI��aʨ���eO�p��L����}�|���ȿ�_��=��&���U������8~�wX���`����5����h�t�L/P��վrJ�W��7�-�d�%��d��&�@q|� /2�AK=����s�#�۩���O���*Q��K��<W����b�&�)rǈm�>�i���}b����!��ӵ q�ўۮ�j	���5D/p���h	���i���M�������6������p PѠ�|��`�~Գ�oy`��ЛuH�^-j⮞ى��?�G�]���I0ߚ��Х+���\MY��Z�G}���h��N�m��ǹ�6�`6���U���M�C��;OKE`��\���s((�R ƈ��S=�������wM߽a�!<���*~���+���,�'�����H�O���<A���f������u���eS$�9��8��?��+��z�dH�_���6�@��R)S�ۯ^���d����[�=��?Y̮��$�!���(��Yqx# )��G�l��n;����F!U�"]�H����S:
�1/4��1�|�������n�B���2G�p�������.��gd�}O���]��>�3�mr�Q����?�dcp�P��ۭP���؁?�=���r"���6|�N*�~���Zz��R��v�fl��cC�������G"�u���^l�t����#A�xg3�c�Eq �s�L4&,L�Uk�A��i|_m��\A��:*l0����n�6i�$l�Ey�����>.���oOҴd�ݝ'_��m�6�mS�m�Yv����Pr���9�pc~.�᰻���V_PSA�S����(^��W�����U��8Z��5�d�QG	���k����p�Y�F�xɡ�w�KW�k��O�1�h1=z$��ޅLN���\W�kbG�1�ͧ�>Ǥp؎(����*��<	��vùp�N�c{��B��@�)���FV�壭bԺ�D�9a�n'����p�D��]Mo��$�N��6�~��5�����E�>��ۨ����ΑF��̴d�/^��0x�4��tSLe�wx�~t��LU3�2��d!�d=���(�Ʃ6�öO\�Fiw�*��֓=�V��������^�\�����-��թ�
N�x����/���3� ��F�k�ވo�����]a��`�Y�<�Hs���2Ƴa ��2G;=ӈ��y�~���h�2=q2ۂ]?7$����gN�nto�[�Ҋ_�;�hc��Gr=��S��>9_��7/a�vq��:���E/<��8¡'����qB��WM���* �l��P�k���v���iɥ��z�Z`���%�PoJN�1�M������k��mT^t0�G4��t_�o���Ã�C��r��V��N]�=%W/���΂B�=>��vK�m�r��V8o���㻮�tu/�"�H�XW?���;��8��ZU��;�v~���"XCf�����c��A�`F�`F�+C����	�Y�ml9ys�Mr[��:��wg���n׼3���	�8-/�����g���V�LS���t��	B2�5�]��S���?��=�����Anl�`�$_v���w��8�� \wݱ���ߧ��(]B�	?;���fʸ40��1�S�{�C�z첼��ZB��l��R�\a3l9bQֆ�(�N���Y��;O�Γ���-�+ڞ+z������쓵�g���{��CHt���e'Cy�ˏ{��'�?���uyi�v��P�������g��=F�+#hN�Y;@wݢջ<݇�F���j1�L��-Ɠ�oAVY�ԥ�~y��G[�Yr;�mmW���_�e�b����%S�a���������^��V:qu d��䉤�k?��Γ,��.��2����6����b�ڐ��A�bnTP�}W|u�(���y�¾���\Ӿ��^ñ�Չ��~}8���?SԄy����V6�Ʃ�U��<�\�z_�o�a��YC��t"V/��������Kc�y����X���\���S�7��n�i��S�֢(�$s��m��i����ڰ���N�j%,htz��o�:����ϐD�"�(H�#����E0I��"D*fb��3W6T��"_N_#�O{s�l���8�:p����|�����������ᖆ��\�w<n�n<�8Ƨ���=���J���_�
�C:����+���ߕ����*�W�\����&��z[fQ�ew�3� ���9��["�bjy!L�׈��8�_oyq�R��t�O�{5=�$}��z5��#|^ϖ/4�q�ŉn�i׹t�O�������+��o�
ؓم�/� �|9UO�����������Lq���0��)5?�m"�A�1uP����)F��`��ۛϓ͙����&�9��N�S�yͣe˛���;�6�}d���:&��~��]HA�ǋ�j��;��	k��kV+���ӧ��\�qt�|#�ߊ��.�'���`e}6	�1�'w���Q��X���F~g�� ������
��L�W��w]�{fd��O%�J���C3] �n��=���D��7�|5i�.�V3v�D�x��4GZ�zG��i��!�{��;gs�Y�$��X�N��=�S!`}��v��d%㐼��7�l(�����&�Z��GՈ7G'���.�X<Uh������_]��=?^LO^� ��M���ܥCy���V~��{�~>����1v�����j�z�^͕fEw:�j�ɪ;�v�8�LY>��
T�Z��QH�ڧ�y���h�@
k���DJ�)�`1�&/�jA[�PD�� m�״v����æ�����.�x��U��	Vh}���M-z����T��K��2$��=U�mOD����c��A+fͩ��O��z�`��`�y�٨+���Q��΢h����=������H��`����� gE�|Ʒ��oO:�� ��n/mnPK�[B&�/���Z4�ƹp.b�g]^�N��� ���<��	�ܚ��R�����_�UC�i0Ym�X<�
qj����@����K"n7���?��.�ap#P�ݻ`�b��Y�����{j4�֯��W6Bu����ƽ}�gr�յ�&�&�ĵ�wO̲�����fX�0��x�:sɥ�
�Ζ�.*�k�����ɧ�~W��h�b����cf:�	��iUL=ic30�c]=�����žp}�E�6�$�'e9��/�u�c����E���#t�ם��A�iȋ1���.�������)O���U�:�.}����Mf��_�a|�"B��цL�iɑ��b:�ls(��lǊ���nhs�S��l�n���V�[�oc�+���Nu'2��쥗�@��)r,s���k�mi	�*�<;�Ý-�&����VgE�����
a����Q^�0�Qju��l��v~�\�C-���_OY(��-���	"���~��X!�Y�Nh]��l+ddc]ڞ\���N�.�/J��m�wK����U]��<����ll+x��E�eM��1�ϟ�̏���>&kةo�[��Y�M�p�' ;ފr��t�m=1�4ꌟmQ��^���;�a�Uym��J[g��$,��ً�h��%�jknJ�.���p���?˶rѰ4H+�?_�D���8�f�� k$D�K+�[�/�;8 �f�������|�|��������J�=�y��l�DM�_~�<����{vdg���k�ߍ�l��G�"�����fMQJ�āUJ��d�e*;U(�Z�J��X��x藨�*Ȩ��n��6��c��㗑���_��m��	�Rcj�x,g�89ӝ��N<αj=�௦�&���ǧח᧟��˫��b+i�~<�h2���,��jϏ+7���y��T��dL��N����h<�9Xc�lI��n�Q�T�����(w�Ý����0�	�|2|��\t����	�%]I�pZ�N���~8��q�� +�`ȫ�0�dj�VZ�e>En�ӱ��qL���]��L'�@�kK������ۊFB=_�6JVU�˰���4Ҫ9�c�,g��
�F��P+JzE�:$��*�M��Ӯ�窍d�J"�_A"�o����ҧF��]+��k��6#�\��zu~��������7k�hv��+֌��F�$:�C7��F`��mߥ��)k(��p���aw}|��{�//R�����kT?q���.a	[�ޣ�u�����x��nrZ�I��
��\�1pN:mMm�z��2�@�*�6�C�S�G6))����|����mԾ:9���~eGwvY[ّ��py��(n|�)���
.oM�R�<����g�s3-��-�Z�d�I9��tV������&�3k�`�S�W����=�\/4Mn�q�/�CQ��v���F�zH�<S��N�=��������������04p-4�s�,�K�d�PU���
4~��7��2
I��s6�&����y��	\������1��m���ŋ�����Jn�D�WG���X��L�bzx'm�_'.o��O�L)�<�����~��7a�&�-�����ÌH�<��T}.�E�0[Or.�S�wW��S���k�f<��ɍ�3�U�!b�g_�Tf���C�^��C|4���Z�@hQ���j}.zh�_j;���u�@
��⸉��/4��G�皫�@�x�\{@�~��;���F�j) Y�n���v�4���iz�������b`�B���[�l��Wk�d���)��0����H7D����u�P��(�r�I�j�,E�?s�y�F�۠�k�w�����Y��G��ѓm��&�Ӟ���1O� ��0<0��},��^���+�g���J���ʯ�nʛ{�5���p�*p��k�8{g\������꺳����&���3��-ͽ�tҎ��O'S�ঢ়��xa'}܅�д1D$�m�`7�΋�G �p�����Iv}���5�o�a��M��#�iV޶�fM�M�GsF��̟���gKwZy��2��p����V�뾢y��r$���Vl1���R�*����&�݃�AK��ԉZΦ�m��q!$���H+U�%G������g�D;����4A�&��3��4��l���������Y�m܊��6�"���\8f�Q��F%h�����h�^�~ӥ;��!���^h�\X�y��񘳅	��ƄW#<�xvNiz���|LZށ�[ʝ��]%��P�we(A��lP�^�����)]?�\^ͼ ]�M��$���jw���g*��̜��\��|�j�{���yYD�L<��i��[6>r��=��Z@h�DF��=s$ԏ�� w_�T��3�ؐ�%�No����ϥ9��ء���l}SPO��T�r�ʍ��0� 0q�T��m �M�����(vtЋ\����*�SA��t����ّ��6!���g�`!�L7N�z�N���6�j,J��ƍgϗ�?5V]���0hn5r��f{�y�Γǉ�^�if$q�d�#U`Uǳ�W_�.|��n����nQW�4�tד�lԗq��f�'E���|��O6␑���>��|�c�ڃ�D�:vګoo`�Hd�W��k�a�_��@AN�f�'�e��q�l��4�ΐ\�����g�����:��7�E�ϙE����Q���(�9�h�
��
P/BUzk^l}�s-����F,ia%Z�;���&�v9�\���7���o�˕�bs�&�t*g�&�����i��p̪�zܬZ��4P�����ůwR�dGdE�GV��C���vKQ�u��� ˩�l̠��AYoN�F�R��o �X�ή���!a�j���h_��Q��Q���s�|jޤam_��F��k�zqk~4����5dlBn�>u�իj��,`��d��[����I����}Z?�SH��a�*x�|Zѩ������)M�m�Q��qZ�$A��LQ��_�?�r�P�.��.��?�b�<o=;"�Hp�4C<tb/��ݞ���:m���k�K[���:�sd6h�s1���r��$M.�Q'n*��,�e�\y�Y��F��X��c'����s�f��y���b�o�/"x [�[�W��Y��Z!}�z���3Z��c��P���:H�sOmx`��������o�����)���9����Y��F�z3���6*k��[����/Z2)��6���_�B:�IX]rNZ��Y�뿄�;����j����Tã6�ة��iH�Y�yn��w��W�@�b�Jv�9ɜ���8�}~�*,<�� ��\��<s��Nc��	��/;�֧�Mx|�FV/�Y[/�׆�#�x~~
�B��aS����{+�nٓ@��{�y�e��|�*�m)����j� 1.����_����}�V�h��<B�/m7V�`9?[!ϕ���tq�%�c��C���Z*C�v�q��7JyV�BO�U���'ڤ���k9��Rm�l�h/��A�0m��������ݹ��t.���1d�W������Nx�PglA��ɪSal1��|�Λ*�����v�\�<��$�<��:��n������ÿ�������;�;�,���K�����Z���tdϿ_~��G������_;�p��6~!��60�&�e��M�ԓ)(7~�*���7ʡ��mYgخ����.*M{A���LT�Ʌ�����m
����d���ZQ�5r��`�<�=�^����jC|>{�$����$I�p~n�M�׶��G���XW�}�q�4%SB�c����K��Y��T��X���ݗ{�,�j�+[t����0s���g�d�-�g<�.�~i�Ѕ�2*W�Ǵ�W8]kW~�<�!eA.����������;�����*��نY�����7���|�)�X��L�w�+fx�>�C�ۋ&��i%X���i�dk�'��;�c՟�� �#�0ٱS�D���%�.�y�%�k����O��+���e��y�B����G�r�M4��Oþ(�~I�ud�M3��,x��99>=^L�d���~�sh������̮�7m-��Vb�7Z�����k��������td=�ӗ=v��&�~�\���ц��kͫn"<[� [}՞6K�;�ä4��5�F�mkhمG���j���L묛�{.��ݥ�N�c�wLc�ƚ�;����n���~��(~>pg6c�*!�kN];}�s $O)�G�Bܮ��V��v?�(j���G��]�NKƷ[|��/���������U�c׎ϧ(0��;h&�Y(�{2�eg�_>G8O�#����N�g`�@�������=�����̻�4�Q���կK����c��}������R�ع�?�*�ي#�d|�����{%��~� >^/	�G�&;��h^Ù[W4����K~Q��h�`l�#���3eYMGѻ7�1HH��Ԛ0��NZY�'k��M]�${tk�Z뭇4�: QՊ�N�:�'i1����e�\�$�p������Ӵ������A��.�1��c���1\ۺ}o��Dܰ� b�^�ὤ��Q�����/k��0��&q(\{����>�8���ݗ`|/y����Ys-!�O=��{;i)�G �O�����d?<]+L������o��t�gŴ?��N�?��|v�k'��y־v��5}����&���I���ߺ�}�H�X�P-�hM�6I�'�<�E��<�x49�wQo�㿆bw�;�fiޥ�)�P*i�o�?�U�I`s3���ZK��[�v��^�����;[JbR�?���=m,�B���d!��Bo��NMg_b^�7!���d���dO�h�l>����,&�&���
92kC�ӱ|�������ιw���߭��9��x��!���I��I�,V��tz��ܰ�Z��	j& E9��@9�K;�a���#�R��=EF��\�==g^A��'�hfz���{W�5�0�^NϮϽ8�����P�~�g/��I|~�E���,����7ca}��t�8y� ⱨ �Ջ7�7uf8;��|�H���O�ß�C����~�����z2���Dn�����g�?��
��{�+��ARAٓ�/a5�TO�p�υ]#y�2�.-�6�.��������̑?�>�������,���p7��r/��:����ǣ��+���|-Ƴ�˿�z�4��e��Ga���O��}����%�t'"2��G�����g�B�`~��rr1;��������'��t8I�é��*I�o�����{#���[n�m�g�ӯ&"D����O�C��'�gٔß������ ��Y��ww��-�sڿ1t���j%�n<T�����`��x~���}��O"z,_L^�E}2��<>����Px��Yk;�&"b4���ȶ���H�P��Q��}3Y�e���ӫ����:��"�.��%��l�z�R8�,�P~!�_�>;���ß��Y����ܮ��Zi�N�'��W<�iy���(q��D�.*���q��igܣ��O/?�Ƿ��ß���!M'�!Ș?�5;a�g/l���tL���\y�M-2˧[5?M�!��B��!j�}z9�t.��O��2�X��>�X�����&��_[��H�0e�O:��f�@�6����d�N멢gz��ue��l`�QgO'�<8{�����������O�p0?�`�rη���zq��Ap'�I�����#a�����X�N^6����>�hH���e�iQY
i'G3���S���_����D=p�^/CP�p���/��ޅ�����Bp�Z$�9�/�P%;ԮʓCtޗ�8>��V:���at���,��A ��#c�AXF�����N_�f���8/�����ny/v��IY���"n�?�b���AJ0�ӥ��p�X산i�������Z���i^��l�**��k�b��#nv��\����^��@�;%���p�ۍ1utE�x	��(ʶ��4ɺ��O����
���X8.���<'�{Vӭ!�:�L�:��^ޠiTgQo#�2���z�Ϧo���Fx����3���BT֠�����Ã�����~`���9�5��OFO{]�Q�sHey�1�4����2��&����I�VE�57���6��ç����4�㍈d����Z�&d-���峉�1�\>��Z5��409���}�]T����W��.�f$l�)�ɒ����蒷��w�BI��'�F}���R�����<8A��7k��5o
�<�j���K���>����b������������y����j�O�C0&*��_�b&I���\��7*��H�%��"*"a�����Q�/a�OS��k��qu
�zO?�;F�����~�ų����xz�F�{�SDg|���]-����B��7�}@K�ç�Sƒ��L�g���kk���W�����ЀJZ�{_L�O���]�Va!l��?r���;B��?�2L�(�D���fty:�_�-����>��ٟ��h��p���ׇ�����d~�g����������uF�׾6s1�+�;��=.�h���ZA��z&��D���/(�yu������a\~Y�i����0�g�Շ�J��Ca��{��wÙ�B�C�p@f�n�V��s�o��G��c�����G�n�w��_n�����nN����WOoh�D �<�-ϗ���\8���^�C�e�����w��\nz�\����zYG7��}�/ݿAk7�D��N�v����l�~� 
�oO既��=t�tJ�*�����i���a�d������U���:�7��u{��s`/qn�T����S�{�o[u_�����]|��$y,f?�'����_7=���Z^ÄF� [qx�����V�9���g��7��v9��d���,kp5��m[-�e�dO�������l:=�a����򨽭�
������l��y�?�"���6Y}�rE�_��m���q��M�{ѷ�?�����}:ҿ'�����&��<�J?//<�G�����7W�x�9|�Kuv�Z�h��0���C����TG������Q&_	&��Q�zv~:x1Y����.dmF�'s�;1��YѺw��l��ͫ3��6	ؘ ����J����S���U���Y�������\�h�H����X^<=[�0୿�;���(�? Y�\�~0���_��^���1�f��G��7zx>�|.�pN�y>���G�{�ُ7qR����=�_����y�<������鏝�b���>Z�^>�]¥��+'/q��@Q�s w����k�x�N����������zz���4���\����0��G^?k ��8�_BYd���(?
��ބ��~�� (��:AH����L�iy o]Zt88�囀��	�,�bf��NM>*�^�@t}���M��p��mᵿ��׷7%���~z1Y���'Lu*K��͍�)ma�ϯ����}���b~*����uE��LOn���?�����Q�G� ~���������Ƴv��V���ẽ��%4 CO_I��6;���8Ȝ/_Xˉ�F�I��h |�&y�~'yv{�jbRx =�&��E�6J��Mc�b��`���Z�L�wt��፵n�-���/�~t�l���W����lv~�$4�mm�K��줵� DO��u�40*�؇@���77���&�y�^��cnH����{��d�������\�MmûQ`�MCt�h���B�K�q$�8H�No������>4�yt���R�o�//[* �������g!)�|�[�g�f�?�����t�x�s����ӛ��9��������tA6+?^��/C��x���ڣg��$f��*"��\�_MW�G
���e��&�"C��E��ї��x�'�dh��X��Me��¨H�z���3�z���@���7A���7�xBx}��/��,_X�G"�����I^(��UJ|�8��� ´�8���@����_�}0�"/���,؍�l��T��/����n0W������G��\؍t�P��?��?}�?�@x��G���ɭ���_�?���V3!ݬ�ZЕx@�����lyu>y�����/_��O�F�⑨{��4�뚱����G
.*G�Tƨ�@�gaθ㈝�ᭉ�z3����9��������r�(�˔e��?`o�h-�
�;�u��!�\�B��-l[2`��[��S�Wd�C�a�^+B����}AQ0��.p0N?�` ���T�8�AJގD�鍶Q�e( ��{v�/��y鳛g�U�O �&���qrs����ś��ӛ��gУp��&��"�����}�o7���m�������U(����\���%�	����R &ԫ����r��n )��G��Y�v�F����&ri��Ϟ�|���n��z����AG��:Ϋ�}�VQ]!	Ia�����^��p��+���Ixr��DD�E+��ܲZ$���� ���q$����dUV�#��.G���F�������8�UVrS>��Q4��8��*%WrOt�r�Q�|�y\E� ��b����r ��<�F�o�����A2,��~��!��a8
�HkS�6�c����Me�ǲi�H2�8�����xP��\�dPe�G�� ��^�g2/�w������Y ���A/���,U*�W�dXː+{-����QjK���߱���A�1����Jq2��^���*�F�tߓ6�/K�A�C�~�$��$�[���QOVk�Kb��7�x�:�u���#�.q=��1��(��?�D��o��[�����'�d���]������Xe2�qp�a�dd2�Q2�ƹZv�����l(+?���\�d��,�*����Tq&0���R^.I���ļ�D�C���/�
� 3��`5��@np����iB��h0������E�/| �D���<&�Gq �Y�ys��=ie<�e��j,���@9��I��8.��R�D�0X=��� �v��R�2Gu���j<���,��!����Q��YU{c��~����M�+��8��.0��\G��|ȋ���C!,�s]�\�e�+2�e����Q!(�ϥi���YZ@|��,��<��B5%t�K�Q?�>�L�n��������l �X�]�e����E|���r�Y\�Y�W��_A��͉!��r��u��qU�J�a4��H�x�y�J���\C��ќL;CcY+�_���F�z�A&�dl&�f@H�|���������	���K�UY)��(҃z��G�BVXw69��a3IiX-��'E��}�?�,��i��8$��c�>�S4�K�� �B��o���c�������w<�u걉~��fȨd��R���(��q�� ��#ޑ-�F�Ͳ��X6|��2�J0�^��*�as��(���f����,8��}LB@2�e�;�?��<��~Q�W� �X�^ H��� ���u��Ej�i���	���Q�+b\g}�F]���Q,ĭ���U`�!Q��
63���X���l�7#iK�l`FC�X�O����F��y��t"��F�qL4L��`|��U���
��.�W�7��%�b2�����ƃ^� �Q�/�2�0+t���P�?��B8Q*C>9��HȲ�M �#Gq��ɁG�#��i:Q�x��;"����G�r�` �|)wULƪȕ�Ni�,N���x������b����F�e��Ԯ!=F���y��郘��R���hݝ ֗�^&�I*���ˀ���$hO�2L�9�dT��@6���D9��1�L�b�	���?|�o�H� "+��)������h,)���x��@�e�d�CPq� ��8�(#,`�!���gX�r\�I�e�e�0�b��
R����6�����E
�4����a��$���	 ��,�/�G,��JЧ�qI�Ѡ�4��
��HF�H�)��KpiY�B�o��Ր2I� ���$����H$���#3B�0�Wz������!j@��4���)�� 9�@���&�Tw�-��*���&���^ �w����"A� �Q�(�H���q`'�
"\�oDւh�Q�r%�����!D֕�ĸ�yDŶ��@!l��F"�1�4��N"a��0׏+B�+��l��u��1=]@���)�p@������W Hḧ́�d)Y��*E<��<P�d�����F���m��@^N!zbjȪu�rU`��`�)�W��_A��
6&���c�B꡷�q���r9T�(/�7CjW���\�:�_���p��d�B��@EH2�QKxFx�$���@x!����g��5�K�Zc8� h	�F;�k�(��_�^�T�q	Ѳ d�n�FG +�;"�|M?���uE� �����m4�7������ YY��}9� (� �<��r�C���ʋj��c� j��YQ���*o�G j)��TʢҶr%����\]J�|���X�p*!��'�^���"���b��:��$�NY����x)hB�'�m�M�tH���1���!`l-P	z��+R]���+zoY��GjZ欜&rX+4$U^q����5��X��T��W��| RR�h(�Ĥ."Y��N!�F"c���]U�G��� �����( ��`O	RȀlO�}>�Ez�$X�ұ	I� "�A�����ݧ��j����C�5U��=9�fX��^�o�U���R)�>@<��8gљ I^n�l��WFԦ�Ģp�mQk�B�z����"aC���bT�BCɩH�C�\�cҎPnX���� O����ػ@�"9�!Yky�yoT��1�9$uz`<�䁐9/D���Jb
����,�C�I��d5U1$�F���j���M��D7j�����:��w�.0�� @U�m��l��� ��@��h%�m{=0N�����g�v��~�2`6)���k"���7�+��}�'���誸(�Uy����ITՖF�ݤ{Jt�!Ω� �X@�H%����F��JoU" =�n�ު�@�8�څ��+ZN��7!(A���N��Y����o�� ����F_���|�܅0=������x:A�����z�!��W��]�a]W�ų����^f6`׎�j�a�#s<�
�,�4)���W��?����D��h�*��~�?����U�&U��I���T.����p��M!�M`/⛤LK�&)�r��Ҿ዁}�e��$+7���o�b�o���o�r����F_�o��O�a\U�'vo٣vŰf��J�4Kkk���ƛq�5k%@�f[��7dfq�������ܵ6�4]k#�]�]�F����I�ko�Cm#pm����͜dm�A�M�	�)qKg&kм�-��#�\��n������^�pGV��p|�{�W�ǻ��{?���ey�o��<��y^I����s�X6�?w_Yg�t��2�R��(k ���rͦ�O]�I�ea�i���KJ�G\y�f��^R�� ��{gܒ4¦�i�`�0��f9�8��77�YG��׷�eM`�CXhpW�/�1/�E������\f�쭶��]�,�*�m���o�G�*�VI��%GSb`�L����m&\ު��&,a����8ںr�\՘Y�!�`�˜��|�45+V�B���j ��bY_vQ'	~W|���楴P��7��_i���3^��1섴�ϲ
�X�ˏƛ"X����R>+1Hi܍�H�#��Ĭ���i��۠Y�g�ռFhc5�.��G0V�g0� "�0�8]��$��r� ��a�a��O���)�rr	֧�@����=���^s�Ze��S��7�r�`�=̼^+�ʽ��:g�`�ҧ��Wz3������c�U ��b��ܨ0J{X�]��*w⊟��G��u%w>m���U���L`� M��w�׷�Wh?��9��o�wRk_���h�{,Gk�׾�������s}��/���N��?���
�p��m��S��s�%�6����	�_z[�r��O9�:
���N����'�CCk��l�aw2�}�_���c����}�1>m���e��>FX3~��M�����1?)����ڂ9���Y�}�
��M�v'jǟ�-�
ǟy��wRo�3�?#�d-x]�>�d�������F��O����������Eдow�}����m�i�X�����'��s��J����(<m�/8~������v�zG�F�~��+��0��}����U`���|�p���;I;�������,�׾������e�د�Mo�N��o��'	�[��$Iݶ_b�xڶ����ѦE�_v���O2���h���/�㍿����TmD%>��8��㧬,�T;~�S��Uq�
oG[x�ow<��8~����-���;������ȹ)����N鍿��+�Fq��V�����?E�=!	l���ko�k������4JZ��<u��Q�;X��Z���ܝ�~*�II��`�.���N�m�J���n���m���x8�4����!�qJ�'!�ME�iڷ;-���XFH�L�Ӭ�_w��_%gi�J�m�<���>��4���ڐ�4�s�y��	�oJ�L�m�"o���i�W����h˸�/�Sx�K��R�N�mӲ�ϸ�i�>�_�x8ZHQn�v��_	�oZq<��i�ީ���ߔ�3!�M=���x듂e��:�,ʽ����>���T�_��Y{��N���os<�M{�C���M�俙�3�m��~�;�dX�L���6K���N���o��Ln�����;�6���f
���0#4��;~��fǓ�}���_��Y��'��ro�펷�9�WF�0!��
o���'&��Uń�6+���;����f�Ϣc5<����f}N�3����6�����G����O-"!�ͪ��/���?�oFm3!��jo�KBT��'	�oFU#!��jo��N˿��\���6������+!�ͩ&䶹�zǇ�*��"S�Z�[���x�O��S�H�m	b�}���s���j�'�����i�>�O�6!��S�쎷�5�qj�	�m�z���x�E��g\Or[��k�D�i�>�O�$!��}��w�V�J�s����y����i�Ô�7������E+��;-��)#,2���m��N�)�o^������e굯w��9~�_)_����9~O�JU"�H�ms�m���NKR��9����6�Z�������km�����	��m�������"*�?����R�߂����~�;-~����+%�-<��;~�	�WA�J��ܝ�S�߂������>�x�����_eR����jF|���Y3g	DP(-��h��B|qX�g�X� �T�9��j��n���[��%5�/����w�qI{^�K�V��ucʃҌ�Ec�Skb����D�.oz���JZ�pY:�\a��9�����9��E�<��(i��ɚ:{EKZ±��J�:i�u��V�6#����*�����X_g�8Sg|�ƩL�͜AN�J>��]��6��f9RW�Vܪ���bf}S�h�wk��ti8k.�Z�|B3)���0����8~��V�lM#�%{P1�j]5fպ��1B���0�Ե~Fk�~V�ʂK�V�g�V�e��:��D�/it�gq��9\����X��Q���ট���=7��`_�un�j\��5������Xʥ��V~�t���]љT����
�0RSl��R�m���NcU�p���!G�2~[P��g�-���[����\?Co�~��hϯ3�F#~MzA��a3�
]�Zm�iHi3"| DE���K>)�!+��#Cڌh��stE�8�KZ���G
*�DF
*p�D
*9&����Gp�HA�G�"2X��qA3;�U�^;f�6}�gb��C�c��������
5�G
5\�>���<i�ӥ�Հ�5N�(�������K�
�-V S��*LL�.A X�b ����
���6�������n�f���=�X���jXWc�_���%zSX�Y�> �t ���E��FW
SPcr��3�!�K����������:U)�3��h��h��v
5��T��4�Y;��Ui;1��d@bP� ��/!/ɐk�B#����vb Փ ���N	]�ځ�H�Vm�P]-�������.m�b���ߵ>�Bg%��͡R�Ő��R��i%�遶$ꁈ��&�������	,��Lj1������K����F�4&Iui�&^��TǖE�$�5�Zj��@h�T��k�5k�r�@k���B�����k-� �r�����81h$-���>ՂM�G��\As�\�D'Q�G���wd')t�jiԹ��$�j����B�,ho�6A{�B�,Z�c$��T�k��MП�P (Q/	�'r]�/�QxJ�.����D⥃���H���D��QiVI^�OP���k�@Z��E�]���*n,� �r]�/Z��A�R��Gt�E�Nᬒr-Rm��J-���a}Ա�h��.!I��	�m�1�*j��N�g�M�RƁ��Sj�PWj��5�$�F�>g��k��(��z*���)Uo��xM�&�1x�Y0�����fٴ�k�l��N�x vd��N�$ʹ}���4_�3Z9�W������7�6K�c��O]��R�a������I[��`���iN��Om;��S�}JwPlD�u�	��$�1�SZ�z�>��;`�r�mB�Q+h��B���*��=�u���W��R�	�p}ɵ��)U\�A��R��h��1gB��������6�@�R�唢�7`���i1��ц�m��W�Ӓ����S�NՈ�k�Uq-�i7���"�U�����}X�"k�ͪ*`�ФH׾0+�\k����>��,��!e��1�Sk��OYl��ªk�k�S�8鞁>e�mm�@��X�	�	�Y^�ƪm�>e�}�>7���*���3�M�an2�*��A�2�M���ڃ>eʿ )�e6��P��}�L��fk�y�A�2�SЧ�p��MV���e��\����:u�c1$
�n��)�HO���r�Ч�
 ۝�q���:	h��5�P����R��N�k�Mq�j���Ed���~��A,�͖װ*�BD�k��)S\��3S�Mb�߲/ЧLq��\k_q��tj����u���P�vu� ��o��S�8�@/�o!�����Y�c�9�$�k���$	�S�x�G�u�@��*'j�����`�G������Wq<}��!�u�}���"/"���6`������p_6���1`�@����O	��\���fA������W��:E��~Żq@�8���*��D�y{�q�����n���%i�֎��^�������B��$�˖�N��J�ɗU�;�1�'��G�m�ћ�z�!���.l�K����s��t��K�����)3�EFs��٤��Rw�^
U�����Xy��Tsj�O���뤯B�ja�C�Mr ��Ar *X�-�Fi���r�zeKh��g4d��x䡪�/��D+�Xx^��@V��:@%ka��r��j�̀���Pm�KeɏY�lY�l��6na�A��6��W�q��ڴ�GȪ͖?�U���Hɓx���T�%I����ѹ�6��j�\���6�aȪ�r�j����������q���d�D���0ϼ7���ι	���㏶ڤ/��[��#Ͽ�Y��T�V�!�Ԝau*��p��שy#_��]�f�)�܃$�����h��m�.�%��n�T]a��K%
u�'�)9ճ�U���8~y��I&A��dR���	���6CVm��J�N�F��;t�.�#���u�����S��?ʄn*��϶i푓N�m��poȫ]�T�V��U:�PK[Xyn<WW��O�dU�x�N�յ�U�m���>@�ma�2i��Jm	la���KVA�ma���KnA���=��y��6�������}|�<�/�h���i+Oț]2��M�)O�!��c�ֶ�����%�h �'[��͒�0��.��V]y#!��*�R�8A�%��궰����%�p�O�e����!PyyY�x���m �h�,�}=������l�����re�lu�|x�	_�VF�=Pw[xSu�|ʐ%����0��>��%�2��.�շ�e���K>A�v��H_�)Cf�ҁ���pY��t@����m �8���~sC�ma�	9�K6A�ma�	ٰK65շ�Q�	�o�2�a�n�!v�F�v�+�0T�V]!v�'��-�|i�.��Tߖ��S���I}z]����E��h��W]9�%�2��d�v�&��b�͙�y/ٔ9�%�2��t'0��M{�"�DK�"ٔiT��Q�\/����.+�p������V���E��ק˸��]$�h��p�+�wў	*l+O��"�u���'�t�lʼ��l�tO�E`���d-K�d�Z�+0�p[�⬥H6e�I�ʼ��ۓr���|-ґh��£N���֪4��l��d�_)�E<iI6Ak�Ma�+����Ş8�>-�MPS[�u�уdӆ�X2��FcJ�&��-���r�NPC�3�a8����E��<i�-Y���{�3���M4x(�M�-%�6��r�q�(�i�S$�6�J6A��9�LS��6��d���|]�^'̳"9$���y/��Y�\�JH�&�i�+���zSk̭b�\̧"Y���UW�'�&x����J� ɦ�sH�i��l��Y��y�=m����y#����Rޠ{ɥ�sEr	>9-�<9W$�6�M�".:��8W�7A�ja���A:���d�(_ow��!/ \��m����Q.�%-T�%�K-NK˚s�J.A5jaY%cNT�%�@-L}��
Ur	jL�Oʗ%��ⴽ���xB�c�L��<��Tɥc�[T�{剱_�3AEia���ho2:bu�\����O�����j_G�/�{�fT�LX^[Xy���J.Amha��u�Jg�z@s�G[q�D�5 V�%,�-�����i9z�߬ҏhs�p/#�oͶG�Im�^�=�p�qè��s{eZ�c��R5`	�Ur	Kp��K;dzݞ���{�*��vn.#t�*���3Vɤ�J�b-��K&�G�$Z��[,�ǝs�pJ_�m�3Xʢ�LdÎp՜���d��(� ?���U�k�Im�ie�L��]�L*k�IXNb�L��u�S8���>����p�IY��oa.4���J($)K4��J��Q6/2�G½v~�L�Q-\�'�YŴ0��@����nka4�R� ��D��zp�)$R� �if~�00`��?i�� #C�6@SB8)��)H�h8$�h�/׹PV�=a7 0ʢ�o���G#A<�)Uh��$&zg9�������L|�<Iw���RIZ2�W/:S,�2�	0r�t�[h0��OI��'	������QB"�=>ļ?$�`1�#XEY�pۏ�G��<�g)q�?r蓏£�mO��G��(k�����$Z���h$�8q�"m%��@�C��.�N��SsGC[�*��)�F#��84/-�~@�u�ǌ:�"lg���b]�ԈC��&���hLaoDZH;��x��$�������.	������EQ�R�E%BS"Z�>�y�N�ڽF��˹�6A��$�/�D���ѕ��=�*�ݫ�G2����"��$��z��bɛ�&i�CEl#mX�D�hɗ��w�Ffv̷9�(��IA����Pʌ�N���Dzڊ8�v�2 �W�F��#f�D���|.hmR�{Ov�6#����e�dWF���?WD�&#x��̢jy��S�FY�73K��%�u�����̲2�nW�	ǑGڎ����eYE�7��.iou�_��9<�Gs$e�$�;���{�e�%�4�X�Ld�䇊HN{��y�E��i崷>%F�I<��G���P�(7�yOQ��d���r�0Ҧ��.S\��	�sBS���[�ee��	M�UbG.
�Q��e��SP�Y~�}����|�%�br<߉2�T
a]7_��
�D���b��
��v�'��b��<���T�<`�mR�&\a�����_L#�	q2���Ub��m���$�"{iꉰM�V�6�^��ߌ2�徲�)��i���Ы�H}���ϫ�'h��A]�լ\T����u�_,�TY��	��x��J�$Z���԰ZVd�Ӌ�7+�p=�3�aW=>�²**,��0؞���RX�]��Q��٣�4h�\BnT$���NV�J�T�5w�S�H�'^�~*��z̶EFV~Q�֐�/;���ġ�R�~J`�-�J�&y�@���.�2?�4Õ�΁#-���V����("ie����;�H�Y� �WB�qW��ڎp�z����x�BM�ۚ��6*�o};$�`k�
����Tud�i-�m�d-�c��M������n�J�m�l���{��X�昕�[����_&�Tj�)�$f��Ij*�gU�D;G�u5&��m�7NԞ�g&>���pa���n�R%�֤<���Ze�}\R���%e�}\R�:P��ҡA�Q�z�3S���2e7d�huW�2�$�ʔ��)'o�{�hEN��B��a=�:qn��k����dM�tT�hz�#�D3���L8��Y��X�l�{vt�����.�ԫ��3�#�D3.U��R%�h�h�醙'�nU�<�(r���kI`�2���Ly.y(St���흊���u�̔���2ՙ^]�+����<uΨ<�9c>\m�JU�:[T�<{�ʃ牔F�kB��e9xf�aD}g����@@�d�~Кhܣ�D#�&���6E��=�	��K��
��i�������U�2�<�ޕ'�w�	X�tg�y��r�*۬(-Sʦ�n��<��D����%:mO��(h9�����̔=-iĽ@i�H�M��E҈�%ۗ��ۃ>��!�p۠p�����H��ЭE���iS�Ņn7���ې� �B6�$4SKIW%A񨌤M��ObO���u����4��?�V�A���(�{�-�*ۦWY{��kT���zh������n�?�����(���v�Z䠕�aE�(9:ŋ�����Q^B�.+�}e�,AP�"Ǎ���:�.;-��8@_Y�{ݖ���� - �-�a�ek4Z����݇5�<7[���>�a���2'����EU���K|��y�Ea}l��C'�tw�i2oL��j�[��A�t��%vU3��cuC>�~\�SI6H��C˽����d5�Ewu<S~��L�.1�NW.7Ri�o��V�V{h\����4�>�lZ+5�%'�����n?�	H�hs��y뭛R#�V�Fq����2�~�O�X3 �[�=��,RpY����3�VD�P��WE[�Q��մ��fN��,]��N�?�Mo�(w��DKY�&Z��UsPV�Z�h1_%eq����0w�I�NH�Ml;�?
�w�S�{��w^���?�~��'/_J�s�]�k��p���>��!����g���?�.��¿&����nb4��D��3�~W���?��[������SkX� |��M ��x�?��3�3�3�3�3�3�3�3�3�3�3�3�3�3�3�N .R�Bp��2�t������*
�2O�&g} �N� �Z�C�%�X+xY��z����\K��&
,��2t��qIP���o�N��u\IWp݊�:`�cm �{ m�HI�xG^�`N��g`�ZĎD>g����]kJ�w���䙃�u�M|���H#��R
�J��- ���0&#[E���઀:�@Lm5����$T^ɗ���!dA�[�*Jڿ��\<e��'1-���Ps����>ܶ���h�^>0��cW�q�l'�ŭw�${ŇW���^"=����̄�+�|�V���L-o���1)0�*~�����8\ו��5�%\��q����y"���a_�r"���a_�r"���a_�;e['�E�^���k)�Ų�AAX�]��Z���s�G�N@��$��]P�cR���`����|�� �4h��HS�����%W���8�_Lpkk�@��t�>�E��w[1 Z��H�<ԏ$�1������	��'���ր�&�y2�nd���-���w�l���$���lz�!�۝ěؘ��N��:N����;f�M括po��%�fY�Z��XW����0�r��[�X�pW$��{�}����C��i���z����-1�:l#��Y�%��܇`�ŸK$�k}�`�ɀ�y	��~H�Ї�� �(D=f1ڤ	�;0���U�6=��$F=(W1�I�r�@��"��6�Ȭ')��B���;������AP�u�mq�u��4䶞B.�De��
����O���;0_�����-2Z;���A�G��ԏL�p�b�4�n�F���f�mṿ�I����8I�)�A\��MzOT�fm���&z��ɾ���ח��}����/��'__�2��?N���e��!���'����8y$��;�1VP��C6�W�� ��UK7h������AD�����4�o,ԙu�2w��l��C��t���T�O��*kI��VG���Z�-���2VV���o&������I�����WWpc�+�?�Ȋ���2���"VP����h������Ka=�L0�R���q�Ĩ��]E�?I��/a��J��<���GΤ��u��������,����Gf���y�"wb9}Jb�H��YlO���C�o�����\��^*~U�'���T���7�^o�!���f��3�N�
6���J��l~w���K��T��21+H
��;��|��Fhp�_W�t�{����nh�����6��k5n��@yʕ3�iL9��t^j�ᰂ��W!��	�� ����"�e�0RсKk�;*���g�Q��v1�Nb����6��0��ڝM8_��N���~Q����z]I��O�y0σ��MJa����k�O���p؀A�����{'�vh@�41{{Z��ށ� ^K �����u���v�h����|`�9��+�m�E2͒d���J��UD��B �n/�i�
��7����Y���m�F*��₱����M���&�s�R�ܭ���e#m�����ᎊ�=(�� ڛ�ѭ'H���� ^��/��+Dk�幚z��.�&Y��&^/����_�F^9�ȸ.J^��%c�@�l?q��u�}��װ|kҴ1~�걨��"��KVg�����M7���(Pi���z�&J��,��L!����7j��Oj���1-k�R���C��Kؑ�ц��z[EI~WEmޤ����B��� l��8���4�hzb����
�V؛l�c���|_��Zp�дvl� B�h[�!w�,wI#�r{��}~Ֆ��X0fw�xi��Ne�F��"֡�����"��A�Sc�,x������+�v��XyX�m �3$O��)d_��}��A{[���+��VP��0@���-�%q߂C��k���0�u�� ������J#�-m�/���^r}R�^؞:O9+4hЭK�EJ�z�P}�R�1����|N��؂f�ŉZu����m�!\��`�޴}��C�y���o��H�kEƍE`�4�<���{9/uuU{�Anމ��>kf����<�-k�oь�~�3����TQ����,P�4�#������_�i_ۆHk�Gm�6��z; `�9ʸ���q�)ci��s<H�&�}��	��[�/X��	����i��v#��׭5��?N�΍�՛{���|��w��>D��!`�P�V�ط>m})�%�K۝^''=�������)��h���m��v��j&-ׇ�`�ǤAUZ����(WʎL����1axbzj������S���>�Q���+���*('IU6���8ߛ��q7F=�M�>-�a����KM��9Y�� -j�:W��w�m��]G��"�����q���K} C�U9+���-
�{=�24�+�#�}}�3ʝM�6���8���a����f򂱅3W���fu8��v{_�k�U=�M�x����M�-�p�˒��S.�h:�n�=	u1�9��:�n�4 D������������4�c�����bW�{�f������-ބ�>����~����ۛ����q�B�B����9�V�;hԡ�6��7+����+wPWLpʥ��+�8�j���\5�5�z��6��M����.YwRp�׾h�z�&O/+6.�ee�&����+��d����������oۮ�i���q���k��ږ�x��m��F:˓xR���M�>Lw��f̹ ��ǟ׃7p�~KU��naI�$5���UY�Dؓ(߈|s�,S�A�2�;L:��T�x\�U�������7�{��G�W�A@=@���%�-!���5��]I˫�8~����9����@d?���O^��۠���_�:����_�~����y��o�|���O/�h����׿�����^�T{:2����^}F�����	���3Z���r���χp5Z�Z��*��M��������pO�;�_�y�e�zu~���o�W���������o��"Zz��8^}��c|��x���Aww�V�x'��L@4Zm���Y	�J��|[nF���
�o�cZ��_�T�'oD��؞\�-�w���B�$k}���D��7ҡ7������ ���4�o�uI��?-{��,Jc���4*Ƌȿ�'-��.+pt�jv��e��$��$:�}���XSz7Ý�a__�/��ջ���;_~���|�����*I�t�U��2����~�.\.	�x_#���n�/6�u�^������`T�C�0"tc�����}��O٧ ���\�B��bP� ��&Pa��p�N(��ۑp5O�;Y��P��&��l���CL��:ILNG��3��+"�!	K1��BLR��?��,�<H����7H9�1`?��n�&/P�m��v�T��O|��X�p6 �f�>���.��Kй]�H��0p,1;X+���Z�n�4+�]�W	��4�8��vO2�0��At�����z�e��taU��$���I��bPz��� F���Af�,�=�|
��n�~�b�b�'
������|4�ɶ:#l䜸���������n�z?��(��*?a�z'���x+��~���]A��H|�^�b�F�.3�  �4{���LN�pUW["1�fA��ÿLY�ي��xB�H��/�������TҬ���4k^��@W�;{�nt$�#�Z�4�qM���dt�5]J���*iֲR@nb($͚
w֕��;r�"Y���H��Mc\7q3nC� �o!K��{�u��\c�������4���MÕJ�@ZX�5	X��2"+qU���˘lu�q<:q`BL\�?�m���ܐ������N���Md���̲�����s�e��Ũ$*r�D �_��V�;9V傪'�Y[;5V%�ڪ�j����Y"��Mk4�@���"C�X��ċH�5N����r� �ZTb�-���|w�VӢ ��E*H~<&Fb5Q�q�iՒi�w�Ċ$�iłǶ 	�8�<�3D�FPШic6�Hb<�� fE ��/Nb�X���	&Y\G '͑����Ki��&������3��D��ȍ��ȍ�Ď�����Q�qh��ю��55k6BN�	�G[sQ��QzD�	\wI�:M#���#��Y��1uqH���O��`�FT�s��ˢ�#Mc0�#r;Dȸ�W���VO4���I��tI�hvǭ�������%�D� I=��"��!-�}�����MC�4M��i��M��#���h�/�\{�t<:��Af4�ȏMc�|��ŷH�H���MS�C�{�싚:�b�#Z[���v�� ��=bg�s�;9�������}|����'΂wQp��Ƌ��4���Q.���i��T�yr�A�D�G���}k��}$q3��X�A�N>�5�s��89��J�1��O����|~ ���9����s�p�VD��#5�i�H�naQ�H�5�h�:�iw�7��A�G�F�\����U�4���#M�/I�h�?��XL�2Zk��b��4���i4&i�-�F3a���T��i4�E�4h��h�<چ�~ƭ�1��� �@�O�FS�����l4��&:A�
��a:�8��[8L�H:AS3nˠ��g�A������N�A�����N?���B�uR6v*BP6v*B��$@�?uZB�ҹ]:�սdzN�� �۬���t��,<ec��	2)I�$ec�.$j��A�h�BR6v��:i	<eC��X'ec��,JCQ6�ꓔ��T���3�')M�I��d��u���1ij����!��E6���!mc��z,��P��=�l4�!)���1�(������l4�)7QБ�QbH4��`Q">��aS-"/S#���Ԉ�i45"i}zÝ�q�tG��6�j4=":Z�T)�g�Mǘ&u"T�N�Hjƽִ2�5�iI�hE��:�")E+Ij�b��x�TL�RQԌ�l��4 �M�HjFS(
p����pR;5c5���O���FT��+ ��7:=0�"�P�]$5��S��/<�zt��`�'
�t�`$ce#����˧r�D�xL:F�#:�@:F�	ޢ|E�hjƍԌ��'5c�goQ/*�+���ݢiӉ���("�@e$=�c�Z��բ�!�:e��5�y�}Z�&}#���^1vzE��*_�+�ʱ���T�Ǥr$��(HF={�bѧF�i�>�	��4�ʓ���w$����H�h�6�(���4��j#����H�h�6�(���ԉ�j#u���H�h@(�4�Tm ~ʦj#]b>�%���t�����Tm�L4U�I>Q��&�Tm�H4U)M����Ii��:� #�MIZD�A��t��B4d"��i�II*��4�eRC����do]5d�O�+O$����B�ȒM�<̦iˇ�"Ms�i"1�s]�a���H��b�w�H��N	��N� '�v�H�oSF�bU'��0����ߦ����u�����>���t��4�
�I#	��N#IJB�H���T���@T�$\M7H�*���6�t�A3��v���ӝV�'����ZI���I7��3�I3y��_�nJ�C'��dڦ�CyMӶ�:�t����%���`Q	������t���u��E7H���fRP�e5�d/w���~4�_P�	�i�x�L�Z>Ӵ�f
@ő�4m� ��� 4M) ���/wڿ\��N�FR��D��M���M���u����i�HM�M�;���߶�.p4Q��F��~�O�yj/��T�e�H�f�4��5�$�EM#IjQ�⑺��H�N�4����D��N#�"��L��)#I�Y-��:�dAM!IJPSH������ʓsN��I����H��|[5�^��[	��uI�3�H�z4��su;�{9���^�t�:q��B����!��i�8�L��yf�6γ��{(�i�8�LӶ�q�B�=SH�p_9�E�g�6R뙦��zқF�;�����:��D�'�$
=ɥ�MSH�Bϴm��1Mi�LӖx�!j8�晦��y�i#U�i�x#b�FR噦���	=�)�H'S�z���-�Py�/�/tpBS�iO'��i�.�B�$ ���͗o�2��L!I�;SH��n�l�3s������������1��D�;�Gby}�"�;�G��N����3}$����q��g��1M�/i+�o<�K���U�Ȝ�������g�;�E.��C����)��()u���&Rb��4Ei(%�Hqg�H,��>r����D7)�N�	Ӵ���H�M���yE�:��h%��h�X�D+�<�Ƙ>r���ԭ��<�G��n׍�&�H��m�60l��T]E�˱��������3M�n�6R���Z����N'���tt�9MSg�H�����蘎�Q���і�~+K�:�G��=��[O4pMW�e/���3�E��n�t�HQӭ��U�j:�0 aEMLG �`::�*K.m�-~R�QF�]ӕz�<Ntta�љ:r׍0٠h`�H�љ:�tt��$�o�wٖ8o�K�tt%N::�h����Z5U$96>�љ:r���9:LI::SG������0u��sTSG����IGg�H�y�:��c����y��!|��3u$-�t�]`֓��ԑ��3u�.`�NG�t�H�ѕm�љ:�tt����e�Y�i"��p�tt��v����ҕvZ즣#ͤ��F4��w�!���	x-�4��e����k�>I;g�H�Ι6�D%��,�-�3��+�tth/Ӷq��-���tt T6K[u������3M$yLZx�llDB���δ���6m$��%l�9/::�F��΀Τ�t=�[�����4�EX�G_b��C��F��n5]�fp���P2I,u:�K�dR!ݡI�Hw(�T�II�:����t��?b��){�Η�^'=I�uғ�^'%�:�$����[�u�Ib���I~g�:�,���'�u5���@"{y#�^g�H�\�7��u��	����I��뉽Μ�����m#!Q�C%ڵRׅ�4ׅ��@�nI,�7r����/�@�dw&���lnttN�P��-�D�sF�;�nB��H�هй-<�#9��{['�S��ED&���;yI�Ť&��3g$.�R%��ROw�}!q��o
�@��F�D5��E�� �P�j0i�� �Tɐ2x�A��2)�>:e)h�'�R%�DAS'T�9#EA���(hHm3��y�%C�G2uV����)�!ŁT$�ޛ4��P&����I#y/R��pϔ'ǤޫǬ(���đX�$�xCn�H1�I�
��61��9��yS^�G|+��t�}����e�:����D�'b���3��*b&Z�����;��J�C1=��,�Jl~Q���,�'	�ē"'�_���*�Iڡ�b�T)�0Ye�7��g=q6�4K�)¦U���/�?�b�T���/N@l�=�:"M��,9ۜ��7K''� ���IN<�a�<V�̃��C�3c"4Q�/��"��E��@O\�b�Z��]�D��b�<��h��@�1jB�&l�|-�aR����հ}�ä2q�1(�"���ϻ���h��D�&��x�m��D1L�,3�a�<y�'B�0�i���n���C����}�ŞۤҶ[�m%a����G�f��/�6�l�F�4o���ir%bѹ;QIg�K��G�,��ǅ7�f(N�������`ڢ�l�'���"�#7Z�>�6��1+.��P:�6�b�Q�`��)�HQa̊,���2�I~��`m�C����&�X���m���"-�S-��qR[*"�ro,�d6���.N{c��lA�����ؘ1���F>o�$���X)j�z�����~�/�R�j��J����OQ�:ߣ�Z;���Ն��$b֪�Ř��sQ.=brQְ���������m�bV�-�OG8"����EUr�~E���Y5B9=���Y����`�W�ȱ���wR˽���}�ȉFt���u�}bz��1G����3��of!��^Y��XI:��l�0-�$E�M�_�m�;�h��*bd)�n��d~�S�����_�3�}f1���$[�z�D�tz7I���6��t�5�W�$A$ē�MkN��LM4+-�����$$&�*����e���9�/�l&��y�D˦���YO/���8K'�lL��$Z���J�E����-�A��ك'H%Q5�Q���ZNͷeѐ�G5���o�M ���Y��v⽷H��l&���{lQw�:sv�ihk"�vg�	lfӐ�(u�nZr��̘@<%0���ű��E�u��m+_�슆T�d�`�?�1�Y����oe�!����*�hȤ'^�<�����$�wэ!��zEuO+m��]���/��<���;���mZ�K�4v>ݜ>��9��k�ֽ�����?����[��4�i�!�iN~K�;�SDn���v�\z�8W"�����>y��e�=dw��-�{n�3�'D�#�����|�� �
�+����
r���J�|e�9P��ןJ�8�d�-�$�����L��"G�D~F�Uv�z���ϰ�3%<�����z��}1��*�p=cDuʈ������+��zʊ�#e�y�����T�����A��<IǓ��GWx:�߆���iɷ���Y���c������%�H_1Q飄46�bi1�z����#�Ş2�
���;f���̂�XZ�����9����0S��0?e�c��G9v����㦴���S{F�ǆ(���_�9�7�<6<
� ���
�v�e����#���C"���t�<�u�Ǖo{sj^�٥�tI0�uh7���0]�����Oz�.�AI������mk[���_{J��_q}���������k������n+��_��_��_��_��_��_��_��_��_��_��_��_��_��_��_�J�_��_ip<��|R�1u�7��"B����I�Y.���ɘ�r.���ɘ�r.���ɘ���S�}�t�I����t�I����t�I����,�M�O���@�EǓBg���W�l��G"�|B�0��������7�oi��\�l�a�`���p8 \
IDp`V�%��1;Xy�r�z]Hu�P[����;H��]�.Z��
�p	��� �"Pok�%��7G���%dBg.����	�����C&t�Z��ЙKh�W%
"
�=�K����Y�$1߇#f9��|���L�}8b��3���'�Y����,"��$1h��C��,���#�Y2��7IШ�~�ѱ� $1�X6�?I�=~��]�C�� �?� $1Xb~���������,`��HbL��$fQ>ߟ$f�H��$1�*�K�� ��PK?I�RW�3|O����� �Y�
�$1����/I̢��IbȠ�C��,`��Hb���$1�� �Y8�~ ��Er����,$?I�2[�{��,�w�2����C��,��?I̢�����,�?I�rj��E����n_����ԧ< ��c< �7y@�� ��W� ��-��0>қ�h�U7?����>��#�I[�J���؆�[�����G���{��Gy|�7�� x�pa��� D���(�^��������Gz�	j�N�[�����G���G����Gu|�7e�L�O~�o}4:�o�� ��c^�ÞHQ�ΰOHQ��u"Ea"����wL����ܑ���� �o 1t�i�EL����� )J�]�ƙ�Di���~cL	�~ۘ4����!Ra�9�����VO�J��G�J�.�p�욌N����'y翿K�x,_���wc�|����wŦ�D��}7�W���;���z�h��ⷱ�/��}�wk�%�g�t���{��v�h��6������Q��0kH7�'�*�s8V����Ң�L��j��0H_sD�c�����R�y�W�?�OF�9Y�E~�\Ӆs��}�7L��p��p��|���!Wl��*P������zt� �l��yb���4�������L��^�6T�\�48��6��p�N��dB7���IX��G��L��	�났�rd�h�� �#��3��x륻l��� 0C�\��\y5;����"�|���'�|�,;�/
6Χ,3`؎p�=D P���u�x�ѹ^x�A^Up�r=���|��&q`� G�w�ç����m qt�A�Ɯq،� :e ���`� 7��?_�-Lx����v�q��������S�1��z���x1�7�1�!��ȉT&���{?9'���h���݃�a�Y�r���Wc�z�~1�Wc5�, ��:2<'����s��k2�q���|�1��)BH��0Ӣ��'O��z�!��a�Y��䉢���)���P�h�����oce���$=��{=D�2=9s�� ��aRA�UO^B��H��-�C%�
1@�SŜ�s�N�"X��5��PL=�O?�UC������S�3���ɃU���-�%��g�ўF�g�F|��u8H	VўF�A$fx/�cN�19���,��k��J�fn�^)$ 	�A��'t�b���4�ߧgR�CGy��3I^/�b��{��0��1��"��=�6Ҧ��g�cN�'	�=�62�`��XDO���n_%�_�=�z��}/��{2�$w�����8���^�d�$O��+}�\)���ةʌ*�4�J��ӣ�����Y��b�3���'��[��tL�*ǜ<��Cd�������pҩ���j�XY����vd{"�NO������N�L����0���Q�3�O&��"�&��^���tFI�<̿��wӵ�mh�d}�{�2td�$���A���<L��bg�V)�VסR�u��Ɇ�`u����JuQa�P��+����X�f�N�	��U$��րV*NX����I��W�֠��[3ɰ�چ��H��  +��T�!���
������C��PPU*�T��J�`O��s�R)�7����!�7R�����g�Q\L�h}"U����2M�J��b��"le5Jx$M���֊DP�l�������&���K&&h*RvM�F�%��Aq�/��V��^�i��A���f���ic%ɘ�=��C�>�"c�.]���$s+��i%r0ɘVmT6��"�����jG�4�6��zB7bk�;]x��5QTLbN"Ӫo��>Kl���gw�:4�~v��D�f+��e22I���e��)�XH.��`MR�P:u
@cM�E��� ��<�h�t!(P�Əߪ;���N��`-@A����eǤ�:x^�Z�����I|T��Kо�2_���n"��j��$�[�gd��O:7��pŶNB7�� �dc
�ա�6�٘D��&i�-/bd!9��u��S7�����~C"� �!1�=rg�2�YlH�d��P�^���5d�fT"��t�r�#�g��d��Т�2�Ye���I���d�*�1e39���lLBv[�=�3m��d�L���LLbu�>vHSz���i?11�I
��I�LL¬���Qd^2cDM,bN"ې�w6�%�Lf�"S5;�v'o���E&o���d��$6#��duR[̶ٶ�L�KmUX�6b_2k�:�ľ����Y��2����O�/9�/�ݩv��μdg��ĨN�Jq�,Ji2'��I鈁���dH�Q��H�LH�?�bmCF&<[̼-�r��KٌKy�!�}��k�YuƣZ��ؗL�F�%��}I��b_2������L�v��l�$��Fb`ʬ�L�F&����i7s��͜�|w3'��dD�.3�`��Pu�:32��h5K�۬e
��S�LL���LLf$"����d"21���LL�#��t�!p���4�Td���D��ȌCdf�|3�Y���d�!23�e��t8M0k�Y��Lfb[�u����,�EȌ~be�LBdaY�ִM&!���bO"K0CӉQ��,f����i����b���&kPΓ5��&Bu%3S������:����b� �3u� ���)h��)(�i)����y�LM9Nf(2�$34� ^���)�^�Mf"�K2CS�B�� P	:��X�|dD'�Gbq�'Gp�dx�f�:��M����xd�3��ጬ/f8#닏���d�3Ȫ�,�L��.�E��Nf3��6���d�����d������$�W�;uo�	��Bbw���4x�q�E!��`�����|��d�32<���O�,Md��X�gg�Y�d"�S,}bw*U�Ne2�驚��Bdw2�ٝ� D�r������o�A���U7dv2��E�Y��� D�$3E�E���I�gԧ�2�3q�@�R]��d!�3���B��zQ�N�A��1����,d 2��).�A�'�f"k���c!q�����1!��=괝��!�a�nu!�{q����Bdn2�P$����i!27�A� ]f�Q�F�/�6�A��`b�L,�,Md2K�c� ����D�"15MD�X�j���D6�CS2C�7C����Ĵ�Z�r��� S��z�)Hu�<3��(�u�0�-�,0?a}��Ad��fh"��^��$�$�%PC��BdY�~�x
i!ba�A�(���r��bX2[��Z��LLM���A��͔�o̔�_{P"ېX�8�;{�̔���Ǔ��-�#�a�B����o� ��=��=��QrJ�Ef[�qN��d���LAŬA=O�gg�{����:�<�4�<�.�<�lB�,L��)6!3�;^���|���թ�H�3sRn�:�0��� 8D;�v���Q�����2%��z��Y����i^O\BN`Wω��<A�!A�^"D�:������b��HsLD2��Y���FXb�1kP�'r��ă{��l���ܛ42F�E'"��*�4��:�*�x^�)�����$yx����?<�0��=.d�y�?½��G1e�V'e�1_�YB`����:����vJI����l.���w��uF.�	2�j��m��F��!�ţ���m�-j"�gL���=b����DB�o��F�#B��՝���xc@~�����6��Y��	@:4�VD/�"ZS��b'��VD%�"4��" �^f{+b��]��R����������m�l&8�j�u4/)�2/,�b������.�<�4���8�,ѤHGN"Nꈿ�|KRO��UJ�dʳ�/�����e"�Bo�A8�A�ᑩ��u5;�7�B*q�/	]�:�[���Yi� �;�˽
���!�T�TPM�jrVH,�����M��6	�K �Jh�I��	g>=�s�&lh����0�vj=ȫ�CEuX��2u�e
�����6q�0�ʷq��y\��M�Y������:&���N����7�#�c�y��;�{�&Y��pȳ���R���e�X�l��}03��'�X`����3u�Q�����^}��V�ť�i_~dҥ�|�f�s�sń��Y�Z���z��3��f�{��`]"r0�a����'��l5�G� �I�0�	-BM� s�FV�R`d�iR�tFq6���ƹY�y5oIS8��	���Q0���򊆴G�
C/a��(�s��G�B`����5a���e�A�7�h�A
6�[|���&(x�G<,�z�q����[���i��m�qV5�{�y�0���x|��8�)��a�9l�� ry��H4��x�>��տ*�'��I�O��n�opoT�*����6���?�-��k�ƿ�ku�g�?<�g�A�?��p�?c>c>c>c>c>c>c>c>c>c>c>c>c>c>c�=�g|{��H��x)�h�!]�p}xx�
���@%@UX��P3pN��P��J����P� D�����nBL)�Ta�
�B�E♵��Ț�����+�?�� +�1�-6�=��_� �#�D0����<�/��F��n��,�5��лt��NĎ��:��v�R�eT �ГJ)F%�@�U�� <\V��l���aU y &	��8?lh�F��W����V��V�u!��_������@��p��y��.�����t'l7��o.���hq��f,�!��<�tO�|M�#"� ��.��Npa� ���A��M��9U`fB�܇��7HH� ���%T���`�ky�5�f�7W����o�=�8���R�Wd ��|#x�DX�2&�N`���܄�C�☆�#d�;�s�5�ѓ�[�;�F��.w��T�����Z���\��1�b�BM�SL�P��
���@���}(��m�@�
ty,з�]��-�@����������e����#����0H����� ���A}yF����m8�����8�����8�����8�����8��	������Cz����uڇ`�Z��aj����J�V�&�[cTt����B���������y_ʕ*�U�@ou%�tJ�B���b˿?@1���&O�b ;�����&�:��@�گ5LP,�f�k!Q��`���h!���aF�`Eo+��p�h�F�5�h��m3zi���t�(�ݩ�CW"�Ԏ���t��k�{�h��_V�	/���~
�JqX�q��Ì�g�Vt.3�Eѳ�f�v�DVt	ˈ.aD�CU}��&p·�=:;Ȟ�f¸��f����F�ft���
+�T�8�'XG��o8�Q�m��4�'wcE�m��FC�4Н]��ø3HZ�#�S� i4�O�{[��l��ԧW�d���x����{'���_)��Op�h������x<�����=)4k���1(u�xɔ��������aL+H���.����5F�O�>���O���鬍W�@n��3CbT�#��m�����Լ���*Ͽ�S
v�'��؆a�*�N
��I������K��?X��7��n�2vL��C������#,�BG:�R���XA �o��Lf�t�6B��A08�K���t���B���,/P�}��0��WblI3��rB2B�;|���%��`$ؒ��L�-)h5��&ؒ�VcK�,Z2��%O��r�В2'<�D��|z|��(i����(/v�k-<���q���hOX�w�x�b�(wz c��C	�, qu�w�ج���P�hԘ����z��ߓD�F��:��N-�?\bk��Ӽھ��h�z57�{/r���d��v7��Ke3��O��āM\�#n��{/�8�1�� �b�\�����>K���P���N�my�v�wԣ����G메h˴�e�@x��D[�U������hK����|*%�2�+㺅�>�9������n�p�lᨏ�@��3?ٽV����XM��!ó��t��%�̃Nt�:}t*=���ң�!L[D�vN��_��mlGu4*���W����D�R����6��]�߹?��R��5�"�e����J��v��xMu=}4����v
g��)��ct�zd/!Lw�Ķ<���)����60zJ��BkQ��v�&@��7�.�����q��4؅����D[�_���9ق'�Z͏N�N�!Ղ�ՐP�[�K5\Ă]����R����P(~��3
r�s�~n������ЖY����~f[�O9gx?�s�g��F���rf[jp�����lK��d6K��'�-q3۲�	,�p~~t�=�mY)�2���ٖٓa�m)7�̶<����쁏m��.|px1J	}�Ed9��U>r�4���i���ES�m���X�[D��������N��R�-7;��Y�4g�V t���-�#��`�Xt�=|\�l@8���YJ����`����va�G�eg[�)bg��Dbcg[j���	�u��z�3���6����6����6��G���;�L������� ���9w��|��2������;^�vK�����%|ǘ���c��5��Q]F7�1��,��4 <���"�.|q@x�3�68��qN��v�#'XA;�F���.gkt�`��k}�	Vv��+h3�$��]�l����i��ٮ��q�N�J�m�q��a���sa�|�l�}�`���bn�)��>�<��ѩ+4=����.�e
xna�������SA�����<�w-^���G��x�-"��z�����8z���F=����]��V0n\�V0DՎu���/��N2I���`~�����H�����7%EB���n��`.�G'!C��"!�=G�/��D۔lOC�8Kö�v9"axGz��:�H���>����H�thb5�1�#�����pt�d8sX�>��8r�Q8�u'?��$��\(i��x*�P9���<z,��,�g蘡�zJ�Ex'�E��{����6���r�,saq�{����\��IO3n�0\W������r|q抺V��Hս�!�"\�Z��)Wa8B�Mt=W֕����fm�8��)
"U���YWʃ�p��.���p�	�F ̞+up9��X��I�3��G�И�C�1�(c����Xg��	���3+*�'����E��]�(������2�&q��#;L�cܖ8>����#��#m3�B|���0��"x�S�a�����U&2�:�)�{*Ӻ��R>�͙߇D �:��1"���9�.3����3���jC��}�����"���(t�U��C�Tw�b O�;.q=��RBl�Op�fjF+|WG��	����M��I��"�1'���� ��uO�"��#}�=���]𞧮S��H��Q�'to�l�����\���+t����ѽ{�m9\�ߍ�X�����cN2����K�
l���cN�����\o��"���>��� W���b����>���W����'��ѥs����0z5=�	,:ү��ק���Ѣc��>���x+��c.G�5b������x���=X�<ѥ�N���X�����9��;�4>��P8Q��۩��9�/�w�f#�����H���'BtZY~��D���c~������1�i"�$}�=�zL<���s%I�[$v�H#
Og�,UyX�:ۧ����	��D��pL0�3��O��:NxB���N�3�u�-`TT����5�W�\��	S�X�x�o=��������g�z�OP�xBWO���Yq"T\�G��9�?�jC�&BO����1'��Y���Y�4�v�,|:�'��N�9�xQ��2�s�����^W��w%Yh��p
��x�mI�h.�FL�"���X=
�=tܿ-�9x��\�]W<]?�����^B�ィ��C��Ig��"�܌��j�㾿 ��1|y�"�	���F�M|0���!��p�Ox��mA3����k\���(���t7q�{H��t�^�O��a�N�r�#�k�^���$6*t��o�k�u��Wx�+�%�E�z����N�T��xc�����r��8����
�G�/�E0żc1�/��}�.V���w�}�aH1t��o�ΐՇ�w�1n"��/.����+��� �y�`�]^�r�Hr��� UY��mÀn�|!��co�--nך�w��?�CS�к<q_Ն�H�к<}.X�kU�C�n�3.��A .�'��q� {�D/1d��l
Wa�1|��a��$_y�ȗ��!�Ixl#_Al2�w��:m��6�\��EW^���mԡry�`x\^�l��M�!�7b�)�_�]T�`H\R��]�Qx���:�g8��a\e�D�+��]IVe(h�$�Y 2��ũ�yc��i=�P�y붨j����w�x���M�����p���ư!n�����z��0�//AqӌUP�O�P6k\�y\ ��v�/���>��{��a��]yMa�_,���Ζt)�0;IPs�qGҔ~%B�Cغ�ꀡŜ�𶼠� �|1�S6�8/+;<m̾DY:$-71���|�0�$Iw	��J��g!�r6�/�5�,�B� X!�:�,�S���|�� }���@�%�Zx@��8� H��6�{�� ��/N_�ԡdu�2��yE�[�:ng�����9�����c7\
>v㵏Y���\���=���`��;�G���~0��Ax�W;��_���W;Pǃ�b7r���|�Z'�p*�m��6#�Z���Y�f�O���n(j^-iMDp04l���E��-�������/����=gij��7�[%l�0�Ѕ��T�~���`�W(I-,�hȧ��"�Яn��6�{|��N�E���:�߼�������!�	�M�o���uHXȪ	K�4]�68tHXȪ	Y����:$,dU����ꐰ�I2$,dU�����7�7�1�k/C�q�~F��v�в���Up��؏���K@�g���l�f��ˀD��21���~_��`�Wn6�	4�����<���Jl3|0��+�,�
˗V^��U�����2.ޠyC���䢡^��C����xs�x�[��Nw(h��ٌ ����<95�+�W�?���|���M#�h��h�Ը~�7����a�3�����2�1��a��>C�>���17��z��Yd�רk�	���W�RC����a�ykXj^1b�+��枲�1
,�y�Q`#<C#/CUS������Ԑ7����|[57!o|	�;��-l�d�[v�����m ����H
�nȕ=��c�E�a�˸ݤ}�.=:�NTrȖ��م��%� [�K�=�d[���7ˏR������2���0<l���M� �;���B��d��6�,�U˳w���pe��d�.5��UW��B�'��(�����BeS�,�q\��T�ׯ�/ڳ!��W6ds������(��>���׺� ����WZ�솦���1�y�+g^�"sz745��nhj����7\��z�uQ�0�4d3/n�/��.JZ)톧��5��(w��+/��� ���klCS�z��Ԙ�{�y��Uײ�F�Qۉ`�Ul'�!Va��F���Ƽ4^*�G|��ޗ~��8%�F�{�8�����K���3<5��O�9�ᩑ^�Μs���<�������y�!��^�w��C���B���a��(O���$X1B�nċ��4X*����,i�d���q�^�r��}܋c����3�|ߋ�ɂ���6@�Q[�PZ����( ��pzR>�;����3��p�,�e�o�yUQ����7��e�u@uŜ(�Kk[�~�l�h+P�.L��r��ȷ���'��^*���-W���4���=M���ش[X�[��M��F�G����g�5��:yi/�f�V]�ޔ�����*3�I�^ƃi(O��ۘ&4��l���\���!�	*w(�a���L�f��Q���f���Q�s�/�p�Z��I�rGGZ�A��F�������n�1�e7�(�W�Xd�@u�V�Rqm� �2,P��ð@(O��ˈ}h����R:�=��o[����B5��y�'��"��m2�`9N�/іKT/[x{�����R�gʃ㠅{{q<f@E���1��!���m��UPͣ]ţT;�T����I��*җ6���i9<7RbJ7��½�dga�9j�y}��U,j<J���� ���38g��_%�F~6ǿU{�]�ۥJ��4l��D��*�Ɩ4���(�d��j4�p�գT�N���':}�����nb�W��bU!�M^�$2��ҕ�"؊�jA��Q;l�k���(�4������D���63�S�eg�L�l�lL�b�Yy�8���"-����X�=��)	R3P�!\�'�f�?|'�T�Y&뷶���Qk�X�~��L��2t�:Lx����!�90�/��*�0E&/��XTZX�r4H"�L��+��g�,��9'<����Le3�C�P\�){�`UҨ�ץ%A��l����9K���˓t{�8��>4.D�n|Ȟ���V�⬥�iaeʞ�8��
UjRaOU�'�3eOK��ۆ�W�=ms���	u��ޖ~�݃�畽+��_���<+�g�"�V��ޣ�$����q�I��Lqv �]N-�?j
�ö�4�Yg��,��� �{�ҙJ{7�l�r4��h����S����Q���Lw4y~��r`���L	��)��!aTZD
�&)H#���"2qzT �{N�Ķo$����H�m�(~a^��9��>��wx��+$�`	��=Ǜ)e*�_	#��J��pH�t
N@�흫���qaS�s����zc+Zc2L�+eJ�'I���������&?���]�̳���"� ����:����О��4�z��'�ͅ�%Ze�n�6ܙ��@6^+<(�"���.޳R�F{��@��i&+�C���E����"'O�eQ�����g=q�E��(��G0����(�_����DvA33���YBٝ��젮DjcSF�(�8T��@/!���Z�nm�E<�mek����?�V�JA�l�����Y:Rg���.�Ur=���;A2�R�L(�@A$�rޞ	��I3MID�RrZ�'��a��#��V��Ϳ�D���`�;�(a�Æ��:+iixC��G�嬢6	�����"f���\z6����*N����z#�i��(kԨ[r'�6�m-I�D6!c�U6��|Y��$�0��

�U5`{	نY��lìR�{	�A�M#V�݉�Z�v���s���;�D)�,�9+Þ�1��X�\��O�m��)�`=�in�N�W�{	q�N��G��"�����K�HvN)D+X�{[%Q�S ��l�/�D�V�Ol�'i�%��l۪�'/�D�V�1��,m{I2ǕW�>E���}��L�
Q>k<mr"l٧��k�"��/�D�&�8Y6�s�d��DPf�H�{"l��̪үCm��&A����|�'B�q�[��V����H�-[i�{ɤ�bo��� q�Ʉr6,vަn�t�
�e�/�DR���]v�b��CE.��k�$���NY���F�&�V/�,ɭ.����&ܕ��u1a<Y�b0QJщЍ(P�EoH��k9�ޠ1�Ϗ���%8�\�&�|qz� m�س�SsR�4i<��������;��>��Ժ��^v�d�u{;vB� /�Y���Yv�&��d^���|������:m3KG���`��)2<=e�ZJ��:�Qd3��)�bI���,�,U��ZR��-0����檣/��e�g��2�Oe_J��K�@2.�/+�R�F����%#h2��@K�6�s�8"�l�4�]Ź���9Iv�4 ��ɣ#}��4n�l/|�,�F���5�>�QG���>������k�i6�uu��5�q��0mc�*b�i',�1�Hv�-��w���̄�;FS�/��	�]��Y�9q�,q��#�D>s��&?�-�1�C�s17�p��Q�#�H�v��If��H�C|8�F7�B�FôC�CE�>�9�e7i��Tf��*��kcj@��`8���4&I�,7�\�ͅ�>="ʹYn��X8��Qf�,���d<<h�1�_�pbd�H ��Of:҇��@ji��Fk;�[^�s���w~
4����Z�IHM���a� *L�����@m�x<
r���[^	Al3���h��ycKS[�	Q�Vq킖Y�U�|��ٕl�l}��[���'x��
�A[u���['[`eZ=�L
�E���i�-b6J�d�gZS�|���:��˸u/���F����;���p�Q�z������©U��9�����y���1oF�6�<Օ2C���Iù[I���w/�a�4_�7�����aZ�q쇉��]d��Hx��*+w��Z3��X�#��@n\DhIE8�m�i��Z:p�'I�u7.QF��y�~�dQ���6�`�\qx��E%�{��Z�1�ĕ��AW�1��i���zL|�&���0����drL�d3xQ2�Y�MxVY��_�r4�]YM�gq`k9������
;:�.����h�v��=��}�]�LDaEkIR� �JPh:Z�j���i\Y�=��e2���Y����aE�Yb��O�cxQ��sXѧFʳ��:����i��9��6;:6� !���M�ͷ�a���t�(Ϥ�*:\��}�CaE��71��:1�P�1��aE��OaE����..� mm�3H�{piJL��9�r��/֫˷@�����,�i�+t�[�|�H[O�s{��3H�_�~*\��@`#<�wx�a��	�m��3H�&��dܶҦU���i����u����W�c�w���b�˝��qWu���ޛ;�pl�ȼ��A�0h�:}&s���j��g #����V�W����?W��<_鶂[����pw�G8D8���2)jժbme�^��$ݕ��iç;� �,�G����Au���/���1n$�����ِ �>v��Q�co�s[�8$��:��ސ�J$�9��."������ ��[ �9�ޛ�Cig��K�Z
\\Z�5(]�F^W�B$�}�&� �2I'���I:�T��V�'����d�9�p!���>�N���E��"��rd��J�C{��4Y���U��	����]�E�΃����#D��'� ��ca��Gล1��"�^Zwa��4�g�P*�1I:��q�G�(�F0ЍDi8�p_��
A�h�[��b�e	Ts�7�3;\�$��d���ʯ�]�	f1���/�P��D��^��� �"���@"��F^b����W'_�����/� ����e�7 r�b�I�B�~I[��H�䵎G��c��xH:z:Hhl�&L�`�&.v��q���E0�4&F��f�Η��ײ���F�N�j��(g�$OI:뵰���y8�%�P�2�N��]�~�Ы.��գk]
ӵ.��ZG�`~��u7;�n7'L3Bõ.�<��0��a��<a��|����d��eڮrxg+�&�·�2m�����+9�%�G�.;1a�;�a�9G�.;ޑ�y�Sx��M�ԉ����sX�.ɱ��Ǥm�:��J��U]�y?�.����\彶3sy�*[��*���nk�{yb�ݙnkI��t[K���,���i(�]�j�+��m���'C<�m-uQ2L��nk��V��a�}�a�b��[�}�Y��(1����0��f�1�ٶu'�7;��d�Ȳ���d��H
'�.:"y��Y��i ��0��>��R?�ꎧ�PΣ� l�������
G�(�%�&[��U9a^�̫(;}'����\v 8#OvA��J�nD�W�nD�WvM�A8h��*�|�ɂ�8�*��#f2��)Z3�Վ]�T���-l'���j�9�cH���D�9��4۸HOs2�!s2١s����ev�B�<�Jԋ}���մay��(d�!��}���]��s.W��춅���s�n�s)%�m�h�X��d�����|v�(�\�&�ʺ�y���'N8Cn�S_�S��8�L��tX%;���01��椝e!��e!S�������d�椝h!S���r&���C-Dd2��+1�
��)��k�h��&�i�؟
ה�[����w�t�J�s2ٵsҮ�M��Zٵs2U�P�E�v
;_�ڭ	e�{�
;�
~N)N����2�T�M7��ַ�tNJv�ũR�� ���PG��}��d�Z��&;�6��$C�B�&;�B�&G�PddR�w|d�9�L�׉֚�$�c���>W��]�x>a� ���R̍l�9��WX��R���d�Z�%�8�n?,�hc���B�%��.1����܅9`gY�Y%;��	(e�0��'�q����S�#`�����C�s�q�m	y������D��mb�&���u�������v�A���nP��`��].1XO�
���v�A��s摽�|E?���xrTg�%��j�Z�(��K;qp\ډ�c�N��N2����!��ܚ8�s�q�?�'{��!�L������p�IvOMvO��L�dgvU��H�jW�V�M����T(8���H<� �m9�qc����Ov �#K�)�wS[rb'�AL��};�p�mc�ee���B嶦ܴ���K��0(�,
��b�%��:�}TN&M�S�fO�4l���M� �J��)nU!E{����˄O��j,�G�X$�M��dK�d����R����WyΪ��uO��]����U�>�z����FK��V�l�cp���]1�!T� X�>Az��(%Ny��7����.��dOC8��=�3�"��>�����.�
��C�>�&J�P���ұ��~��4 r!T���ۆ�o����C�������z�;�F��=\����dǸ]'�e ��8 �ht��Զ�e���N&ٳm�r@��QJ�ݸ��O�XM=&,1��'�����XV=�Xe���FO����E�M�H�1k
��KVzU!��H_1���M���?���bN���-���	�P#}XT��H���y�Ŷ�>��z��[]�2U�v�K�Ǭ��Y�m��&�����m�ӑ>O�>a|�F���94x�V� ,m�X}��š��Ϲ��s�����W̩�����,�	��ǜ�SY�c���ob�1����x �ASsk��t�8;�'H�<j�a೶p�X}�9a�qo�TXO$��>ǜ1QQ~����+Վ�ȧQ5��ύ�|`h��x4����9�h����B;�D����b��_1��Y�ai�V�b�	�',�ثT�y�?pN���G��[ZU$x���s�����҆�EgU>����2a��YK�X��9��&��P\��Վ�I�S���˯[w�g�$����L��?d��Ҟq`3EoL,�̭aƙ�;�g�;Vh�IM����&�2�¤����tp�A��d�X?U�i|f�� \=�0�q��=�Կ�&�\4`r�����f�脽Gl�th�C�kj�z�.e�	{�بI�4�LG��#v�b��c���M)�q�.��>�FM�ע�d(��^UL>a����/;K{��UL>����˪bgi�S��9�|ޒ�)h��;�g�I���C�d��p�x����o`�"FX���ޭ�_X���~a�5����R�	6*�>�FM��-,mS*���g�e����x���uZ/����QY��$�S�	����|�j{���cN������n̸zx����`�6���U�Ǖ��7�Q�tb�����47�L���;�$Op��u�CƖ��/�>�Fͺ��)c�9�sN��f�c�"��r�7�Q�e�Ҟ�c����/5���\YZ���R�ĩo5�끶��&�#}Ŝ�Ky�/�bZ/f��?�F��36j+!un�/���M�cNث��'�/��z�=&��g���TZc[O������بy݄��Ҷ��lT>}�����L;�L0Yϯ3���Y�d̸9c�.|�5k����{U1S� 6j^wa����Կ�������Q�� 8�pYq�F���ח����`b�F�05ʿب�u�F](�C�ҊA���[&�0��FÃEw�Q���݀�Oi7 �S��Y�:�n�p�n�Ч�����)�6�Hښ ��C�U�i�F�rҢ�;^β�	�бQ������):�Qe5� �n*@;]�2
���U� �n]���V���u�X�Ivs���_�.��#S�d��T�E�W���h���n�h�Яa� �Q}�OlT_��VM�FM��j]��Q���aMO�����~!�I�nq��#lT\�+~�����]�)uׯp[�WcJ�ҡc���ߗ���7�)�=�GIk��u�%�޺��.pW_�&\��*�W��>MG��'6����{8c��g9�~�����}b�� �5�{��J�V����ᕰ/RqL:�)��=�6���+��KR\9��A�+ ����i���;�m�����=���=��=�[���j{�}�N��|=̲�!Nبz&lTZ���QS0�.��B�7M���!��G[���X�����e?�5���i���M�y�O���o�|=���B�7�Z|F��0��Fu:ȷ��i�p8^��:���n�"�6�x�$�恍:L  ���?B��?��}�̫~][wL�0n�um|��+I_a���ז����%���y�kk����8���� ���u�uv�� �i��ח���E
`C��6jlT��QS옦q���6<��	�f�E�1My���Zt���/�s����/��w�4E�Ӕ����i�/��4+�E��6ynS�T�)A��d �d ��d�m��h�LS��5�~�FMƩ��x4�)�nҌ�J����Ư��x�8�ȣ㘶�s4�)MV�cJ�c��dń����K�$�d�	4Y1V)MV�������NK_N�i����@y��4B�6�8a��g�O䖙ب)vӨ+��~ᾞ.��~���"�O&�d��K��t��qL�4;�|�f5M����b
�Lݦ���=g!���'�v^ȷ��"��6c[̶�������mR��Q�yAu��yAwY30�dU7d�u~èA��������0j�u~:]����W��_�/ݨ��5`?Ѝ`��:�h�Q�n����Lyۯ;��6f*���.d�q��.ግ���oi��艍�M d��Z��F�.�Q�L�`[5L h`��� ��������s�B>u�����l��1�a[�:�)m�S
�d|q`���3��Ec�C��d�R�������
��ب�X�<��F4��QMyJ�ب����|��O���;6���2,h�c����b+��b���c�������x�_��t�
��ǹ�錍��m��Z�۞�Q���i��m5h�c�ҒNa�l�p�d�QN&E&
�L6*�	l�Q�4ـ��&�f�Le^���7�d���/����/����/�95�j/5]f
M�5e�&�t�[�,"'����0�J����+�u�@w#Xu#��d\u��n�ۍ@dAa�RȉLfvb�&c��>匍���.Ç6qNب����1ֺ�.�WJ��F{����.����Kiha��H�]��0�Jxf��J�7fj�f%	y٬��f%�K�fw}��=+2Ϡ)J=c�&c��t�����vlԔw�e��Z�fD�.���U�<U0����V���vLC�}��*���Ps����匍���.l���^' ��H=��l��2��s�إ���.弴���d��8/m��yi<S�K��p.��a�¹h��{;c��|�T��/������N��Fc�"��tlԔ%�2��d�L�Vc���Ř�uX���d5�h�4!ØF�Kgl�n8#��6A���.�au�.%3&&�.�]J0f*�0�1S��2�;�{2�;l���݁����.��s:l1��M�dL�a�C��V�6j2���[z�2v)�[�]�ssc:&c�5�ب��#6j�t��/�/��4���R9�o���Q�mM_�:a�����0l^l�C��l�T� 3�i)O��-˒��4�/���Q]+-���6j2ֻliZ��Q���q�:07��L롍�ҥ0D�q�7�k��n��3Ś���������/0�˩|���ب���2�)����M�h�3�H
�{c��}����썽q,�4єɘ�H���i��ҹ�,&_4jz���Nبݦi�EVþ	ب�x�ǩ�gǩ�K9N�_ʱi��l��6j2�;͊6�W�,��+�x����)��n0����0��.�$�ӎ�����	�+�9�c�i�X���:a�&������d��-����-��u2�;�[w�5"�d{��بi�X�	L�'l�dlw�2�۰��IW2+6�Q�I�L�$�x�k�w`�&c�;�t�FM��*M�u?a�&c�a�-�Pv]�8��F�6b2�2|)�p�d�w緝�QӞ�V�<r}���v	!Xx������Ҍ���f�;�r�FMu_l��36j2�;l�z�ȡ[�	+,��g�M�m�d<f�R!Ӂm��� e.��ɼ�6�|ȑQX9�y%������$�(��F�-�Q[x�	��5ѝw�h�6j2�;L�fi�t�7�L-��{6j2���-���w��s#B�	5ֽ��{��xʔ=-ql�a�Ǟ�����q�F�	�c7�k۵6j2�;�Qg�&}�L�7�c�vS?Xi%C�3]�q�FM�s�	^�=J c��k����Kqv`|w��c��0�/�%�z��QaK�^��^\�بɘ�p��a�Ǝ����.?×�|_y2�p��Q���e�gvm>��7?;��S�06�0P�P7����5�]�����Q����<�4f4f*MC�F�F��(6���-gl�dp��=��p>�L\��X���N�`[D�$�]�����Q���e��{�6j2�;�y�Ng�N�����N`;c�&C�ˈQ.�5u�L�"QD/[c�ӡ���t��6��6��^��	5�]��%�a�R_
?�b��u���FM{w錍�6faRv�z>d_��}a��(�M~���2Uግ���Jٔ���بI��uL���2/�h���У/�='6*#���_x^������/U�5	��V���;a��j�R�t݆1)/�:r�	�m+wy�ٶ����/�+T5|)�[��fE�)=�p�FM�h��ۗ��Q�9*�&��K�b�脍ڞ)%�ٶ��B��9��+�Q��*�֨CN`;c�&b�/� %1��F��<��{1��Q�@�mV���#6j��/���d�$6j�~��o�i&0p�	�� ���*�6j7��lC*��r�FMBp�a*���Nl��@��Z�g�U�I�V���	�Р;B]m6�(lT��8��8c��j���Mg����-mۍA�Ł��ӱj����iOب�`	�V4j�G'l�T�V�w#�6���e[�0_,��m%�RYƒ(ob�vC�����_��ب�7��,�u�ب�z7�M��Ł��S�j���mtOب���l��8�8����J�n�{�Fv�ha��'Jk�=0���m�*���r3H&���8c�&��7̆��[H��FmaJ�8PZ�<���n��8q�`���h�����,!t	 `����8��4�U�G7�'6j����H����˝��"d��t<�F��36j:�V�J垥�Q�aX3l�d��_�Y�4:V�4I>������q�=qQ�G'l�$��n��f:r:�%���6�,�bv�M�b9c�&�,��w�Y:��%�o��.����%ki;d�r� ��脍�dYg��r�Rٓ�����LdOG̾��D2��,��>T���^ٗ�����6j��̓�)KE ˉ���N�X(t���ʇgl�d��C��s�PG6�;�r�~Ъ{�'��=��/���T�r�F�Fk����/�L�بYE�a�-��	&
�>�/5�fʇgl�,�D�	��5ب� f~�b�o����e1F�5��بy=��ʖ��_�����'~��F��36j^�_*C�~)�pO���� �RO�RE���Kl�,4%���Kq�/m�*��/����=��_�rc˵؀x��v��~id��3'c��<�F��36jld7��gq�6�Ob{�M�g��=c����بĨ�66*m�Nب��#6��Pa�\���_'��� t�'^�Y�ˉ���}�t�N�@1��6��6bB�����k	8c;'ڙ�6�6���׶��;G8��#;���G���N����X�ݰ�=���y%7z��N�{\�C��@��;�G���M����ϘnɄ=��NG0'�~񊇳腾"7��>�� $ k^e��%��~YǘM:m�q<�m���l{=�xd���O�]�����>[��o�����?y�zy��G˗��|���~qy����o^���˿|��w���?�����'���������>��U��g�����>��Y׵mH#��P��5�M��s��EZ��6���o.��j����Ͽx��r���|��凿�⏽��o^�z���E��M������~񣛏^}��G��k��w�_������\>����>�_޽l?nb���g_���׿�B�:?Ѧ��O._����կ��݋�/!>�ⓗ?�pP��[�{�뗟�����?z�Ҿ��C������W_~��ǟ�����r��Cym�ضW��~t�귿}���/{���������O.���w���k����/���߾�w�ɋO?��ǟ�t-.?�թL|鿽x���/�x�����>�����_Z"��~���/?�[�x���[*�|��˫/����/xB��5�8���R�x���?�o�_}���_���������^�Z���X�k��C>���򣗿�����{?{�����{����^�����ś��oZ��o~�����ݼ���������/^����O^|��=���O>����'����콯>����z�V��~�I��cꏷ�(���8�}�������1���:��O� �7��^N��ˏ�����HM��D>��^���է����!������'_~���O[5�B��7�>}�������XN9�_m_�mU�]/l�7�w~��X7Vj�E�ǟ�@�w�i+��u����#f��?����/�x���/~��un����rsy�z���./>����"+\>�������W�_|��^\PX��?�҉���O�sk��^�Q�}����k�O�S�_���W/_~�fi��/?�hyoF��6�����>����o��)p�e����_�Sh͵��^~������Vƭ����>��~��?<���_��ߏ~��/ڒ�ϫF��.-�Ṽw}�����g//����EM��O�x�{Gݶ�{i��?o?��{�h���ˋׯ_|��w�q����_�w��ǟ|t����������6�~�
������Ҥ����{�z���Z�W-�?ą��I�Y���Z֗O^���U���5L��?����W��C��h���׸��ѯ>������'~�^�Y��e~����W�!Ǜ�M�&bP�Q����~�������O��o.Gί_��o�<��тg�O���ԟ�/^����q<�;^Y�;���K����z�E����K�Z�A˵�؂��ES�gܷ�}�������C���gB������}����ڀi	�~զ�/.7(n�4!����b��b!Z!yi����5�����������oX#����Z����߼���W��[�.s:��ǡ}��ӯ/?f��3jv����>*L�^>�pP�����Y���eZx헗׿�Û�lI����֩߾��_.mEi��֔��͛�gK���gK��[��=�o_}�!��}�i�������+H�}�}�´�����o~��U��T�y6�ǟ�N��1�7x		�?m�~�UK��&w\�V����2�|��5�P�����i�օ@��q�x�@j�Rx�jĿ�^�����j\����j�fV�~#�6������F6�w���'�G>j&w����jWzu��ǟ|�9G��k[}��o=����[�7nGT�j����F�g��ӛ�q{�u�f��֘7$|������I#0"_��׎T(�VDz����<>y���,G������|#E�_������7�}���S��3��O?�R�����F����b O~q��n��|S�݌���h/r�|�Di˦���K�����͇��}�������+~�7�K��R{��p�0��E*E�o_}���W�=^�Km�\�L�nB�`��A����C7����c돟?��*"Z����ڦ���
a)r�~���/g�/�����>k�:�7_�;�������`�5�{֙~����B�j,�M=n�=�z'-�?ú4�|�o�B[ `�Ǫ���u߇_�����o�T{�J?.;����˧��i���-�}�um����ԟ��w{��ܝLi���S���k�y|������ɾ�K<��������YIo��G_�_�����/9�:��;���'/�~���?�����6�_�_�?n����ڶ��~3�oO�??y��G.�#�R�R�j �s[�Ӆ�����+g4o������U���~V�x�r���h�7h��x-�����3!}����7Z�28S�`�m��i~����/�j��M��oO*�Y��x��)xa����)b�Ǌ�@k��8GP�ϒ����ҁ*���/^p\P�q�/��x鿼����EO0��~�����7?ʗ����(1��͏"��>
�_�Y�ߦ����">~�7��7��_�(�߽9g�ɛ�.-�ߵ�oL6���W��sQ��,w}�B���7��}������7 ������ʶ���/,Q��~�f���h��m��d��{�
3�mKu�-�������w�+o�۪���a���������~����ڶ��G���u-��#ć��&��z��P�t��R��|��z��<,(�7����>h��c|���ܯ$d�p�����6\��XS-w���u�o�
�u�桕��f-wk������Ҟ���ć���
y��r���M�G�� �n7����a�o�v�p�|[�wK��a���_��|���Z�}���u}�Y����u�]{K�e��Z����������F�Q�^Q���>�C��n���!$�Ѫ�n�p��u�	۵�/��Z��5�]�:�KB�����bJ��5o�}��Ǻ��M��ZN���<�fm�V��%j����0r���5ʘP��J���c�I������)[��r���kU�A����Z�U?�����S�fa_�V-����]�ع��ϏV������QrԶ���J�!�ʂ�0��fi��kkJ���]{n14�&C}�P0�����}+��o�����{�7J��?V�e�?Z�^Y�۫��޻�ז�vۚ+���b�]�x��okl��߇��_09>���9Xn���&D���0��v�4\� h%_�pۊ�꼷8�I�zk,��+�C�5��Vtx9�#�5ʝ>lݍ���قy���u�ElkN�o���ZoK{q+�V{��6��{��5l-.�n7�Hh۵������|ޒn��=Kǂ1����;|�6M���6���j_w��6�r[�77��9�bxx�)�V�y�y����zSjm-��V1��Zo�`����6���k��-*y$d{�P�P�$�-�{�����K�� ЦU��a��]q�8`� kc�h" dp(�d��w�hi
m��=�!:5�����B���Ʉ�|�Z�� �i��\k��n˸5[g-��[�!®�&�rw�����������p��j��4?J�����ju���u	j�&�~���!?l7{@8�b���;��F���Uk�������g��u_���vݮ
�A��;�
y����p�2��ncp{x���Y#Fd�5F>K���������m�m��7mܵ�j�p����俥�m�t�v�����E�J�y�s^��]m�������ݶ���kMݣMݏ.�e����$H6I�&�,���Y ]1%�$��{A�J�G+�>E}��|	 L�U���!�銹�Zf���r��Q��>��D��]��z�ƚ���|צ���
QbsE+wO+�ƥtjǸ�������,�`���@Ep�ݤ��z��M
$<�mj�ת�$ց5���@}Ke���w,��� ��dR��	�wX�}@�R�u���Y @Z+7��n}���aˡ�T)Z�+	#�!�ƺ�h�r-��l`�� ������Ѯ��-��F7>�+#dv,Lm��l7��&X�Oι�r��������nWL�j�<�'�^[S�U`"p�
z�J��B��nn� ��r���ǭ��+.�����yk�t�J٠>�v�P�`E{�[��,���66(õ.l��i�!�Jن{{�%�
����?#4Պx@��y��[� �q����*B8@︧.t��(z��Z�[�]�`5c�B5I1�\[m2�s�%�4,�h�	��a�pl�`;c��$mrܡ}�ܱ��� a�[���
�n7����Y���=��ĨB�71��؊7�=�^��q�h��L�n�_��C�1��43T�5Q#��-4� ��Z���L��6j��&�#�kŶL��цP�5�p[�][�������pԺ	��ZaO�&�rYG��7��
�V؛l�c���|Y0e���Z�B}؛ܸ�����a
޻���Ԅ!x[��aQ>���5�R�ZW��$6��ќ�P��n�VW�DM^/)�hC;F�v��X��i
.�/�Pmw��ٲr̴!���]E�~c_��z��X�X���m�,��Y�M����,w�tI�k�A(�$RZ�Ry�.�F(�Z��/�,R�*�W�n���\�y���i���J�[��'�BMˁ\������ �G���������o� �|��n۴�������)�7�����@����=�f�ZL�&��
P��s���}.uj,u@XN����m2$i��2�dΞ5 �t�[\�K���M������mO�m��zDhU�!���ZBǉZ�!�ڒ��s�_Sx��k��+��������6����J�H{X<k��V�%}Ϝ���dx��?�.�����Wj�L���+�vx�	����ڡY�2@x��T=��c�Q��W���Q�"���3th$��Eq��9��� 
-hH��u���6C(���}��:xҹ��v$�G�2z{d�����{h1�w?ˀ��mj���{X���)+��|�����/���bח/����˟\���)r�%}���"��|���/>�_����Ӥ��l>��M���W��݄Q5�ywa.j�n�B�e�����M��8��\��n�%�N�Դ}��<��WQ	o�]_�#���>�ُ��C~��o~S�7��7Bvk_�Ps�%�#�%�S�(N����s��"�	r
�7t�<�Z���/ξ0�q�����H򠏬 �d����Sf�ްOwcko�.��r�;��:?r#�nz����)dϹ�@�A.3�;��w�d�1ja�I���M&��(ݜ��sc��n.p��i����@h ����}�΋���D�o�}�\�8����t��ħ̔Ȼ��f��᭑B1��	���;���n� ����黱"�����w�Q3cx���i�F��S=�_�v�=�-n���V��5T������AhK�3���/���r��S�N�3��|��T�� r���o�^�ǂ��ޡ����9�U/��c~- @�Xn�����=���i(@��&Q�aKo�K��T���#F�<�%d�m�-"<c��5�lЙN��u����Y�!H�����3E��6G���V��5��1>z���<��e��ԩ%���H���&��T�91�M�& �S�8�Ǭ�#��v&��a�p"R�!G�!*{�Y���ڄ稴�1;��@f��B������Y��m:�Y���#�s�"�t�Pq=mG�r�&�ڍ�p�}�m��Y�M���t/D�����Ync��#%�W=����Y�b�� TӞ��!���m��؞~6j/�#�1�w��̅���=b���Z��
d�/�H[s���T��i ��i;b��Ж���6lXz_:b� q5�FKW�(T}v�#��"g�ql����]�(cT�'�ȸtA�c/�#z�,���B>��(dO��$D� �?�f1s�i+b��:���Pp�i��y�9a����ݛz�loұ�/��&�6�+�p��rق�.z�1ܛ	ƍ��U%N��1\�p��Ѝ	����!���V��ʅu�R��#�k�R�c�#�0�➖o-5���,Im��ʇd�ЋafY�u4:�)KEl�VX�����N�{w$�����">�( ��!�p��z
rU$��п��ÿ��AX\;ۨ\FIc.���Q�����M��@X@!�:ݘ	 �H*[a��Swc&��0�#��p�T'L@�#)c��X����4�����N>��h���~���e4,�R���P��� |�`���K�zzq�� (�F�nz�{���r�,K� 1?��c"��&4%0�ä��ϞM@d;䳭��L`M����-Lh�*��G{��<q.� �)MB� ��$�C�(�ؚ��@�H���_6UxPv�B9tjRt���r����iu���^��H�	��X��+�y�o`�>�6j�Ķ��m�ٶĉ�T`$P8Ah�I*R�H F��3l���@��d��ږäèls��һ.�6)Q����A &������F`��q��m.���&D+VC����2\E��F����}�	N����	�E�H3"��ے���z�C7�H
Q���� �Y��h���$�У����1pvV��¦p��)�6��KTᚨ��j� ���0��hҐ&��2E���C�e���QYO	�Lᔹ
��� �)z,��&����T���v"��O��=�1r����P������
��x�p��+ZXMw���%�O4GNx��}q[� �Ĺ#QE���FJ`�I�캬<�ud���j�v����6�d�0��K�3��HX>�KE����&�oM�]c/JQ^:�@��B|C��˳,��_�y����R�3�<�q/�����G �D��V)?;�W¶�t�("B�|��ʜ����6QʑH�ld��)d��Qa�K�)��5]!'P��,a��FY
ihH �	�����)O����
��hb�*Y�3s!���p��c#ϼ.р	��E���K�_�� ����XS��UtMG�����X4=6fwj���:���e����S!mU�Ш�w�wj[2VI�TCf �N�����H������	�L�G*�k���5����[c!ǔ�Z��۫���q>�c1�
&�C�`ZfЊ �ja�(��ka�l��U�[�XĢ�ϗ�=������T�F�����,"U4�"���R�Ze��H��C��r��=�
Da,#������.5�fL���&�y+�Q6j��F!U��ܢh�έ�B��SR�*ǔ�Q嘒< N�Y��+T-���2�.L�`�69��Hn4ɞ��M}���QMj6�@����_�GdQ=$�*Ǘ�Q���*T�k&l2�#�2r|I�1�C��ʯ�X���<2a<�ϣQɣcE;Jk�O�X3X	ǚ�>ka�$͏f9F_w�@ca�.#���Ĭ�=�٢��д�T��ɗh )�����\�2~ԅI����p�`XD�T�c�����V؆��{�\hT,�h�,yvڣ�B���}Ԕ�U�L�Рh�.LW�GMc�Q'm�T%�T���[S�D㇑���/r�U�2�UiGM��2
:��}4#c�����W%�H�W	�H�KN���|�5�%��Qך�_8g����A����	l~�<�J&a9�����uĥ���Q�]b֬�ûɣ��(�:.�6��W&dh�����SEs���q� ��V�(�!Xo7�ƵP��zĚ�'d+#�|�F�����>��G5��a�+S|�,!�(5��UW�\��(����|�n������?���e�x7��{T��Qyr�G��k�j��j�q�y�>�ª+�{P]9�iBW����r��x*_������r<�u�;���<AZ)�In(��(�ۈB�L+���<��Uyr쯪+�>�T�뉂��n(�Cu���f�[�&�	.ď������ I�-¡r�i�X�^'\�	�[Db{1��(����R��p�0J&�(Zyn)� I���*%�k���T���b�K	��ѳB��J�xK���c��(tUnġ�]�� *K�:ha�!�]yb�+Le�(X�D����"
B�����GTu��ª+Y�w勹RD��~+D%��Da��ro�N�7����Z�@�o�/t�bzZ�0�K"��s�PW"b,����,��T���Jlɥ��ϲ�J&y�Xan	Q�gg�H�2(Ryg�#��גM�Ou孂dU �|�u�<B2���ɪ����x-����(Hf�Hr#����X$�pΉ�
��yUW�3Q'γ�|9�$���dS�<��7��喬
�a��,p�I.�8
ޚ��Q�Ld^���^x ��3�y���B���[E���=$�"/4%�"��d�Ǣ��S��[9�y�.�o�0Fa�����S}L+���>
c�G�-�)���h;�
�l�K�9/�0�N����u���+֭�r��芌�\�%�@-�M��n:��؁����l�������Ϋ�(������� ���ȍ��g�Vѽ�Nj0^�D�л�A!P��"���(
�>ŭ�ww×a�
�WO-�<1_w�&�h�;�0��.��{���И�B�'�[J�=���y�w�Oc��F{�|�%�\����b���M�?�aK�o�W��*��#�X�hu!�^��M��Z���gi�l7��.�$�"�&޹
ڌ׭-�1�y,�^�FQ2��WT����p {#��/����ިC�Y�1�qgݞm��aOq��R$�p5EI�[vRU,�`����]��-xMEy�Qaಿ�Q��v�Ґ	�.���=ڐa��m�h9h	�����h<d`!z�VD�~�B#�Df�	���.���������iGx�Ak���
b�����z�I��Mr"tᮂ��W�J��=�q�qu7����I�9�T�S�}2�I��L�Lb�h�c�_ o%�b���SD�"�#��I�`�a�	��Eݑ�,vR-_�?�0*���ñ�q�Σ~���8.]e�穦��΋�ഭ�Z:L��J�h3<�q�� ���.�3�@�>M\�3�Δ���j��Qp���k���Ў1P׉WΪ4ۏŚ!�����&Ϋf�l����D�]c��:n��I����h����m �
���"�Qp�1���.&�`�$�e����ª;�����q�}�ڊ��`a�Z��iШ=w�'�0=�6�Q�i�'���9t�]�N� ��N������m������G���W��^���}��o@fAHY
��J|������������\6`ύ��-�� �� �Z����� � � � � � � � � � � � � � � �� ���  �&U��A�C�|)F���=<���{? A ���+=0_��S��P��p-׻uy�&!� M��X �
e������O�V(��]�Y�;��=< ���aAN��</����300��r$������2G�MMh9���47ſ�.eE�Bi^?&�PL��� �=��- �P��2�����}^�߉�u��?��*���P=n�Os]���a�ʚ�B�&?��&�ߞ�j�j  )��¿��x�!-��*�^�����HD��
{�a5�Oj�X�t�~Y`����R����@
+B$�
Q�)�
�j����+���uOz �����'`������ 8Z���!\��-�A>5`�1��xrWK-�}%�Sאo���pV��f�/�]�Y�ϛ�A��е�~�=�����k�+�������������Pϗ��F�5c����vxV�������ټ��=��na��`3��]�{ u���?,������?$�f"�fz�����<����� O.o�<�6��� O����6ȓo<�|o�I�m�ȓ�ȓ��'�q��i�÷�8\�4���C.���@n��ao�r��@��E9�s ��ۢ�9���mQ�����(��py[��?r��-���9\���ρ.o�r��@��E9�3 ��ۢ�9���mQ�����(��py[��?r��-���9\���ρ.���v(�˟�9�#[b����;,�m����}�R�kR�buh]��^���#�+��80���Uͮq��ׄsO9����@���`��f��O`',�:.`�+]��	�F�OF��z�x7,+:��F�]�e����|�fX�a+��*yF�:ޮ���aE���/;�K�6�D]������A�Bͳ��1� �_G��q�z�Ⱒ�4�V���T`��9ͷV�zz{�Ke6F*�1пV�M@>A�l��
��s��8+N&�A�ň^O%_gS�av��}�-�����V�_�����I�
���o�HH���_v�H��Vr�o�9�a1�;�r2o�%s�o�x�U���'�W2ƥ�;��_s.6��m��6S��f����T�|�ޏD{�1�7{S���5F�O�~{7�.nk_ � D�\�3��hP���8�w�{�iD nQ�Ｔߑ��u�PFa����'Ab� X$}�dr��$?���z4VF0b̮&!� ��J#����`��I���=@�Pu<J�B�����_�XM�����L��A[�*��AT��p$�5��w�vڂ�;����]�%������x�v�s}�=\q[����KC�l�I��>�l��qق,\\2]�܂,��2���>L��[�gA�hGx�dzT8� ����v�tڠo}��l��,bijP�A��²\�
.(Y���6�,�3M �[�u?��R\�}�C4�~��-x�2p��t�90�2%-]�3��`߂(��3���%g�@��>:��4�G��Y;\��R� r��Y���H/��Lz��2�S{�&�蜥I�b|z�gztұ>�E�H��4n��X d���81�S�� \��U� ��|P���p�qc�3G1�$h�G$K�ۃ���3t,��ѕ~[OY��
�}���}l�ۆ@����8����q��hJ����~�� ��Ph"H�)�W �ҭ)�JB��82���˸q �v�m�߾q ��aἆU�L#EzH��o̒��+�޷��2����s�̈́�)H�%���6/��Ĝ0��M%�8�6��j�T2�M �؝�ia�M*]������m2>*v*j%#6eQ�0v6n�-�B(��u��a�l��FF�Ke���x!�f陟J���X�Fzq�8����HЫ�$ߎ����UF���~3�����ڬ�m�%tg��t��io� �����a(�!��,*���Y�9�
��/- ���j=�!y���D�Ң�\���K�r���A�sI/my�zf˃/z}j��	wm ��Z��P��A�M'i9(�	�q1�IZ�-���c�� [�t���p�:f������)����	�\>�����ղ�4�uYn�!��q7P1]O�Sb�ȉ>ɻ�)}���
���p�ma8�j�҉x�`�G�CS�X$��"����{J������h�O.Esh��b������Ĕ��)z���kң�taט�l1(4�֍��ΥG��<D9�s��$1��5���c�����2��J�����L\�0%���-���Ѕ��Qr�ĉ�X�����~���~�t� �]���O���c�}�S2%ց���)c�ʙ��ͮ��]J���~f���}"2T�ϒ��?eL=��Ŏ�2}	ר�ca���g�q�����8��82���>|0�6"���O��>QV406"���?��4��(!�+"�����d��c�,��'!��w��������+Q\(���+Ȭ��c��}"�hU�S�`�zy����Q���C��;K���/��S�D=� ĤWqk8���E�:�_ ���_�%����;*����3���u���}@A��3�WL��@�!��A#}ǜ��QG�G�O��S7�P�3/�69�l�"���w�1˓�#1W���9��������� J7e�>FD��mX	gt�ܹ���#� �#!�(�e����y=��.a�=8z�~z���I��!���F�P��,[�=ru�����@�y9�����Ĉ�f��8�E@�������	c����1u�5u������3G�� �b�� ����9�75���Nm���4���8�.q�&BT&�6�꫘���a ���~��/d��L��x��Lh�8 v�	8ǆcN}���r�&��}�9��̩+�;�c�N���Կ��Yp��[��x_1q��*�Pa{$�ў���C&��ux*�?O5�W̩�M�̕1b[5�W̩��s)z��M����cN���t����^�� w�4�w�'Än\8Os�1����%x�jh�1�s��N��UЗ�Z멾��i멾��g�%$�zώ�s~.��9�0G�� ���"�g1Di�ۚ�+�T_�Pz�]uL��cN�����ƒ8�=}ǜ�K�M��u�"u*?��t�_�"�� y��cN�?�%(>ͺ����}����6�ԲS����:�x��jY=��1S�L`1|�a��ў����_��3|�*Ȱ)z̬/���+��5�W�~z�g1��7��O�vJp?+u�2�'��������Q�F��Sf�vX2�jQq��T�9�W�^�4�	o6�,|:�SOPgG���(&�����h�P\XmG�����
�c��������
6*��H�1��h���:����g���>���/.���^�??��ͪ� �@����(�J!Zi�/D+��B���?&p?%D�<�}���4"�.6�B�y���m�]�tO�T���$Fx
B��USO�׍�[:60UZ��)*�9Q��Q�����E�h�~�̓�"�x�pO���^om.�D��)��t�&T)�Nu�m���Ĕ^LjT�y��^�`AhQ���^^b��Yl|����
UՎD~j��6��ē"U�<��C�N>���w�'�;e� ,Te���
��'�!Q`�ʓX:�����(�*����˝���s�Dq#����IJ�Ȥ��D��DVA�^n
(��%�������N��z���+�������i�0�]9�u�2�����x�ҧ�i�^wJw�&�Q�Y\V��N\�Rx�}/_�	�al�gu�< �i�a�@���:}�i���îd�z��w������ҩ�����U0�Q*�>�q`E��2���j�p/�Op���ۓ�zy���l`\����uҙ���J�d.�̐ڏDOfJ����WHe�Ž-!�s�����*ר%���B�fjjW�G��rt����t�e�.�8#GE���F�E�q9����CGen+3�qcز)+c��z#����6�!)�zYa�z���&-�T�݊l/19u�c�8fQF�k^�}�����������j��Q4h]���C]�{�� h�;	���m�̭$1�Þ�6�����4�,�
�sϧ��XG�B6�Z��c/�b�|B�p?����o�z��_
Q�5�ˎ�z1�v�����e/w��v�p�E��J��؟Y���˸?��Z��,�4�*�QV�Y!�.��jaˬ3e�����6�"Z��ϓ$�#�����#.4���T����ѽ�i�'���i���-�!y����uD�����:�|���3C���s�@�4:��7A?R�=�z���F�3�q������R.
d~`��_v�A�(l�xc+�O�'�G��U�����+�o�eE��2%���x�,���"�/M%Qi5�}��zֽ.Fq&-��H�žT���Tn��,�{G0ڢ��%�V�����Y��ay<��ꨈQǰ<�(��mR	�Z��xم_+�+!�`��2H��Y9��R���bk�'�!A㠳'�}�NA��3�8X�xKY�ȭd���C�E�Xg��eV-˜��y��Y4�]N�Z��� Wk]Kq`	{X��E�y�#P>j'��?�Q`�:�s���X$�-�t�[1�6��n�O�!����6��G�BR Α�`��iS��W�T��Z�|Dh3��I���� (ⶪ�2nV�kg���C$u���i��^"� Q�.N��K"� �/Z{��D[/���ח�z�Ÿ#�^A	�W��{���@Zz����X���8*�}��>ibZu<M�SI��2:j�$v��/����<\!��$��o�٥��m���9r�$����W!5GԬCx!5�tg��'�H�>	W�f�����a����G�}�n����|{�ۃ�o��?�m����g=�Y��ML�A��}��}�I���F
�e��BF�m�n�g�K�YHO���`��ģ�����Ͻ�0X�MC�}���P��K�֬<9~|-r�[偭�>�Og8���ŞǱ�$�˒a�)�f�(ڸ���Fh�i��i��f2�Ѳ�W4�� ��j� ʲf�.�~!4���]�L4��Mh˘�yі�䘓 �LV64B���LI�(�C�����C0��"T~��sn�vS�
fc7��]yr̙�F����mf"��1�ms���q.�$A�(�JJ�?�4�rl����=̈����SJI�`�,�@�${`KH>>��n\Ţ��k���},#m��	�n�E�BXr�rLVn%e�E�AZ����Jne�.ڪ�����.6E��&y��&G�f}-,�bR��mg�%��i�g:B�b��9����t]��\����t���v�}��D�#n\e{�֪�����Ѷz�,��	m�GcB�gY�4�[6�#,%�6�A�� ^�m�I*�>�^��vD9���ӥ�6C���,e2h�F�	��Q�p�$�Ж�h�����d��1�L���Q��h�S����8v�-q����e瘍��l�ׇ��6��H&m��3F5��7_r�J&Ѣd�5'o�$�0a�ʼp3&�TNk��r�ۊ�"�ƭ�6,���h��IN���K;�M%���Z�:�(�	�p��P���f�dZ��?�j&��b�\]��j�"�Ƽ��m|)�m�K�A[�dІ�.w���\�lOLR
�^'�0W�~�p���X�s5�e��y�r
\�w	!�a�l��m��b8���QK���
�^�3cڌ�j���u�+�k���G�#���'��m�M���׽���λ4Q?�%㷰�ĘΒK4,�bۉ�.�D����U��VM.o�$���-թ�ڀ�����iq��H���wW]�����̺��~#]k�����H��Q�����Ƿ�Xqk�%�
M��+�Ґ6���[x༷0�0=��dS�%~6�g�t���P`fM�(_lJ�h��p��]n	d��� �O�iѠ:{��{�*�z�1�Lv��^�Y>�O��$	��Ӡ<!�s4�g����-,	�f:�k�R��5�	���M�c^�$���7�vh6c*ǼS�?�|�@B9�zN}�p̛A�cdrG��y�Y��^tcl>�6g�/�e&Q�i�)@�'3��;��#�}���G��xc�3���]qx�o��qGA��yd��̚z䋽d��̚��X�b0=��B��?�9M0�i$���f��{�d���$�h}"G=��&�&X��F��FI���{O��&�����p�A���4�v��I%K 9XɊH~W�Z��E�#{iɒ)�95���E�'�zɄ#t0Yb%3�ҩ�̩t��]�ma�6���S�{����	vhܤ�ʸM6�d�T�?&3�f�eӕA��x�f1M�,*�t̔�u!I>U8�$�'�rӉ0�H2{��1eu�b�wm^.��2�t̞�y�̞
6�d�T̓$�"ǘ:{jP�6���$�蕅K��f�#fO�1{*�]6ŀ�̞�9��SQF��b�HfO=�r��r�H>��4�=�s���"�����I��G�I��f7I����:�*�GgPe�fPe�fPe�2�����tt�J�A5� ��F<��j/�t��V�<��4�=TӉA5u�V��TV:��oEhK��#�b����AuCXuME�@�fS��1uE^�� J>�ėJg�͢�#L�HF�hU����2��FX1��X�,�LG�b�%��͢�����$M��֣��`#3O����<O�cgQE�:�j�i�¨_gQEۛE�\3fQŜ��O ��������]�i�E5�t�a��,�X?�YS�70��ɢ�'aE��@�cgRE��êN)f���!�/��f�3��9;�j���l���E��hfŨ�6K�Ql� B�Q�`�D�b�A�e����#�I�G4�*�q.��a3���fR��ͤ�}f4�jd�ʗs#�5�s�3�"�Τy��p�2��g����U�O�~l1����)5M٘f�j�D-�4�/֍h6U���b?ͦ�yb6U��l{���nL+���|	fpE�\��?����h{���b�ͦ��6�*���Tq�ͦ�9c6ղ�T���Q��dh<Ck0�*t�`6U:3�Ms&t6�&s��T1g��SkYգZ�aW�iW�iFU�'�3��+_��jfӴ�#����X���Y[�f<��`^��]���Z�����ۣYYA��pѽͣYYC���Ok!=����w�U�[��w�u��`�D̟����'���I0�*-�lf��E<e`fmy�Q5�O=��5tFU��U��V�Ɗ4͠��%lfrE97���63�-�Ϊ�����L����i*_̟`VU̟`VU�3���?����:k&��BgYeZq�������zg3����QuՅ��X�d�C��'�R,�d`�Q��fU��:�ꪋE��2�)�쬪HӬ��KfU��1�*֟`VUΥΪ�q�YUQ�Ϊ
>�Ϊ�4�/��YT���`6W�4�8�$��:�*�ܙU7��0�1%�B���)���`fյs��}�ų�K/XCgZEZ�d���:�*�3�j��̣�V�d]QV����u���(��dVW�(���vfU�$�7��̪Ls2��'fյ3��1�JF�s�̪H�3�"�ά�!,�K̥�3���]'���̪�d4�*�OV�>��s�̪H�̪�ì�S��\�YNW��<�!u-f9E�̮JrI��b��vvU����i2yb�f[%�>�z�
j<���fV��Y;�j��X=�2�)�����G!�j�e�okgRE�6L��Y%��$�nf9E��YN��YN��YNіfW��Y�d9]�d9]�d9]ͮ����]�g�y0��ҥȷ��]�(@fW=�&�Mp�X�	�&��i&�����L�HSr���k2�i�Yɣ�KW�)گ��Sd+]%��V�F3��̒S���֛��Y	�j�!U7��V1 c>�)6T�c􌼄�2��s��z�p�iq�D�7��`!��>��*�Ufk��ԇ�ϭ�=!\���:�x	�j3� �LW;����N�a����z��0iL�9�ܦ�"�af�$�u�����fƴ��(�I��N�۴�Ȕ^b2���!�0�>qH��U�1���.�^��qD�V� ���7� y�p�y[z�ђDH�;I��������IKN��uIZ29c��rJc0�#�U7ӘbgdE*��m'v�F<jG��R��#I��U��]y����A�%o�p+������cy��2�N-J�Y[��g�:�M>2�qk�����E`�t\��M�S����h�J������������=�{�������������i�e� �                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   
